A global view on star formation: The GLOSTAR Galactic plane survey. VI. Radio Source Catalog II: $28^\circ < \ell < 36^\circ$ and $|b| < 1^\circ$, VLA B-configuration

As part of the GLOSTAR survey we have used the VLA in its B-configuration to observe the part of the Galactic plane between longitudes of 28d and 36d and latitudes from -1d to +1d at the C-band (4--8 GHz). To reduce the contamination of extended sources that are not well recovered by our coverage of the (u, v)-plane we discarded short baselines that are sensitive to emission on angular scales $<4"$. The resulting radio continuum images have an angular resolution of 1.0", and sensitivity of $\sim60 \mu$Jy~beam$^{-1}$; making it the most sensitive radio survey covering a large area of the Galactic plane with this angular resolution. An automatic source extraction algorithm was used in combination with visual inspection to identify a total of 3325 radio sources. A total of 1457 radio sources are $\geq7\sigma$ and comprise our highly reliable catalog; 72 of these are grouped as 22 fragmented sources, e.g., multiple components of an extended and resolved source. To explore the nature of the catalogued radio sources we searched for counterparts at millimeter and infrared wavelengths. Our classification attempts resulted in 93 HII region candidates, 104 radio stars, 64 planetary nebulae, while most of the remaining radio sources are suggested to be extragalactic sources. We investigated the spectral indices ($\alpha$, $S_\nu\propto\nu^\alpha$) of radio sources classified as HII region candidates and found that many have negative values. This may imply that these radio sources represent young stellar objects that are members of the star clusters around the high mass stars that excite the HII regions, but not these HII regions themselves. By comparing the peak flux densities from the GLOSTAR and CORNISH surveys we have identified 49 variable radio sources, most of them with an unknown nature. Additionally, we provide the list of 1866 radio sources detected within 5 to 7$\sigma$ levels.

==> TabCan.tex <==
\begin{table*}
 \begin{center}
 \scriptsize
 \renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\caption{}
 \label{tbl:glostar_can} \begin{minipage}{\linewidth}
\begin{tabular}{cccccccccc} 
 \hline\hline
 GLOSTAR name& $\ell$ & $b$&SNR &$S_{\rm peak}$ & $\Delta S_{\rm peak}$ &$S_{\rm int}$ &$\Delta S_{\rm int}$ & SIMBAD & D-conf. \\ 
{}& (\degr)&(\degr)& & \multicolumn{2}{c}{(mJy\,beam$^{-1}$)} &\multicolumn{2}{c}{(mJy)}&class & name \\ 
(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\ \hline 
G028.0142$+00.5778$&28.01418&$ +0.57782$&5.2&0.20&0.07&0.34&0.07&...&...\\ 
G028.0181$+01.0039$&28.01809&$ +1.00390$&5.1&0.34&0.11&0.54&0.11&...&...\\ 
G028.0210$+00.8308$&28.02103&$ +0.83082$&5.3&0.18&0.07&0.37&0.07&...&...\\ 
G028.0217$+00.3191$&28.02170&$ +0.31913$&5.1&0.18&0.07&0.35&0.07&...&...\\ 
G028.0252$-00.1458$&28.02525&$ -0.14580$&5.4&0.20&0.07&0.35&0.07&...&...\\ 
G028.0288$+00.7505$&28.02882&$ +0.75047$&5.0&0.20&0.07&0.33&0.07&...&...\\ 
G028.0295$+00.1057$&28.02948&$ +0.10573$&5.3&0.20&0.07&0.39&0.08&...&...\\ 
G028.0431$+00.5314$&28.04308&$ +0.53136$&5.8&0.32&0.07&0.39&0.07&...&...\\ 
G028.0514$-00.7841$&28.05139&$ -0.78409$&5.1&0.18&0.06&0.32&0.07&...&...\\ 
G028.0573$+00.2387$&28.05733&$ +0.23871$&5.8&0.21&0.07&0.40&0.07&...&...\\ 
G028.0576$+00.8389$&28.05756&$ +0.83895$&5.1&0.16&0.07&0.33&0.07&...&...\\ 
G028.0790$-00.7437$&28.07896&$ -0.74374$&5.0&0.18&0.06&0.32&0.07&...&...\\ 
G028.0894$+00.5602$&28.08940&$ +0.56018$&5.3&0.20&0.07&0.36&0.07&...&...\\ 
G028.0980$-00.7435$&28.09799&$ -0.74353$&6.7&0.25&0.06&0.42&0.07&...&...\\ 
G028.1029$+00.8823$&28.10291&$ +0.88229$&5.2&0.19&0.07&0.33&0.07&...&...\\ 
G028.1052$+00.3603$&28.10524&$ +0.36031$&5.3&0.18&0.07&0.35&0.07&...&...\\ 
G028.1083$-00.5941$&28.10828&$ -0.59415$&5.1&0.15&0.06&0.28&0.06&...&...\\ 
G028.1265$-00.5728$&28.12648&$ -0.57276$&5.3&0.17&0.06&0.31&0.06&...&...\\ 
G028.1274$-00.8462$&28.12743&$ -0.84618$&5.2&0.17&0.06&0.32&0.07&...&...\\ 
G028.1287$+00.0694$&28.12872&$ +0.06941$&5.1&0.22&0.07&0.34&0.07&...&...\\ 
G028.1396$-00.5791$&28.13961&$ -0.57908$&5.3&0.18&0.06&0.31&0.06&...&...\\ 
G028.1467$-00.0044$&28.14671&$ -0.00441$&5.8&0.17&0.07&0.40&0.07&...&...\\ 
G028.1484$+00.6347$&28.14842&$ +0.63470$&5.0&0.20&0.07&0.33&0.07&...&...\\ 
G028.1512$-00.9582$&28.15117&$ -0.95821$&6.5&0.54&0.08&0.47&0.08&...&...\\ 
G028.1527$+00.3982$&28.15267&$ +0.39823$&5.2&0.20&0.07&0.36&0.07&...&...\\ 
G028.1540$+00.6003$&28.15398&$ +0.60032$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G028.1731$-00.3190$&28.17309&$ -0.31900$&5.3&0.21&0.07&0.34&0.07&...&...\\ 
G028.1811$-00.3166$&28.18108&$ -0.31657$&5.0&0.21&0.07&0.32&0.07&...&...\\ 
G028.1861$-00.1841$&28.18608&$ -0.18414$&5.5&0.18&0.07&0.36&0.07&...&...\\ 
G028.1933$+00.7231$&28.19328&$ +0.72311$&5.2&0.18&0.06&0.32&0.06&...&...\\ 
G028.1944$-00.9473$&28.19438&$ -0.94730$&5.5&0.18&0.07&0.34&0.07&...&...\\ 
G028.1961$+01.0159$&28.19611&$ +1.01592$&5.6&0.43&0.12&0.65&0.13&...&...\\ 
G028.1967$+00.9778$&28.19673&$ +0.97779$&5.1&0.24&0.08&0.39&0.08&...&...\\ 
G028.2062$-00.3023$&28.20622&$ -0.30233$&6.1&0.28&0.07&0.44&0.08&...&...\\ 
G028.2098$-00.9912$&28.20979&$ -0.99120$&5.3&0.24&0.08&0.43&0.09&...&...\\ 
G028.2309$-00.5053$&28.23094&$ -0.50532$&5.1&0.19&0.06&0.31&0.06&...&...\\ 
G028.2328$+00.6970$&28.23280&$ +0.69699$&5.2&0.25&0.07&0.34&0.07&...&...\\ 
G028.2336$-00.8801$&28.23355&$ -0.88007$&5.3&0.17&0.06&0.32&0.06&...&...\\ 
G028.2432$+00.2024$&28.24324&$ +0.20239$&5.4&0.19&0.07&0.36&0.07&...&...\\ 
G028.2433$-00.8704$&28.24335&$ -0.87042$&5.2&0.20&0.06&0.31&0.06&...&...\\ 
G028.2461$+00.0148$&28.24609&$ +0.01475$&6.6&0.42&0.08&0.53&0.09&Rad&G028.245+00.013(F)\\ 
G028.2467$+00.0132$&28.24671&$ +0.01323$&6.3&0.50&0.08&0.50&0.09&Y*O&G028.245+00.013(F)\\ 
G028.2572$-00.7280$&28.25718&$ -0.72798$&5.3&0.16&0.06&0.32&0.06&...&...\\ 
G028.2587$-00.8857$&28.25870&$ -0.88570$&5.8&0.20&0.06&0.36&0.07&...&...\\ 
G028.2655$+00.2452$&28.26546&$ +0.24524$&5.0&0.22&0.07&0.33&0.07&...&...\\ 
G028.2696$+00.9173$&28.26960&$ +0.91729$&6.2&0.23&0.06&0.37&0.07&...&...\\ 
G028.2852$-00.3643$&28.28518&$ -0.36435$&5.3&1.62&0.21&1.06&0.20&cor&G028.287-00.364(F)\\ 
G028.2872$-00.3710$&28.28719&$ -0.37101$&6.8&1.01&0.16&1.03&0.16&Rad&...\\ 
G028.2885$+00.8414$&28.28849&$ +0.84138$&5.6&0.20&0.06&0.36&0.07&...&...\\ 
G028.2906$+00.8041$&28.29058&$ +0.80408$&5.6&0.19&0.06&0.35&0.07&...&...\\ 
G028.2969$+00.6489$&28.29691&$ +0.64893$&5.4&0.18&0.07&0.34&0.07&...&...\\ 
G028.2998$-00.1643$&28.29977&$ -0.16427$&5.6&0.22&0.07&0.38&0.07&Rad&...\\ 
G028.3011$+00.4888$&28.30115&$ +0.48879$&5.0&0.35&0.14&0.68&0.14&...&...\\ 
G028.3225$+00.2803$&28.32247&$ +0.28031$&5.6&0.18&0.07&0.37&0.07&...&...\\ 
G028.3331$+00.0848$&28.33310&$ +0.08475$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G028.3346$+00.9267$&28.33461&$ +0.92667$&5.1&0.17&0.07&0.33&0.07&...&...\\ 
G028.3470$+00.9185$&28.34704&$ +0.91847$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G028.3472$+00.1739$&28.34720&$ +0.17392$&6.1&0.24&0.07&0.39&0.07&Psr&...\\ 
G028.3546$+00.9428$&28.35461&$ +0.94278$&5.3&0.17&0.07&0.34&0.07&...&...\\ 
G028.3573$-00.1614$&28.35727&$ -0.16136$&5.2&0.19&0.07&0.36&0.07&...&...\\ 
G028.3707$+00.0809$&28.37074&$ +0.08093$&5.0&0.16&0.06&0.31&0.07&...&...\\ 
G028.3775$+00.5966$&28.37754&$ +0.59657$&5.1&0.23&0.08&0.40&0.08&...&...\\ 
G028.3815$-01.0118$&28.38148&$ -1.01183$&5.2&0.37&0.12&0.60&0.12&...&...\\ 
G028.3828$-00.0996$&28.38275&$ -0.09955$&5.2&0.17&0.07&0.34&0.07&...&...\\ 
G028.3876$-00.7275$&28.38760&$ -0.72749$&6.6&0.19&0.06&0.38&0.06&...&...\\ 
G028.3893$+00.7651$&28.38934&$ +0.76512$&5.1&0.21&0.07&0.33&0.07&...&...\\ 
G028.3961$-00.7985$&28.39608&$ -0.79847$&5.8&0.16&0.06&0.34&0.06&...&...\\ 
G028.4087$-00.1034$&28.40872&$ -0.10337$&7.0&0.28&0.07&0.46&0.07&WR*&...\\ 
G028.4231$+00.0420$&28.42310&$ +0.04204$&5.4&0.23&0.07&0.37&0.07&...&...\\ 
G028.4233$-00.2686$&28.42331&$ -0.26858$&5.0&0.16&0.06&0.29&0.06&...&...\\ 
G028.4262$+00.9767$&28.42621&$ +0.97674$&5.2&0.19&0.08&0.38&0.08&...&...\\ 
G028.4266$-00.3384$&28.42657&$ -0.33844$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G028.4410$-00.4142$&28.44102&$ -0.41421$&5.8&0.21&0.06&0.33&0.06&...&...\\ 
G028.4425$-00.2182$&28.44247&$ -0.21823$&5.1&0.21&0.06&0.31&0.06&...&...\\ 
G028.4430$+00.8092$&28.44296&$ +0.80915$&5.2&0.18&0.06&0.32&0.07&...&...\\ 
G028.4474$-00.1807$&28.44741&$ -0.18066$&5.2&0.18&0.06&0.32&0.06&...&...\\ 
G028.4506$-00.8116$&28.45059&$ -0.81159$&5.2&0.17&0.07&0.34&0.07&...&...\\ 
G028.4519$-00.8802$&28.45191&$ -0.88021$&5.4&0.23&0.07&0.36&0.07&---&G028.452-00.880\\ 
G028.4542$+00.9721$&28.45420&$ +0.97209$&5.4&0.20&0.07&0.38&0.08&...&...\\ 
G028.4591$-00.5183$&28.45914&$ -0.51831$&5.1&0.15&0.06&0.28&0.06&...&...\\ 
G028.4672$+00.6239$&28.46720&$ +0.62386$&5.5&0.23&0.07&0.36&0.07&...&...\\ 
G028.4844$+00.5946$&28.48442&$ +0.59456$&5.3&0.25&0.07&0.39&0.08&...&...\\ 
G028.4847$+00.1939$&28.48470&$ +0.19392$&5.0&0.14&0.06&0.30&0.06&...&...\\ 
G028.4863$-00.2113$&28.48629&$ -0.21129$&6.1&0.17&0.06&0.35&0.06&...&...\\ 
G028.4910$+00.5229$&28.49102&$ +0.52289$&5.2&0.28&0.11&0.55&0.11&...&...\\ 
G028.4936$+00.9115$&28.49359&$ +0.91146$&5.0&0.18&0.06&0.31&0.07&...&...\\ 
G028.4937$+00.7803$&28.49372&$ +0.78033$&5.9&0.22&0.07&0.40&0.07&...&...\\ 
G028.4969$-00.5907$&28.49692&$ -0.59074$&5.1&0.15&0.06&0.29&0.06&...&...\\ 
G028.4987$+00.0741$&28.49866&$ +0.07413$&5.0&0.17&0.07&0.32&0.07&...&...\\ 
G028.5074$-00.5332$&28.50741&$ -0.53317$&5.0&0.16&0.06&0.28&0.06&...&...\\ 
G028.5145$-00.4230$&28.51449&$ -0.42296$&5.1&0.17&0.06&0.29&0.06&...&...\\ 
G028.5153$+00.6580$&28.51532&$ +0.65803$&5.5&0.23&0.07&0.38&0.07&...&...\\ 
G028.5206$+00.4536$&28.52060&$ +0.45365$&5.5&0.37&0.11&0.58&0.11&...&...\\ 
G028.5222$-01.0149$&28.52220&$ -1.01488$&5.2&0.48&0.13&0.67&0.14&...&...\\ 
G028.5223$+00.8205$&28.52234&$ +0.82054$&5.0&0.18&0.07&0.34&0.07&...&...\\ 
G028.5297$+00.2691$&28.52970&$ +0.26906$&5.2&0.18&0.06&0.32&0.07&...&...\\ 
G028.5350$-00.7380$&28.53505&$ -0.73805$&5.3&0.21&0.07&0.35&0.07&...&...\\ 
G028.5398$-00.8117$&28.53984&$ -0.81166$&5.1&0.22&0.07&0.32&0.07&...&...\\ 
G028.5454$-00.1321$&28.54539&$ -0.13212$&5.1&0.21&0.06&0.32&0.07&...&...\\ 
G028.5471$-00.8861$&28.54706&$ -0.88612$&5.0&0.18&0.07&0.36&0.07&...&...\\ 
G028.5564$+00.3375$&28.55643&$ +0.33746$&5.5&0.17&0.06&0.33&0.07&...&...\\ 
G028.5669$-00.3233$&28.56685&$ -0.32330$&5.2&0.17&0.06&0.30&0.06&...&...\\ 
G028.5717$-00.7411$&28.57172&$ -0.74110$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G028.5746$-00.7489$&28.57456&$ -0.74888$&5.1&0.19&0.06&0.31&0.06&...&...\\ 
G028.5798$-00.0537$&28.57984&$ -0.05372$&5.4&0.20&0.07&0.35&0.07&...&...\\ 
G028.5808$-00.9721$&28.58082&$ -0.97210$&5.0&0.20&0.08&0.39&0.08&...&...\\ 
G028.5862$-00.7580$&28.58616&$ -0.75798$&5.0&0.22&0.06&0.32&0.07&...&...\\ 
G028.5869$-00.8857$&28.58693&$ -0.88570$&6.1&0.20&0.07&0.43&0.07&...&...\\ 
G028.5894$-00.7789$&28.58936&$ -0.77888$&5.2&0.21&0.07&0.33&0.07&...&...\\ 
G028.5917$+00.1394$&28.59171&$ +0.13941$&5.6&0.20&0.06&0.33&0.06&...&...\\ 
G028.5978$-00.8099$&28.59783&$ -0.80993$&5.2&0.20&0.06&0.33&0.07&...&...\\ 
G028.6027$-00.3442$&28.60269&$ -0.34421$&5.2&0.17&0.06&0.31&0.06&...&...\\ 
G028.6114$-00.1413$&28.61136&$ -0.14129$&6.1&0.30&0.07&0.40&0.07&...&...\\ 
G028.6142$+00.3297$&28.61421&$ +0.32969$&6.1&0.21&0.06&0.38&0.06&...&...\\ 
G028.6185$+00.4730$&28.61845&$ +0.47302$&5.2&0.21&0.06&0.31&0.06&...&...\\ 
G028.6227$+00.0539$&28.62268&$ +0.05392$&5.0&0.23&0.08&0.37&0.08&...&...\\ 
G028.6243$-00.8256$&28.62429&$ -0.82555$&5.1&0.18&0.07&0.35&0.07&...&...\\ 
G028.6325$-00.3302$&28.63248&$ -0.33018$&5.2&0.18&0.06&0.32&0.06&...&...\\ 
G028.6366$+00.2904$&28.63664&$ +0.29045$&5.1&0.16&0.06&0.30&0.06&...&...\\ 
G028.6391$+00.6261$&28.63908&$ +0.62608$&5.1&0.19&0.07&0.33&0.07&...&...\\ 
G028.6394$-00.0534$&28.63935&$ -0.05344$&5.1&0.19&0.07&0.34&0.07&...&...\\ 
G028.6424$-00.4343$&28.64241&$ -0.43428$&6.6&0.22&0.06&0.39&0.06&...&...\\ 
G028.6438$-00.9108$&28.64381&$ -0.91077$&5.1&0.19&0.07&0.38&0.08&...&...\\ 
G028.6486$-00.9458$&28.64861&$ -0.94585$&5.0&0.19&0.08&0.37&0.08&...&...\\ 
G028.6530$+00.1163$&28.65303&$ +0.11628$&5.4&0.18&0.07&0.34&0.07&...&...\\ 
G028.6604$-00.1278$&28.66039&$ -0.12782$&5.2&0.19&0.06&0.33&0.07&...&...\\ 
G028.6612$-00.6365$&28.66124&$ -0.63651$&6.1&0.23&0.07&0.41&0.07&...&...\\ 
G028.6621$-00.2474$&28.66206&$ -0.24740$&5.1&0.14&0.06&0.30&0.06&...&...\\ 
G028.6689$-00.1118$&28.66886&$ -0.11177$&6.0&0.26&0.07&0.42&0.07&...&...\\ 
G028.6696$-00.0933$&28.66963&$ -0.09330$&5.1&0.22&0.07&0.33&0.07&...&...\\ 
G028.6725$-00.1047$&28.67248&$ -0.10469$&6.0&0.27&0.07&0.42&0.07&...&...\\ 
G028.6810$-00.8945$&28.68104&$ -0.89452$&6.0&0.25&0.08&0.46&0.08&---&G028.681-00.894\\ 
G028.6957$+00.0648$&28.69574&$ +0.06475$&5.2&0.18&0.06&0.33&0.07&...&...\\ 
G028.7069$+00.4410$&28.70686&$ +0.44101$&6.2&0.21&0.06&0.37&0.06&...&...\\ 
G028.7100$-00.0420$&28.71004&$ -0.04198$&5.1&0.17&0.06&0.31&0.06&...&...\\ 
G028.7222$-00.5343$&28.72221&$ -0.53428$&5.2&0.19&0.07&0.33&0.07&...&...\\ 
G028.7283$+00.2205$&28.72831&$ +0.22052$&5.1&0.18&0.06&0.31&0.06&...&...\\ 
G028.7330$+00.8312$&28.73299&$ +0.83117$&5.0&0.17&0.06&0.31&0.06&...&...\\ 
G028.7411$-00.8317$&28.74111&$ -0.83167$&5.8&0.22&0.07&0.40&0.07&...&...\\ 
G028.7426$+01.0181$&28.74258&$ +1.01814$&5.0&0.35&0.12&0.60&0.13&...&...\\ 
G028.7428$-00.5382$&28.74276&$ -0.53817$&6.1&0.21&0.07&0.40&0.07&...&...\\ 
G028.7453$-00.2843$&28.74533&$ -0.28435$&5.0&0.16&0.06&0.30&0.06&...&...\\ 
G028.7462$-00.7977$&28.74618&$ -0.79770$&5.4&0.21&0.06&0.34&0.07&...&...\\ 
G028.7641$-00.1142$&28.76407&$ -0.11421$&5.2&0.17&0.06&0.31&0.06&...&...\\ 
G028.7670$+00.6463$&28.76701&$ +0.64629$&5.6&0.21&0.07&0.38&0.07&...&...\\ 
G028.7681$-00.7001$&28.76812&$ -0.70013$&5.1&0.17&0.06&0.30&0.06&...&...\\ 
G028.7734$+00.6083$&28.77339&$ +0.60831$&6.0&0.24&0.07&0.39&0.07&...&...\\ 
G028.7735$-00.5314$&28.77346&$ -0.53137$&5.4&0.18&0.06&0.33&0.07&...&...\\ 
G028.7738$+00.8687$&28.77376&$ +0.86874$&5.6&0.19&0.06&0.35&0.07&...&...\\ 
G028.7816$+00.6669$&28.78159&$ +0.66685$&5.3&0.19&0.06&0.34&0.07&...&...\\ 
G028.7870$-00.7442$&28.78701&$ -0.74416$&6.3&0.21&0.06&0.39&0.07&...&...\\ 
G028.7916$+00.0902$&28.79164&$ +0.09024$&5.1&0.15&0.06&0.30&0.06&...&...\\ 
G028.7968$+00.1780$&28.79678&$ +0.17802$&5.3&0.26&0.07&0.37&0.07&...&...\\ 
G028.7987$-00.6901$&28.79875&$ -0.69006$&6.1&0.20&0.06&0.36&0.06&...&...\\ 
G028.8028$+00.6412$&28.80284&$ +0.64122$&5.5&0.22&0.07&0.35&0.07&...&...\\ 
G028.8044$+00.4070$&28.80436&$ +0.40705$&5.2&0.15&0.06&0.33&0.07&...&...\\ 
G028.8086$+00.1693$&28.80859&$ +0.16927$&5.6&0.53&0.08&0.40&0.08&...&...\\ 
G028.8103$+00.1728$&28.81033&$ +0.17281$&5.6&0.56&0.08&0.40&0.07&...&...\\ 
G028.8209$+00.0261$&28.82088&$ +0.02607$&5.7&0.18&0.06&0.34&0.06&...&...\\ 
G028.8238$-00.5535$&28.82381&$ -0.55345$&5.0&0.16&0.06&0.30&0.06&...&...\\ 
G028.8304$+00.0602$&28.83039&$ +0.06017$&5.0&0.20&0.06&0.29&0.06&...&...\\ 
G028.8305$+00.1200$&28.83046&$ +0.11996$&5.6&0.21&0.06&0.35&0.07&...&...\\ 
G028.8314$-00.2515$&28.83137&$ -0.25150$&6.0&0.20&0.07&0.40&0.07&Rad&...\\ 
G028.8315$-00.9740$&28.83148&$ -0.97404$&5.5&0.31&0.08&0.43&0.08&...&...\\ 
G028.8318$-00.7640$&28.83181&$ -0.76402$&5.1&0.18&0.06&0.32&0.07&...&...\\ 
G028.8341$+00.0718$&28.83414&$ +0.07177$&5.2&0.17&0.06&0.29&0.06&...&...\\ 
G028.8342$+00.9836$&28.83419&$ +0.98362$&5.1&0.21&0.08&0.38&0.08&...&...\\ 
G028.8381$+00.7348$&28.83813&$ +0.73477$&5.0&0.17&0.07&0.33&0.07&...&...\\ 
G028.8382$-00.0831$&28.83824&$ -0.08309$&5.2&0.18&0.06&0.33&0.07&...&...\\ 
G028.8476$-00.7251$&28.84764&$ -0.72513$&5.3&0.16&0.06&0.31&0.06&...&...\\ 
G028.8493$+00.6507$&28.84931&$ +0.65067$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G028.8539$+00.9952$&28.85392&$ +0.99522$&5.8&0.24&0.08&0.46&0.08&...&...\\ 
G028.8550$-00.1605$&28.85505&$ -0.16046$&5.3&0.20&0.06&0.33&0.07&...&...\\ 
G028.8551$+00.0432$&28.85512&$ +0.04322$&5.2&0.18&0.06&0.31&0.06&...&...\\ 
G028.8562$-00.1474$&28.85623&$ -0.14740$&5.1&0.21&0.07&0.33&0.07&...&...\\ 
G028.8569$-00.7158$&28.85695&$ -0.71582$&5.4&0.17&0.06&0.31&0.06&...&...\\ 
G028.8596$-00.2151$&28.85956&$ -0.21511$&5.4&0.20&0.06&0.35&0.07&...&...\\ 
G028.8612$-00.7539$&28.86119&$ -0.75388$&5.5&0.18&0.06&0.34&0.06&...&...\\ 
G028.8615$-00.6938$&28.86153&$ -0.69381$&5.7&0.18&0.06&0.34&0.06&...&...\\ 
G028.8648$+00.4252$&28.86478&$ +0.42517$&5.2&0.18&0.06&0.32&0.06&...&...\\ 
G028.8678$-00.0033$&28.86782&$ -0.00330$&5.4&0.18&0.06&0.33&0.06&...&...\\ 
G028.8776$+00.8698$&28.87759&$ +0.86979$&5.7&0.23&0.06&0.34&0.06&...&...\\ 
G028.9020$-00.3752$&28.90200&$ -0.37525$&5.0&0.23&0.07&0.33&0.07&...&...\\ 
G028.9059$-00.5985$&28.90590&$ -0.59845$&5.3&0.22&0.07&0.36&0.07&...&...\\ 
G028.9064$+00.5859$&28.90639&$ +0.58587$&5.6&0.22&0.06&0.34&0.06&...&...\\ 
G028.9116$+00.0463$&28.91158&$ +0.04628$&5.0&0.23&0.06&0.31&0.06&...&...\\ 
G028.9190$+00.2027$&28.91901&$ +0.20274$&5.2&0.19&0.06&0.31&0.06&...&...\\ 
G028.9266$-00.9008$&28.92663&$ -0.90077$&6.3&0.21&0.07&0.43&0.07&...&...\\ 
G028.9373$-00.3023$&28.93735&$ -0.30233$&5.2&0.17&0.07&0.35&0.07&...&...\\ 
G028.9402$-00.8999$&28.94017&$ -0.89994$&6.4&0.20&0.07&0.42&0.07&...&...\\ 
G028.9434$-00.4888$&28.94340&$ -0.48879$&5.2&0.19&0.07&0.35&0.07&...&...\\ 
G028.9493$-00.0921$&28.94929&$ -0.09212$&5.4&0.20&0.07&0.37&0.07&...&...\\ 
G028.9510$-00.5755$&28.95097&$ -0.57553$&5.2&0.23&0.07&0.37&0.07&...&...\\ 
G028.9555$+00.5755$&28.95549&$ +0.57553$&5.2&0.20&0.07&0.35&0.07&...&...\\ 
G028.9573$-00.8030$&28.95732&$ -0.80298$&5.0&0.16&0.06&0.32&0.07&...&...\\ 
G028.9654$-00.8274$&28.96538&$ -0.82736$&5.0&0.16&0.07&0.33&0.07&...&...\\ 
G028.9656$+00.1157$&28.96561&$ +0.11573$&6.9&0.26&0.07&0.49&0.08&...&...\\ 
G028.9697$-00.2621$&28.96971&$ -0.26205$&5.2&0.22&0.07&0.37&0.07&...&...\\ 
G028.9710$+00.8735$&28.97101&$ +0.87354$&5.1&0.19&0.07&0.35&0.07&...&...\\ 
G028.9839$-00.4963$&28.98389&$ -0.49629$&5.0&0.24&0.07&0.36&0.08&...&...\\ 
G028.9994$-00.2009$&28.99943&$ -0.20094$&6.6&0.28&0.07&0.45&0.07&...&...\\ 
G029.0216$-00.0896$&29.02164&$ -0.08962$&5.2&0.22&0.07&0.37&0.07&...&...\\ 
G029.0250$-00.8967$&29.02498&$ -0.89667$&5.2&0.19&0.07&0.35&0.07&---&G029.025-00.897\\ 
G029.0334$-00.6892$&29.03341&$ -0.68915$&5.0&0.18&0.07&0.35&0.07&...&...\\ 
G029.0402$-00.2787$&29.04017&$ -0.27872$&5.1&0.19&0.07&0.34&0.07&...&...\\ 
G029.0412$+00.0552$&29.04122&$ +0.05524$&6.0&0.20&0.07&0.42&0.07&...&...\\ 
G029.0437$+00.0241$&29.04372&$ +0.02406$&5.3&0.19&0.07&0.35&0.07&...&...\\ 
G029.0443$-00.2662$&29.04427&$ -0.26622$&5.2&0.19&0.07&0.35&0.07&...&...\\ 
G029.0487$+00.7906$&29.04868&$ +0.79061$&5.9&0.25&0.07&0.38&0.07&---&G029.048+00.791\\ 
G029.0573$-00.3140$&29.05732&$ -0.31400$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G029.0592$-00.6488$&29.05918&$ -0.64880$&5.2&0.21&0.07&0.36&0.07&...&...\\ 
G029.0608$-00.1369$&29.06080&$ -0.13691$&5.2&0.19&0.07&0.35&0.07&...&...\\ 
G029.0647$-00.7279$&29.06466&$ -0.72791$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G029.0823$-00.5035$&29.08232&$ -0.50352$&5.1&0.21&0.07&0.34&0.07&...&...\\ 
G029.0839$+00.3668$&29.08385&$ +0.36684$&6.4&0.30&0.08&0.51&0.09&...&...\\ 
G029.0841$+00.0643$&29.08414&$ +0.06427$&6.0&0.24&0.06&0.38&0.07&...&...\\ 
G029.0898$+00.2284$&29.08983&$ +0.22836$&7.0&0.28&0.08&0.51&0.08&...&...\\ 
G029.0935$-00.5061$&29.09350&$ -0.50609$&5.6&0.23&0.07&0.38&0.07&...&...\\ 
G029.0997$+00.0111$&29.09969&$ +0.01107$&5.3&0.21&0.07&0.37&0.07&...&...\\ 
G029.1152$+00.2461$&29.11525&$ +0.24614$&5.2&0.20&0.07&0.36&0.07&...&...\\ 
G029.1192$+00.1394$&29.11921&$ +0.13941$&5.2&0.19&0.07&0.34&0.07&...&...\\ 
G029.1194$+00.6317$&29.11939&$ +0.63171$&5.5&0.23&0.09&0.48&0.09&...&...\\ 
G029.1255$+00.5151$&29.12551&$ +0.51511$&5.0&0.19&0.08&0.41&0.09&...&...\\ 
G029.1286$-00.8824$&29.12861&$ -0.88243$&5.5&0.19&0.07&0.35&0.07&No*&G029.128-00.882\\ 
G029.1310$-00.4460$&29.13100&$ -0.44602$&5.5&0.29&0.07&0.38&0.07&...&...\\ 
G029.1498$+00.1922$&29.14976&$ +0.19218$&5.1&0.19&0.07&0.35&0.07&...&...\\ 
G029.1523$+00.6498$&29.15231&$ +0.64984$&5.5&0.20&0.07&0.39&0.08&...&...\\ 
G029.1569$-00.4241$&29.15691&$ -0.42407$&5.2&0.25&0.07&0.34&0.07&...&...\\ 
G029.1569$+01.0147$&29.15693&$ +1.01474$&5.1&0.35&0.12&0.59&0.12&...&...\\ 
G029.1636$-00.4619$&29.16357&$ -0.46192$&5.2&0.19&0.07&0.35&0.07&...&...\\ 
G029.1654$+00.6052$&29.16537&$ +0.60518$&5.9&0.36&0.08&0.48&0.09&...&...\\ 
G029.1716$+00.2397$&29.17157&$ +0.23968$&5.8&0.27&0.07&0.41&0.08&...&...\\ 
G029.1724$-00.7784$&29.17237&$ -0.77840$&5.0&0.15&0.06&0.32&0.07&...&...\\ 
G029.1770$+00.6001$&29.17704&$ +0.60011$&5.1&0.16&0.07&0.36&0.07&...&...\\ 
G029.1776$+00.6496$&29.17759&$ +0.64963$&5.0&0.17&0.07&0.33&0.07&...&...\\ 
G029.1806$+00.1588$&29.18060&$ +0.15878$&6.3&0.19&0.06&0.39&0.07&...&...\\ 
G029.1812$+00.9188$&29.18118&$ +0.91882$&5.3&0.20&0.07&0.36&0.07&...&...\\ 
G029.1820$-00.7345$&29.18203&$ -0.73450$&5.5&0.24&0.07&0.37&0.07&...&...\\ 
G029.1843$-00.7675$&29.18432&$ -0.76749$&5.0&0.21&0.06&0.32&0.07&...&...\\ 
G029.1890$-00.3704$&29.18899&$ -0.37039$&5.3&0.16&0.07&0.34&0.07&...&...\\ 
G029.2020$-00.5352$&29.20197&$ -0.53519$&5.0&0.23&0.07&0.35&0.07&...&...\\ 
G029.2086$-01.0197$&29.20861&$ -1.01975$&5.0&0.39&0.14&0.71&0.15&...&...\\ 
G029.2087$-00.2714$&29.20865&$ -0.27136$&5.6&0.24&0.07&0.37&0.07&...&...\\ 
G029.2099$-00.9276$&29.20987&$ -0.92758$&5.1&0.18&0.07&0.35&0.07&...&...\\ 
G029.2115$-01.0009$&29.21146&$ -1.00085$&5.1&0.27&0.10&0.50&0.10&...&...\\ 
G029.2187$+00.2669$&29.21865&$ +0.26691$&6.2&0.23&0.07&0.42&0.07&...&...\\ 
G029.2206$+00.7043$&29.22065&$ +0.70428$&5.1&0.23&0.08&0.38&0.08&...&...\\ 
G029.2254$-00.9893$&29.22542&$ -0.98932$&5.1&0.24&0.09&0.45&0.09&...&...\\ 
G029.2347$-00.5323$&29.23468&$ -0.53234$&5.3&0.21&0.07&0.34&0.07&...&...\\ 
G029.2415$-00.7317$&29.24148&$ -0.73173$&5.1&0.17&0.07&0.32&0.07&...&...\\ 
G029.2434$-00.7185$&29.24336&$ -0.71846$&6.0&0.22&0.06&0.38&0.07&---&G029.243-00.718\\ 
G029.2491$-00.3763$&29.24907&$ -0.37629$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G029.2493$+00.1223$&29.24928&$ +0.12232$&5.2&0.19&0.07&0.34&0.07&...&...\\ 
G029.2532$+00.0930$&29.25317&$ +0.09302$&5.7&0.21&0.07&0.40&0.07&...&...\\ 
G029.2600$-00.3707$&29.25997&$ -0.37074$&5.0&0.17&0.06&0.32&0.07&...&...\\ 
G029.2759$+00.4088$&29.27594&$ +0.40878$&5.1&0.19&0.07&0.37&0.08&...&...\\ 
G029.2807$+00.7394$&29.28072&$ +0.73936$&5.3&0.22&0.07&0.38&0.08&...&...\\ 
G029.2984$-01.0025$&29.29842&$ -1.00252$&5.9&0.35&0.10&0.59&0.11&...&...\\ 
G029.2992$-00.6773$&29.29920&$ -0.67735$&5.1&0.19&0.06&0.32&0.07&...&...\\ 
G029.3017$-00.7612$&29.30169&$ -0.76124$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G029.3247$+00.9374$&29.32474&$ +0.93736$&6.1&0.24&0.07&0.42&0.07&...&...\\ 
G029.3264$+00.1241$&29.32643&$ +0.12406$&5.3&0.19&0.07&0.34&0.07&...&...\\ 
G029.3347$-00.8888$&29.33468&$ -0.88882$&5.0&0.17&0.07&0.33&0.07&...&...\\ 
G029.3538$+01.0018$&29.35377&$ +1.00182$&5.0&0.28&0.09&0.47&0.10&...&...\\ 
G029.3634$+00.1883$&29.36345&$ +0.18829$&5.3&0.16&0.06&0.32&0.06&...&...\\ 
G029.3839$+00.0640$&29.38386&$ +0.06399$&5.1&0.15&0.06&0.30&0.06&...&...\\ 
G029.3962$-00.1580$&29.39616&$ -0.15803$&5.1&0.20&0.07&0.34&0.07&...&...\\ 
G029.3987$-00.8524$&29.39871&$ -0.85243$&6.9&0.25&0.07&0.45&0.07&...&...\\ 
G029.3988$-00.6185$&29.39879&$ -0.61845$&5.7&0.22&0.07&0.36&0.07&...&...\\ 
G029.4105$-00.7619$&29.41052&$ -0.76194$&5.9&0.18&0.06&0.36&0.06&...&...\\ 
G029.4166$+00.9948$&29.41656&$ +0.99480$&5.3&0.26&0.09&0.46&0.09&...&...\\ 
G029.4328$+00.1543$&29.43282&$ +0.15427$&6.7&0.20&0.06&0.40&0.07&...&...\\ 
G029.4330$+00.6088$&29.43303&$ +0.60879$&6.5&0.25&0.07&0.46&0.08&---&G029.433+00.609\\ 
G029.4358$+00.4395$&29.43581&$ +0.43948$&5.2&0.20&0.06&0.32&0.07&...&...\\ 
G029.4367$+00.5760$&29.43671&$ +0.57601$&5.3&0.23&0.07&0.38&0.07&...&...\\ 
G029.4371$-00.6834$&29.43705&$ -0.68339$&5.0&0.17&0.06&0.31&0.06&...&...\\ 
G029.4432$+00.7569$&29.44316&$ +0.75686$&5.2&0.20&0.07&0.34&0.07&...&...\\ 
G029.4453$+00.0678$&29.44532&$ +0.06781$&5.6&0.21&0.06&0.35&0.07&...&...\\ 
G029.4468$-00.9697$&29.44677&$ -0.96974$&5.6&0.20&0.08&0.40&0.08&...&...\\ 
G029.4518$+00.0952$&29.45178&$ +0.09517$&5.3&0.19&0.06&0.32&0.06&...&...\\ 
G029.4528$-00.1608$&29.45275&$ -0.16080$&5.2&0.22&0.06&0.32&0.07&...&...\\ 
G029.4553$-00.5595$&29.45525&$ -0.55949$&5.2&0.19&0.06&0.32&0.07&...&...\\ 
G029.4559$-00.4525$&29.45595&$ -0.45247$&5.0&0.19&0.06&0.31&0.07&...&...\\ 
G029.4655$+00.1707$&29.46553&$ +0.17073$&5.1&0.16&0.06&0.29&0.06&...&...\\ 
G029.4717$-00.6907$&29.47171&$ -0.69075$&5.1&0.18&0.06&0.31&0.07&...&...\\ 
G029.4736$+00.1868$&29.47359&$ +0.18684$&5.0&0.19&0.06&0.31&0.06&...&...\\ 
G029.4875$+00.5067$&29.48747&$ +0.50670$&5.1&0.18&0.07&0.34&0.07&...&...\\ 
G029.4884$+00.2880$&29.48838&$ +0.28802$&5.0&0.19&0.06&0.30&0.06&...&...\\ 
G029.4967$+00.1493$&29.49671&$ +0.14927$&5.2&0.16&0.06&0.31&0.06&...&...\\ 
G029.5032$+00.8265$&29.50317&$ +0.82652$&5.4&0.24&0.08&0.40&0.08&...&...\\ 
G029.5035$+00.8273$&29.50352&$ +0.82728$&6.0&0.29&0.08&0.45&0.08&...&...\\ 
G029.5053$-00.4903$&29.50525&$ -0.49032$&5.0&0.17&0.06&0.31&0.06&...&...\\ 
G029.5069$+00.8231$&29.50692&$ +0.82311$&6.9&0.35&0.08&0.50&0.08&...&...\\ 
G029.5171$+00.1414$&29.51706&$ +0.14142$&5.5&0.21&0.06&0.34&0.07&...&...\\ 
G029.5215$-00.5960$&29.52150&$ -0.59602$&5.2&0.15&0.06&0.32&0.06&...&...\\ 
G029.5302$-00.4766$&29.53018&$ -0.47664$&5.0&0.18&0.07&0.32&0.07&...&...\\ 
G029.5409$-00.9173$&29.54088&$ -0.91730$&5.1&0.19&0.08&0.38&0.08&...&...\\ 
G029.5489$-00.3523$&29.54886&$ -0.35226$&5.6&0.18&0.07&0.37&0.07&...&...\\ 
G029.5509$-00.5221$&29.55088&$ -0.52213$&6.9&0.21&0.07&0.45&0.07&...&...\\ 
G029.5644$+00.7578$&29.56442&$ +0.75776$&5.0&0.21&0.08&0.38&0.08&...&...\\ 
G029.5730$+00.5234$&29.57303&$ +0.52337$&5.3&0.17&0.06&0.32&0.06&...&...\\ 
G029.5841$+00.1145$&29.58414&$ +0.11448$&6.1&0.32&0.06&0.37&0.06&Rad&...\\ 
G029.5844$+00.7326$&29.58436&$ +0.73255$&5.0&0.20&0.07&0.36&0.08&...&...\\ 
G029.6089$-00.8044$&29.60887&$ -0.80444$&6.4&0.30&0.08&0.52&0.09&...&...\\ 
G029.6121$+00.1411$&29.61206&$ +0.14114$&5.5&0.16&0.06&0.33&0.06&...&...\\ 
G029.6132$-00.3211$&29.61324&$ -0.32108$&5.0&0.20&0.07&0.34&0.07&...&...\\ 
G029.6196$-00.8133$&29.61957&$ -0.81326$&6.9&0.29&0.08&0.54&0.08&Y*?&G029.619-00.813\\ 
G029.6216$+00.5025$&29.62165&$ +0.50254$&5.1&0.16&0.06&0.32&0.06&...&...\\ 
G029.6360$-00.9877$&29.63604&$ -0.98766$&5.2&0.31&0.09&0.45&0.09&...&...\\ 
G029.6464$-00.8096$&29.64638&$ -0.80958$&5.4&0.23&0.07&0.39&0.08&...&...\\ 
G029.6484$-00.7465$&29.64839&$ -0.74652$&5.1&0.19&0.07&0.34&0.07&...&...\\ 
G029.6486$-00.5025$&29.64859&$ -0.50248$&5.0&0.18&0.06&0.32&0.07&...&...\\ 
G029.6490$-00.9899$&29.64896&$ -0.98995$&5.3&0.29&0.10&0.49&0.10&...&...\\ 
G029.6546$-00.0383$&29.65456&$ -0.03830$&5.0&0.18&0.07&0.35&0.07&...&...\\ 
G029.6613$-00.7312$&29.66131&$ -0.73117$&5.2&0.21&0.07&0.35&0.07&...&...\\ 
G029.6663$-00.4707$&29.66630&$ -0.47067$&5.0&0.18&0.06&0.31&0.07&...&...\\ 
G029.6847$-00.0550$&29.68470&$ -0.05504$&5.2&0.19&0.07&0.37&0.07&...&...\\ 
G029.6860$+00.0638$&29.68602&$ +0.06378$&5.2&0.18&0.07&0.34&0.07&...&...\\ 
G029.6914$-00.1967$&29.69143&$ -0.19671$&5.8&0.22&0.07&0.39&0.07&...&...\\ 
G029.6947$-00.5325$&29.69471&$ -0.53248$&6.0&0.23&0.07&0.41&0.07&...&...\\ 
G029.7056$-00.9627$&29.70556&$ -0.96265$&5.1&0.26&0.08&0.41&0.08&...&...\\ 
G029.7121$+00.2427$&29.71206&$ +0.24267$&5.2&0.18&0.06&0.33&0.07&...&...\\ 
G029.7135$-00.6257$&29.71353&$ -0.62575$&5.1&0.17&0.07&0.33&0.07&...&...\\ 
G029.7241$+00.2229$&29.72414&$ +0.22295$&5.1&0.16&0.07&0.33&0.07&...&...\\ 
G029.7257$-00.3635$&29.72567&$ -0.36351$&5.8&0.25&0.08&0.45&0.08&...&...\\ 
G029.7257$+00.5944$&29.72568&$ +0.59442$&5.1&0.18&0.06&0.31&0.06&...&...\\ 
G029.7309$+00.9095$&29.73091&$ +0.90951$&5.0&0.22&0.07&0.35&0.07&...&...\\ 
G029.7506$+00.5487$&29.75061&$ +0.54865$&5.1&0.19&0.06&0.31&0.06&...&...\\ 
G029.7621$+00.6512$&29.76208&$ +0.65123$&5.4&0.21&0.06&0.34&0.07&...&...\\ 
G029.7648$+00.1623$&29.76477&$ +0.16232$&5.4&0.20&0.07&0.36&0.07&...&...\\ 
G029.7651$-00.6090$&29.76506&$ -0.60901$&5.4&0.19&0.07&0.36&0.07&...&...\\ 
G029.7747$+01.0003$&29.77474&$ +1.00029$&5.8&0.28&0.09&0.51&0.09&...&...\\ 
G029.7766$-00.8024$&29.77660&$ -0.80243$&5.2&0.24&0.08&0.42&0.08&...&...\\ 
G029.7827$+00.1877$&29.78269&$ +0.18767$&5.0&0.20&0.07&0.35&0.07&...&...\\ 
G029.7861$+00.3153$&29.78609&$ +0.31531$&5.1&0.19&0.07&0.35&0.07&...&...\\ 
G029.7874$-00.5593$&29.78742&$ -0.55928$&5.2&0.17&0.06&0.32&0.07&...&...\\ 
G029.7901$+00.3589$&29.79012&$ +0.35885$&5.1&0.21&0.07&0.34&0.07&...&...\\ 
G029.7987$+00.9114$&29.79869&$ +0.91139$&5.2&0.22&0.07&0.35&0.07&...&...\\ 
G029.8036$+00.4266$&29.80360&$ +0.42663$&6.0&0.30&0.07&0.41&0.07&---&G029.804+00.426\\ 
G029.8356$+00.5173$&29.83562&$ +0.51733$&5.0&0.17&0.07&0.32&0.07&...&...\\ 
G029.8410$+00.0811$&29.84102&$ +0.08114$&6.0&0.23&0.08&0.50&0.09&---&G029.841+00.081\\ 
G029.8413$+00.4545$&29.84131&$ +0.45448$&6.8&0.28&0.07&0.46&0.07&...&...\\ 
G029.8499$-00.8350$&29.84994&$ -0.83500$&5.4&0.29&0.10&0.50&0.10&...&...\\ 
G029.8556$-00.5494$&29.85562&$ -0.54942$&5.1&0.20&0.07&0.33&0.07&...&...\\ 
G029.8575$+00.6212$&29.85750&$ +0.62122$&5.4&0.19&0.07&0.36&0.07&...&...\\ 
G029.8605$+00.3444$&29.86047&$ +0.34441$&6.6&0.29&0.07&0.47&0.08&...&...\\ 
G029.8622$+00.2645$&29.86220&$ +0.26448$&5.2&0.21&0.07&0.34&0.07&...&...\\ 
G029.8784$-00.8270$&29.87835&$ -0.82701$&6.0&0.42&0.14&0.83&0.15&...&...\\ 
G029.8788$-00.5846$&29.87882&$ -0.58463$&5.1&0.17&0.07&0.34&0.07&...&...\\ 
G029.8807$-00.9981$&29.88073&$ -0.99814$&5.0&0.24&0.09&0.45&0.09&...&...\\ 
G029.8899$+00.9688$&29.88989&$ +0.96883$&5.1&0.24&0.08&0.38&0.08&...&...\\ 
G029.9045$+00.4494$&29.90450&$ +0.44941$&5.0&0.17&0.07&0.33&0.07&...&...\\ 
G029.9061$-00.7433$&29.90612&$ -0.74325$&5.2&0.17&0.07&0.35&0.07&...&...\\ 
G029.9067$+00.6667$&29.90667&$ +0.66671$&5.1&0.15&0.07&0.33&0.07&...&...\\ 
G029.9182$-00.2896$&29.91818&$ -0.28955$&5.0&0.18&0.07&0.34&0.07&...&...\\ 
G029.9185$-00.1693$&29.91852&$ -0.16934$&5.2&0.22&0.07&0.37&0.08&...&...\\ 
G029.9336$-00.0516$&29.93359&$ -0.05164$&6.6&1.34&0.28&1.83&0.29&...&...\\ 
G029.9340$-00.0530$&29.93401&$ -0.05296$&6.3&2.98&0.31&1.78&0.29&HII&...\\ 
G029.9376$-00.1854$&29.93755&$ -0.18539$&5.2&0.22&0.07&0.34&0.07&...&...\\ 
G029.9418$-00.5118$&29.94180&$ -0.51178$&5.0&0.18&0.07&0.34&0.07&...&...\\ 
G029.9523$-00.8574$&29.95225&$ -0.85736$&5.0&0.24&0.08&0.41&0.09&...&...\\ 
G029.9553$+00.1279$&29.95526&$ +0.12795$&5.3&0.25&0.08&0.39&0.08&...&...\\ 
G029.9630$-00.2936$&29.96297&$ -0.29358$&5.5&0.22&0.07&0.37&0.07&...&...\\ 
G029.9751$-00.5122$&29.97514&$ -0.51220$&5.1&0.15&0.06&0.32&0.06&...&...\\ 
G029.9787$-00.2602$&29.97874&$ -0.26025$&5.2&0.18&0.06&0.30&0.06&...&...\\ 
G029.9973$-00.0982$&29.99734&$ -0.09816$&5.1&0.53&0.10&0.47&0.10&...&...\\ 
G030.0128$+00.9371$&30.01275&$ +0.93709$&5.4&0.23&0.07&0.36&0.07&...&...\\ 
G030.0179$+00.2606$&30.01788&$ +0.26059$&5.9&0.19&0.06&0.34&0.06&...&...\\ 
G030.0184$-00.0433$&30.01844&$ -0.04330$&5.9&0.46&0.13&0.75&0.14&...&...\\ 
G030.0212$-00.5785$&30.02119&$ -0.57852$&5.9&0.22&0.06&0.34&0.06&...&...\\ 
G030.0225$+00.1084$&30.02247&$ +0.10836$&6.4&0.36&0.08&0.49&0.08&...&...\\ 
G030.0244$-00.5854$&30.02439&$ -0.58540$&5.5&0.15&0.06&0.32&0.06&...&...\\ 
G030.0464$-00.2282$&30.04642&$ -0.22823$&5.9&0.23&0.07&0.38&0.07&...&...\\ 
G030.0465$-00.3729$&30.04649&$ -0.37289$&5.1&0.14&0.06&0.31&0.06&...&...\\ 
G030.0480$-01.0030$&30.04803&$ -1.00301$&5.3&0.21&0.08&0.43&0.08&...&...\\ 
G030.0530$-00.0283$&30.05303&$ -0.02830$&5.2&0.38&0.10&0.52&0.11&...&...\\ 
G030.0531$+00.9023$&30.05311&$ +0.90229$&5.3&0.19&0.06&0.33&0.06&...&...\\ 
G030.0550$-00.4571$&30.05496&$ -0.45706$&6.7&0.22&0.06&0.39&0.06&...&...\\ 
G030.0560$+00.4204$&30.05600&$ +0.42038$&5.7&0.20&0.06&0.35&0.06&...&...\\ 
G030.0574$+00.1664$&30.05740&$ +0.16642$&5.4&0.24&0.07&0.34&0.07&...&...\\ 
G030.0648$-00.2848$&30.06483&$ -0.28476$&5.0&0.17&0.06&0.32&0.07&...&...\\ 
G030.0847$+00.7312$&30.08473&$ +0.73116$&6.3&0.20&0.06&0.37&0.06&...&...\\ 
G030.0940$+00.0633$&30.09400&$ +0.06329$&5.2&0.22&0.07&0.37&0.08&...&...\\ 
G030.0996$+00.1150$&30.09955&$ +0.11496$&5.0&0.20&0.07&0.33&0.07&...&...\\ 
G030.1130$-00.8663$&30.11298&$ -0.86632$&5.2&0.15&0.06&0.29&0.06&...&...\\ 
G030.1156$-00.7644$&30.11556&$ -0.76437$&5.2&0.18&0.06&0.30&0.06&...&...\\ 
G030.1209$+00.1914$&30.12087&$ +0.19142$&5.7&0.20&0.06&0.36&0.07&...&...\\ 
G030.1258$+00.3930$&30.12580&$ +0.39295$&5.3&0.18&0.06&0.32&0.06&...&...\\ 
G030.1288$-00.8023$&30.12882&$ -0.80229$&5.2&0.16&0.06&0.29&0.06&...&...\\ 
G030.1482$+00.0650$&30.14817&$ +0.06503$&5.3&0.18&0.06&0.32&0.06&...&...\\ 
G030.1660$-00.8562$&30.16598&$ -0.85618$&5.7&0.16&0.05&0.30&0.06&...&...\\ 
G030.1808$-00.3223$&30.18080&$ -0.32226$&5.7&0.16&0.06&0.32&0.06&...&...\\ 
G030.1827$+00.5634$&30.18267&$ +0.56337$&5.5&0.19&0.06&0.33&0.06&...&...\\ 
G030.1835$-00.8650$&30.18348&$ -0.86500$&5.2&0.18&0.06&0.30&0.06&...&...\\ 
G030.1839$+00.3143$&30.18393&$ +0.31434$&5.0&0.15&0.06&0.30&0.06&...&...\\ 
G030.1977$-00.8004$&30.19765&$ -0.80041$&5.2&0.15&0.05&0.28&0.06&...&...\\ 
G030.2041$-00.3320$&30.20407&$ -0.33199$&5.1&0.17&0.06&0.28&0.06&...&...\\ 
G030.2108$+00.4287$&30.21080&$ +0.42872$&6.0&0.31&0.07&0.38&0.07&HII&G030.211+00.429\\ 
G030.2112$+00.0293$&30.21122&$ +0.02934$&5.0&0.23&0.10&0.48&0.10&...&...\\ 
G030.2195$-00.6571$&30.21947&$ -0.65707$&5.6&0.15&0.05&0.28&0.05&...&...\\ 
G030.2279$+00.4556$&30.22788&$ +0.45559$&5.0&0.17&0.06&0.30&0.06&...&...\\ 
G030.2284$-00.5346$&30.22843&$ -0.53456$&5.0&0.14&0.06&0.27&0.06&...&...\\ 
G030.2345$+00.8060$&30.23453&$ +0.80596$&5.1&0.15&0.06&0.28&0.06&...&...\\ 
G030.2350$-00.7399$&30.23502&$ -0.73985$&5.5&0.17&0.06&0.32&0.06&...&...\\ 
G030.2357$+00.0682$&30.23567&$ +0.06816$&5.1&0.20&0.07&0.34&0.07&...&...\\ 
G030.2365$-00.3415$&30.23650&$ -0.34150$&5.0&0.14&0.06&0.28&0.06&...&...\\ 
G030.2382$+00.0454$&30.23824&$ +0.04545$&6.0&0.27&0.09&0.51&0.09&...&...\\ 
G030.2468$-00.2881$&30.24685&$ -0.28810$&5.4&0.19&0.07&0.34&0.07&...&...\\ 
G030.2623$+00.3908$&30.26233&$ +0.39080$&5.1&0.17&0.06&0.30&0.06&...&...\\ 
G030.2637$-00.1969$&30.26365&$ -0.19691$&5.4&0.24&0.08&0.42&0.08&...&...\\ 
G030.2666$+00.4691$&30.26656&$ +0.46906$&5.9&0.18&0.06&0.34&0.06&...&...\\ 
G030.2685$+00.9147$&30.26849&$ +0.91472$&5.0&0.15&0.06&0.28&0.06&...&...\\ 
G030.2735$-00.6666$&30.27350&$ -0.66658$&6.7&0.17&0.06&0.37&0.06&...&...\\ 
G030.2854$+00.1299$&30.28539&$ +0.12989$&5.1&0.20&0.07&0.33&0.07&...&...\\ 
G030.2988$+00.2157$&30.29879&$ +0.21573$&5.0&0.16&0.06&0.28&0.06&...&...\\ 
G030.3056$-00.7380$&30.30558&$ -0.73805$&5.1&0.15&0.06&0.29&0.06&...&...\\ 
G030.3062$+00.2052$&30.30615&$ +0.20524$&5.0&0.18&0.06&0.30&0.06&...&...\\ 
G030.3123$-00.0864$&30.31227&$ -0.08636$&5.1&0.17&0.07&0.34&0.07&...&...\\ 
G030.3164$-00.9272$&30.31641&$ -0.92716$&5.0&0.16&0.06&0.29&0.06&...&...\\ 
G030.3174$+00.6491$&30.31739&$ +0.64907$&5.6&0.17&0.06&0.33&0.06&...&...\\ 
G030.3175$+00.8915$&30.31745&$ +0.89146$&5.1&0.17&0.06&0.29&0.06&...&...\\ 
G030.3208$+00.7938$&30.32079&$ +0.79381$&5.5&0.19&0.06&0.34&0.06&...&...\\ 
G030.3305$+00.5165$&30.33045&$ +0.51650$&5.5&0.17&0.06&0.30&0.06&...&...\\ 
G030.3441$+00.6828$&30.34413&$ +0.68276$&5.9&0.18&0.06&0.33&0.06&...&...\\ 
G030.3451$-00.4431$&30.34511&$ -0.44310$&5.1&0.15&0.05&0.26&0.05&...&...\\ 
G030.3452$-00.1903$&30.34518&$ -0.19032$&5.5&0.24&0.07&0.36&0.07&...&...\\ 
G030.3465$+00.0563$&30.34650&$ +0.05635$&5.0&0.15&0.06&0.30&0.06&...&...\\ 
G030.3727$+00.9219$&30.37274&$ +0.92195$&5.6&0.16&0.06&0.30&0.06&...&...\\ 
G030.3822$-00.9371$&30.38218&$ -0.93709$&5.3&0.17&0.05&0.28&0.06&...&...\\ 
G030.3874$-00.3557$&30.38740&$ -0.35567$&5.5&0.18&0.05&0.30&0.06&...&...\\ 
G030.3874$-00.1728$&30.38740&$ -0.17282$&6.1&0.22&0.06&0.38&0.07&...&...\\ 
G030.3889$+00.8424$&30.38885&$ +0.84235$&5.0&0.14&0.06&0.29&0.06&...&...\\ 
G030.3935$-00.7719$&30.39351&$ -0.77194$&5.5&0.14&0.05&0.29&0.05&...&...\\ 
G030.3943$+00.3270$&30.39428&$ +0.32698$&5.1&0.20&0.06&0.30&0.06&...&...\\ 
G030.3957$-00.3550$&30.39574&$ -0.35504$&5.0&0.17&0.05&0.26&0.06&...&...\\ 
G030.4049$-00.2849$&30.40490&$ -0.28490$&5.8&0.17&0.06&0.33&0.06&...&...\\ 
G030.4096$+00.0464$&30.40956&$ +0.04642$&5.1&0.19&0.06&0.31&0.06&...&...\\ 
G030.4106$+00.2215$&30.41060&$ +0.22149$&5.2&0.13&0.06&0.28&0.06&...&...\\ 
G030.4158$+00.6328$&30.41580&$ +0.63282$&5.5&0.16&0.05&0.29&0.06&...&...\\ 
G030.4233$+00.8258$&30.42330&$ +0.82575$&5.4&0.18&0.06&0.33&0.07&...&...\\ 
G030.4243$-00.6965$&30.42434&$ -0.69651$&5.0&0.14&0.05&0.26&0.06&...&...\\ 
G030.4352$-00.4501$&30.43518&$ -0.45011$&5.1&0.16&0.06&0.28&0.06&...&...\\ 
G030.4410$-00.0362$&30.44102&$ -0.03622$&5.0&0.22&0.07&0.35&0.07&...&...\\ 
G030.4447$+00.4980$&30.44469&$ +0.49795$&6.8&0.20&0.06&0.39&0.06&...&...\\ 
G030.4463$-00.2527$&30.44629&$ -0.25268$&5.1&0.15&0.06&0.28&0.06&...&...\\ 
G030.4517$-00.9288$&30.45170&$ -0.92876$&5.8&0.15&0.06&0.33&0.06&---&G030.452-00.929\\ 
G030.4538$-00.9631$&30.45379&$ -0.96314$&5.1&0.18&0.06&0.31&0.06&...&...\\ 
G030.4546$+00.2243$&30.45456&$ +0.22434$&5.5&0.13&0.06&0.30&0.06&...&...\\ 
G030.4619$+00.5914$&30.46192&$ +0.59136$&5.1&0.16&0.06&0.28&0.06&...&...\\ 
G030.4633$-00.3582$&30.46331&$ -0.35824$&5.5&0.15&0.06&0.31&0.06&...&...\\ 
G030.4757$+00.0848$&30.47574&$ +0.08482$&5.3&0.21&0.07&0.34&0.07&...&...\\ 
G030.4773$-00.0887$&30.47734&$ -0.08872$&5.5&0.21&0.07&0.36&0.07&...&...\\ 
G030.4802$+00.9873$&30.48025&$ +0.98730$&5.1&0.19&0.07&0.36&0.07&...&...\\ 
G030.4864$+00.7081$&30.48636&$ +0.70810$&5.2&0.17&0.06&0.30&0.06&...&...\\ 
G030.4866$-00.9822$&30.48664&$ -0.98217$&5.5&0.20&0.07&0.38&0.07&...&...\\ 
G030.5015$+00.5986$&30.50150&$ +0.59858$&5.9&0.16&0.05&0.32&0.06&...&...\\ 
G030.5034$+00.0575$&30.50345&$ +0.05746$&5.5&0.24&0.08&0.46&0.09&...&...\\ 
G030.5043$-00.3951$&30.50428&$ -0.39511$&6.4&0.22&0.06&0.35&0.06&...&...\\ 
G030.5191$-00.8081$&30.51914&$ -0.80805$&5.2&0.15&0.06&0.30&0.06&...&...\\ 
G030.5239$+00.0900$&30.52393&$ +0.09003$&5.3&0.28&0.07&0.38&0.08&...&...\\ 
G030.5257$+00.1213$&30.52567&$ +0.12128$&5.1&0.19&0.07&0.33&0.07&...&...\\ 
G030.5301$+00.1316$&30.53011&$ +0.13163$&5.1&0.27&0.07&0.34&0.07&Rad&G030.530+00.131\\ 
G030.5325$-00.1015$&30.53254&$ -0.10150$&5.0&0.17&0.06&0.32&0.07&...&...\\ 
G030.5356$-00.2341$&30.53560&$ -0.23414$&6.3&0.21&0.06&0.37&0.06&...&...\\ 
G030.5362$+00.0204$&30.53616&$ +0.02038$&5.7&3.89&0.30&1.46&0.24&...&...\\ 
G030.5374$-00.6735$&30.53741&$ -0.67353$&5.0&0.15&0.06&0.27&0.06&...&...\\ 
G030.5383$-00.4455$&30.53831&$ -0.44546$&5.3&0.14&0.06&0.30&0.06&...&...\\ 
G030.5487$-01.0157$&30.54873&$ -1.01572$&7.0&0.44&0.12&0.80&0.12&...&...\\ 
G030.5501$+00.1114$&30.55011&$ +0.11142$&6.6&0.24&0.07&0.45&0.07&...&...\\ 
G030.5524$+00.8413$&30.55241&$ +0.84131$&5.3&0.14&0.05&0.27&0.05&...&...\\ 
G030.5532$-00.8294$&30.55324&$ -0.82944$&5.4&0.17&0.06&0.31&0.06&...&...\\ 
G030.5548$-00.3499$&30.55484&$ -0.34990$&5.1&0.17&0.06&0.28&0.06&...&...\\ 
G030.5570$+00.6439$&30.55699&$ +0.64393$&5.2&0.16&0.05&0.27&0.06&...&...\\ 
G030.5580$+00.9399$&30.55804&$ +0.93986$&5.4&0.18&0.06&0.32&0.06&...&...\\ 
G030.5634$+00.1993$&30.56345&$ +0.19934$&6.7&0.23&0.06&0.40&0.06&...&...\\ 
G030.5690$-00.0595$&30.56900&$ -0.05948$&5.0&0.20&0.08&0.40&0.08&...&...\\ 
G030.5769$-00.1055$&30.57692&$ -0.10552$&5.1&0.21&0.08&0.40&0.08&...&...\\ 
G030.5774$-00.9385$&30.57742&$ -0.93848$&5.0&0.15&0.07&0.33&0.07&...&...\\ 
G030.5821$+00.9089$&30.58207&$ +0.90889$&5.5&0.16&0.06&0.30&0.06&...&...\\ 
G030.5832$+00.8143$&30.58318&$ +0.81429$&5.5&0.17&0.05&0.30&0.06&...&...\\ 
G030.5994$-00.3396$&30.59942&$ -0.33955$&5.3&0.15&0.06&0.31&0.06&...&...\\ 
G030.6021$-00.9076$&30.60214&$ -0.90765$&5.7&0.21&0.07&0.36&0.07&...&...\\ 
G030.6028$+00.0243$&30.60282&$ +0.02434$&6.5&0.28&0.09&0.60&0.10&...&...\\ 
G030.6060$+00.8801$&30.60596&$ +0.88007$&5.4&0.17&0.06&0.31&0.06&...&...\\ 
G030.6090$-00.4303$&30.60901&$ -0.43032$&5.0&0.18&0.06&0.29&0.06&...&...\\ 
G030.6094$-00.2498$&30.60935&$ -0.24983$&5.0&0.14&0.06&0.30&0.06&...&...\\ 
G030.6209$+00.0155$&30.62088&$ +0.01552$&5.2&0.29&0.09&0.46&0.09&...&...\\ 
G030.6287$-00.8533$&30.62874&$ -0.85326$&5.0&0.17&0.06&0.30&0.06&...&...\\ 
G030.6419$+00.4500$&30.64192&$ +0.44997$&5.1&0.13&0.05&0.27&0.06&...&...\\ 
G030.6542$-00.7533$&30.65416&$ -0.75326$&5.4&0.15&0.06&0.31&0.06&...&...\\ 
G030.6668$-00.8531$&30.66680&$ -0.85313$&5.1&0.17&0.07&0.33&0.07&...&...\\ 
G030.6669$+00.0219$&30.66685&$ +0.02191$&5.8&0.36&0.10&0.58&0.11&...&...\\ 
G030.6700$+00.6987$&30.66999&$ +0.69873$&5.1&0.16&0.05&0.27&0.06&...&...\\ 
G030.6734$+00.7292$&30.67339&$ +0.72922$&5.0&0.13&0.05&0.27&0.06&...&...\\ 
G030.6818$-00.8446$&30.68180&$ -0.84458$&6.1&0.21&0.06&0.37&0.07&...&...\\ 
G030.6837$-00.2575$&30.68373&$ -0.25747$&6.4&0.26&0.07&0.44&0.07&...&...\\ 
G030.6845$-00.2593$&30.68449&$ -0.25935$&6.2&0.24&0.07&0.41&0.07&...&...\\ 
G030.6867$-00.0728$&30.68671&$ -0.07282$&5.4&0.70&0.24&1.31&0.25&smm&...\\ 
G030.6868$+00.9447$&30.68681&$ +0.94473$&5.0&0.14&0.06&0.30&0.06&...&...\\ 
G030.6877$-00.2608$&30.68769&$ -0.26080$&5.8&0.50&0.07&0.40&0.07&smm&G030.685-00.259(I)\\ 
G030.6891$-00.2536$&30.68914&$ -0.25358$&5.2&0.24&0.07&0.35&0.07&...&...\\ 
G030.7009$+00.9438$&30.70091&$ +0.94375$&5.2&0.15&0.06&0.32&0.06&...&...\\ 
G030.7053$-00.1675$&30.70532&$ -0.16754$&5.0&0.24&0.07&0.35&0.07&...&...\\ 
G030.7057$-00.3898$&30.70567&$ -0.38983$&6.4&0.21&0.06&0.40&0.07&...&...\\ 
G030.7140$+00.4437$&30.71401&$ +0.44372$&5.1&0.15&0.06&0.29&0.06&...&...\\ 
G030.7356$+00.9563$&30.73556&$ +0.95632$&5.6&0.20&0.06&0.35&0.07&...&...\\ 
G030.7409$-00.5386$&30.74089&$ -0.53859$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G030.7413$+00.9465$&30.74133&$ +0.94653$&5.0&0.15&0.06&0.29&0.06&...&...\\ 
G030.7442$+01.0066$&30.74418&$ +1.00661$&5.1&0.34&0.12&0.58&0.12&...&...\\ 
G030.7487$-00.2418$&30.74866&$ -0.24178$&6.8&0.22&0.06&0.39&0.06&...&...\\ 
G030.7487$-00.6123$&30.74874&$ -0.61227$&5.8&0.21&0.07&0.39&0.07&...&...\\ 
G030.7508$-00.0047$&30.75081&$ -0.00469$&6.1&1.00&0.21&1.21&0.21&...&...\\ 
G030.7519$-00.0013$&30.75185&$ -0.00129$&5.5&0.75&0.21&1.12&0.22&...&...\\ 
G030.7542$-00.0463$&30.75421&$ -0.04629$&6.1&1.14&0.32&1.88&0.33&...&...\\ 
G030.7560$-00.6262$&30.75596&$ -0.62623$&5.1&0.16&0.07&0.33&0.07&...&...\\ 
G030.7570$-00.8103$&30.75702&$ -0.81034$&5.2&0.21&0.07&0.35&0.07&...&...\\ 
G030.7610$-00.0480$&30.76102&$ -0.04802$&5.9&1.15&0.30&1.75&0.31&...&...\\ 
G030.7641$+00.4498$&30.76408&$ +0.44976$&5.0&0.16&0.06&0.29&0.06&...&...\\ 
G030.7658$+00.0753$&30.76581&$ +0.07531$&5.0&0.25&0.08&0.39&0.08&...&...\\ 
G030.7664$-00.0323$&30.76636&$ -0.03226$&5.6&0.96&0.25&1.37&0.26&Cl*&G030.783-00.027(I)\\ 
G030.7669$-00.0346$&30.76692&$ -0.03455$&6.6&1.09&0.25&1.61&0.26&*&G030.783-00.027(I)\\ 
G030.7671$-00.0436$&30.76713&$ -0.04358$&6.1&1.10&0.26&1.55&0.27&Rad&G030.783-00.027(I)\\ 
G030.7682$-00.0441$&30.76824&$ -0.04414$&5.5&0.93&0.26&1.39&0.27&...&...\\ 
G030.7683$-00.0432$&30.76831&$ -0.04316$&5.2&0.84&0.26&1.30&0.26&...&...\\ 
G030.7785$+00.7400$&30.77847&$ +0.73998$&5.6&0.17&0.06&0.33&0.06&...&...\\ 
G030.7807$+00.1893$&30.78074&$ +0.18934$&5.3&0.23&0.09&0.45&0.09&...&...\\ 
G030.7812$-00.0258$&30.78123&$ -0.02580$&6.3&1.37&0.33&1.98&0.34&...&...\\ 
G030.7814$+00.2017$&30.78144&$ +0.20170$&5.2&0.18&0.08&0.40&0.08&...&...\\ 
G030.7835$-00.0288$&30.78352&$ -0.02879$&5.8&2.77&0.35&1.89&0.34&Rad&G030.783-00.027(I)\\ 
G030.7837$-00.0281$&30.78373&$ -0.02809$&5.1&1.16&0.33&1.62&0.33&smm&G030.783-00.027(I)\\ 
G030.7850$-00.0298$&30.78505&$ -0.02976$&5.3&1.07&0.33&1.69&0.34&Rad&G030.783-00.027(I)\\ 
G030.7854$-00.0322$&30.78539&$ -0.03219$&5.6&1.94&0.33&1.77&0.33&...&...\\ 
G030.7858$-00.0313$&30.78581&$ -0.03129$&6.3&1.68&0.33&2.00&0.34&...&...\\ 
G030.7870$-00.0165$&30.78699&$ -0.01650$&5.2&0.83&0.24&1.23&0.25&Rad&G030.783-00.027(I)\\ 
G030.7874$-00.9727$&30.78745&$ -0.97266$&6.1&0.27&0.08&0.49&0.08&...&...\\ 
G030.7944$-00.9242$&30.79439&$ -0.92425$&5.4&0.20&0.07&0.39&0.08&...&...\\ 
G030.8146$+00.1613$&30.81463&$ +0.16128$&5.2&0.23&0.09&0.46&0.09&...&...\\ 
G030.8157$-00.3280$&30.81575&$ -0.32803$&5.9&0.17&0.06&0.36&0.07&...&...\\ 
G030.8234$+00.0671$&30.82345&$ +0.06711$&6.2&0.24&0.08&0.50&0.09&...&...\\ 
G030.8242$+00.0672$&30.82421&$ +0.06718$&5.3&0.28&0.09&0.45&0.09&...&...\\ 
G030.8276$+00.3689$&30.82762&$ +0.36892$&5.1&0.19&0.06&0.32&0.07&...&...\\ 
G030.8305$+00.2832$&30.83054&$ +0.28316$&6.5&0.18&0.06&0.39&0.07&...&...\\ 
G030.8313$+00.7041$&30.83125&$ +0.70415$&5.4&0.13&0.06&0.31&0.06&...&...\\ 
G030.8319$+00.0668$&30.83192&$ +0.06677$&5.2&0.29&0.09&0.44&0.09&...&...\\ 
G030.8393$+00.8953$&30.83932&$ +0.89534$&6.9&0.22&0.06&0.42&0.07&...&...\\ 
G030.8398$+00.3212$&30.83977&$ +0.32121$&5.0&0.20&0.07&0.33&0.07&...&...\\ 
G030.8449$+00.4840$&30.84492&$ +0.48399$&5.1&0.17&0.06&0.29&0.06&...&...\\ 
G030.8495$-00.1155$&30.84949&$ -0.11553$&5.0&0.21&0.07&0.36&0.07&...&...\\ 
G030.8562$+00.0082$&30.85623&$ +0.00822$&5.3&0.22&0.08&0.39&0.08&...&...\\ 
G030.8589$+00.6633$&30.85889&$ +0.66331$&5.1&0.13&0.06&0.28&0.06&...&...\\ 
G030.8665$-00.5714$&30.86645&$ -0.57144$&5.2&0.20&0.07&0.34&0.07&...&...\\ 
G030.8803$-00.3157$&30.88033&$ -0.31567$&5.2&0.16&0.06&0.32&0.07&...&...\\ 
G030.8855$-00.3932$&30.88547&$ -0.39317$&5.0&0.16&0.06&0.30&0.06&...&...\\ 
G030.8905$+00.3848$&30.89047&$ +0.38476$&5.2&0.22&0.07&0.34&0.07&...&...\\ 
G030.9034$+00.9330$&30.90343&$ +0.93299$&5.0&0.16&0.06&0.29&0.06&...&...\\ 
G030.9037$-00.4996$&30.90374&$ -0.49963$&5.2&0.15&0.06&0.33&0.07&...&...\\ 
G030.9043$-00.6901$&30.90431&$ -0.69006$&6.3&0.23&0.07&0.43&0.07&...&...\\ 
G030.9088$+00.8962$&30.90885&$ +0.89618$&6.7&0.21&0.06&0.41&0.06&...&...\\ 
G030.9145$+00.8948$&30.91454&$ +0.89479$&5.3&0.18&0.06&0.32&0.06&...&...\\ 
G030.9157$+00.9234$&30.91573&$ +0.92340$&5.1&0.18&0.06&0.32&0.06&...&...\\ 
G030.9221$-00.3275$&30.92207&$ -0.32754$&5.2&0.19&0.07&0.33&0.07&...&...\\ 
G030.9271$+00.0138$&30.92713&$ +0.01378$&6.1&0.25&0.06&0.38&0.07&...&...\\ 
G030.9278$-00.4038$&30.92784&$ -0.40379$&5.3&0.22&0.06&0.32&0.07&...&...\\ 
G030.9294$-00.4741$&30.92937&$ -0.47407$&5.3&0.18&0.07&0.34&0.07&...&...\\ 
G030.9318$-00.5138$&30.93180&$ -0.51380$&5.0&0.16&0.06&0.31&0.07&...&...\\ 
G030.9320$-00.1249$&30.93199&$ -0.12490$&5.2&0.17&0.06&0.33&0.07&...&...\\ 
G030.9497$+00.9162$&30.94969&$ +0.91618$&5.1&0.17&0.07&0.34&0.07&...&...\\ 
G030.9517$-00.6939$&30.95175&$ -0.69388$&5.1&0.15&0.06&0.31&0.06&...&...\\ 
G030.9541$+00.1134$&30.95408&$ +0.11343$&5.4&0.21&0.07&0.39&0.08&...&...\\ 
G030.9576$+00.0858$&30.95762&$ +0.08579$&5.6&0.61&0.08&0.44&0.08&...&...\\ 
G030.9578$-00.9761$&30.95782&$ -0.97606$&5.5&0.24&0.08&0.43&0.08&...&...\\ 
G030.9606$+00.3668$&30.96061&$ +0.36677$&5.1&0.18&0.07&0.33&0.07&...&...\\ 
G030.9612$-00.1534$&30.96123&$ -0.15344$&5.1&0.17&0.07&0.33&0.07&...&...\\ 
G030.9678$-00.0468$&30.96776&$ -0.04684$&5.2&0.15&0.06&0.32&0.07&...&...\\ 
G030.9710$-00.2295$&30.97103&$ -0.22948$&5.2&0.24&0.06&0.32&0.07&...&...\\ 
G030.9805$+00.5002$&30.98049&$ +0.50025$&5.8&0.19&0.07&0.38&0.07&...&...\\ 
G030.9913$-00.6746$&30.99133&$ -0.67457$&6.3&0.20&0.07&0.41&0.07&...&...\\ 
G030.9966$-00.2991$&30.99656&$ -0.29914$&5.1&0.29&0.07&0.38&0.08&Rad&G030.996-00.299(I)\\ 
G031.0029$+00.9122$&31.00289&$ +0.91222$&5.6&0.22&0.07&0.36&0.07&...&...\\ 
G031.0133$+00.3748$&31.01329&$ +0.37483$&5.0&0.16&0.07&0.32&0.07&Y*?&...\\ 
G031.0142$+00.6269$&31.01418&$ +0.62692$&6.5&0.22&0.07&0.42&0.07&...&...\\ 
G031.0209$-00.4364$&31.02086&$ -0.43636$&5.3&0.16&0.06&0.32&0.06&...&...\\ 
G031.0306$+00.9066$&31.03061&$ +0.90660$&5.0&0.16&0.06&0.31&0.07&...&...\\ 
G031.0387$+00.9269$&31.03866&$ +0.92695$&5.5&0.17&0.06&0.35&0.07&...&...\\ 
G031.0397$+00.8989$&31.03970&$ +0.89889$&5.0&0.21&0.06&0.30&0.06&...&...\\ 
G031.0497$-00.1121$&31.04969&$ -0.11212$&6.7&0.25&0.07&0.46&0.07&...&...\\ 
G031.0542$+00.7483$&31.05417&$ +0.74832$&6.2&0.19&0.06&0.36&0.06&...&...\\ 
G031.0551$+00.5930$&31.05509&$ +0.59296$&5.2&0.16&0.07&0.34&0.07&...&...\\ 
G031.0555$+00.9635$&31.05553&$ +0.96348$&5.7&0.21&0.07&0.39&0.07&...&...\\ 
G031.0565$-00.7753$&31.05646&$ -0.77527$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G031.0629$-00.6760$&31.06293&$ -0.67603$&5.0&0.17&0.06&0.31&0.06&...&...\\ 
G031.0715$+00.3956$&31.07149&$ +0.39559$&5.1&0.16&0.07&0.33&0.07&...&...\\ 
G031.0730$+00.6289$&31.07300&$ +0.62893$&5.2&0.19&0.07&0.35&0.07&...&...\\ 
G031.0756$-00.6407$&31.07557&$ -0.64075$&5.0&0.16&0.06&0.31&0.07&...&...\\ 
G031.0759$-00.2616$&31.07587&$ -0.26164$&5.1&0.16&0.06&0.32&0.06&...&...\\ 
G031.0935$-00.0106$&31.09351&$ -0.01059$&6.5&0.22&0.07&0.41&0.07&...&...\\ 
G031.0954$-00.2982$&31.09538&$ -0.29817$&5.0&0.16&0.06&0.29&0.06&...&...\\ 
G031.1003$-00.8786$&31.10034&$ -0.87862$&5.3&0.16&0.06&0.32&0.06&...&...\\ 
G031.1030$+00.5992$&31.10301&$ +0.59921$&5.2&0.20&0.07&0.35&0.07&...&...\\ 
G031.1064$+00.8644$&31.10639&$ +0.86444$&5.3&0.18&0.06&0.31&0.06&...&...\\ 
G031.1140$-00.6749$&31.11397&$ -0.67492$&5.3&0.18&0.06&0.31&0.06&...&...\\ 
G031.1193$-00.3350$&31.11934&$ -0.33497$&5.2&0.14&0.06&0.31&0.06&...&...\\ 
G031.1205$+00.2724$&31.12045&$ +0.27239$&5.3&0.17&0.06&0.31&0.06&...&...\\ 
G031.1341$+00.5016$&31.13413&$ +0.50156$&5.3&0.18&0.07&0.35&0.07&...&...\\ 
G031.1486$+00.8992$&31.14861&$ +0.89917$&5.8&0.18&0.06&0.35&0.06&---&G031.148+00.899\\ 
G031.1489$+00.1444$&31.14886&$ +0.14441$&5.4&0.20&0.06&0.35&0.07&...&...\\ 
G031.1507$-00.5475$&31.15072&$ -0.54755$&5.3&0.19&0.06&0.32&0.06&...&...\\ 
G031.1597$-00.5509$&31.15968&$ -0.55088$&5.2&0.19&0.07&0.34&0.07&...&...\\ 
G031.1614$+00.3970$&31.16142&$ +0.39698$&5.1&0.17&0.06&0.29&0.06&...&...\\ 
G031.1652$-00.9033$&31.16521&$ -0.90334$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G031.1662$-00.2747$&31.16622&$ -0.27469$&5.0&0.16&0.06&0.31&0.07&...&...\\ 
G031.1725$+00.5346$&31.17246&$ +0.53462$&5.0&0.20&0.07&0.33&0.07&...&...\\ 
G031.1907$-00.6099$&31.19065&$ -0.60991$&6.9&0.24&0.06&0.43&0.07&...&...\\ 
G031.1943$-00.7261$&31.19432&$ -0.72610$&5.1&0.18&0.06&0.31&0.06&...&...\\ 
G031.2061$-00.8130$&31.20606&$ -0.81298$&6.1&0.18&0.06&0.37&0.06&...&...\\ 
G031.2258$-00.9274$&31.22584&$ -0.92744$&5.3&0.19&0.07&0.35&0.07&...&...\\ 
G031.2304$-00.6035$&31.23038&$ -0.60345$&5.2&0.16&0.06&0.32&0.07&...&...\\ 
G031.2343$+00.8443$&31.23425&$ +0.84430$&5.3&0.19&0.06&0.31&0.06&...&...\\ 
G031.2368$+00.4826$&31.23684&$ +0.48261$&5.2&0.16&0.06&0.31&0.06&...&...\\ 
G031.2377$+00.8399$&31.23765&$ +0.83992$&5.2&0.19&0.06&0.31&0.06&...&...\\ 
G031.2421$-00.1116$&31.24206&$ -0.11164$&6.6&0.87&0.24&1.54&0.26&MoC&G031.243-00.110(F)\\ 
G031.2447$-00.1134$&31.24470&$ -0.11344$&6.3&1.06&0.23&1.43&0.24&HII&G031.243-00.110(F)\\ 
G031.2456$-00.1107$&31.24560&$ -0.11066$&5.1&0.91&0.24&1.20&0.25&cor&G031.243-00.110(F)\\ 
G031.2503$-00.6185$&31.25031&$ -0.61845$&5.2&0.18&0.06&0.29&0.06&...&...\\ 
G031.2556$+00.7751$&31.25558&$ +0.77512$&5.0&0.16&0.06&0.29&0.06&...&...\\ 
G031.2608$+00.2962$&31.26080&$ +0.29621$&6.6&0.19&0.06&0.39&0.06&...&...\\ 
G031.2673$+00.9274$&31.26730&$ +0.92743$&5.7&0.18&0.06&0.35&0.06&...&...\\ 
G031.2699$+00.3181$&31.26990&$ +0.31809$&5.1&0.16&0.06&0.30&0.06&...&...\\ 
G031.2702$-00.3840$&31.27018&$ -0.38400$&5.5&0.24&0.09&0.46&0.09&...&...\\ 
G031.2702$-00.5762$&31.27024&$ -0.57616$&5.4&0.19&0.06&0.33&0.06&...&...\\ 
G031.2717$+00.9849$&31.27168&$ +0.98494$&5.3&0.18&0.07&0.37&0.07&...&...\\ 
G031.2739$+00.6573$&31.27392&$ +0.65727$&6.5&0.25&0.07&0.46&0.08&---&G031.274+00.658\\ 
G031.2783$+01.0061$&31.27827&$ +1.00612$&5.1&0.24&0.09&0.43&0.09&...&...\\ 
G031.3032$+00.3827$&31.30316&$ +0.38274$&5.1&0.16&0.06&0.30&0.06&...&...\\ 
G031.3044$-00.6605$&31.30441&$ -0.66054$&5.7&0.22&0.06&0.33&0.06&...&...\\ 
G031.3070$+00.7245$&31.30704&$ +0.72449$&5.9&0.22&0.06&0.35&0.06&...&...\\ 
G031.3079$-00.1622$&31.30789&$ -0.16219$&5.2&0.22&0.07&0.36&0.07&...&...\\ 
G031.3120$+00.2653$&31.31199&$ +0.26531$&5.4&0.17&0.07&0.34&0.07&...&...\\ 
G031.3195$-00.2157$&31.31949&$ -0.21573$&5.3&0.17&0.07&0.35&0.07&...&...\\ 
G031.3315$+00.1815$&31.33150&$ +0.18149$&6.5&0.21&0.06&0.40&0.07&...&...\\ 
G031.3459$+00.3018$&31.34588&$ +0.30177$&5.1&0.18&0.07&0.37&0.08&...&...\\ 
G031.3505$+00.4086$&31.35053&$ +0.40865$&5.0&0.16&0.06&0.31&0.07&...&...\\ 
G031.3574$-00.0630$&31.35741&$ -0.06296$&5.1&0.18&0.07&0.33&0.07&...&...\\ 
G031.3786$-00.9474$&31.37857&$ -0.94744$&5.8&0.23&0.06&0.36&0.07&...&...\\ 
G031.3804$+00.2285$&31.38039&$ +0.22850$&5.2&0.18&0.07&0.36&0.07&...&...\\ 
G031.3811$+00.7373$&31.38108&$ +0.73734$&5.4&0.17&0.07&0.35&0.07&...&...\\ 
G031.3895$-00.3831$&31.38949&$ -0.38310$&6.0&0.78&0.16&0.94&0.16&Rad&G031.388-00.383(I)\\ 
G031.3900$-00.0990$&31.38997&$ -0.09900$&5.8&0.20&0.07&0.38&0.07&...&...\\ 
G031.3976$+00.3983$&31.39761&$ +0.39830$&5.2&0.17&0.07&0.33&0.07&...&...\\ 
G031.3986$+00.7381$&31.39865&$ +0.73811$&6.0&0.23&0.07&0.43&0.07&...&...\\ 
G031.3997$+00.2406$&31.39970&$ +0.24059$&5.1&0.18&0.08&0.39&0.08&...&...\\ 
G031.4014$+00.9133$&31.40142&$ +0.91333$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G031.4067$+00.5458$&31.40671&$ +0.54580$&5.1&0.15&0.06&0.28&0.06&...&...\\ 
G031.4136$-00.6280$&31.41358&$ -0.62797$&5.2&0.20&0.07&0.35&0.07&...&...\\ 
G031.4172$+00.5794$&31.41719&$ +0.57942$&5.1&0.17&0.06&0.29&0.06&...&...\\ 
G031.4232$+00.4117$&31.42324&$ +0.41170$&5.0&0.15&0.06&0.31&0.07&...&...\\ 
G031.4297$-00.1981$&31.42970&$ -0.19809$&5.5&0.19&0.07&0.36&0.07&...&...\\ 
G031.4335$-00.1434$&31.43352&$ -0.14337$&5.2&0.14&0.06&0.31&0.06&...&...\\ 
G031.4379$+00.7812$&31.43789&$ +0.78124$&5.1&0.14&0.06&0.31&0.06&...&...\\ 
G031.4389$+00.6050$&31.43886&$ +0.60504$&6.4&0.23&0.06&0.39&0.07&---&G031.439+00.605\\ 
G031.4399$-00.8635$&31.43990&$ -0.86354$&5.2&0.17&0.07&0.37&0.07&...&...\\ 
G031.4425$+00.6825$&31.44247&$ +0.68255$&6.2&0.21&0.06&0.39&0.07&...&...\\ 
G031.4611$-00.1380$&31.46109&$ -0.13803$&5.1&0.15&0.06&0.29&0.06&...&...\\ 
G031.4672$+00.9556$&31.46719&$ +0.95556$&5.3&0.17&0.06&0.32&0.06&...&...\\ 
G031.4692$-00.3598$&31.46921&$ -0.35983$&5.4&0.32&0.13&0.70&0.14&...&...\\ 
G031.4868$-00.9291$&31.48678&$ -0.92911$&5.4&0.20&0.07&0.36&0.07&...&...\\ 
G031.4875$+00.8136$&31.48754&$ +0.81360$&5.1&0.17&0.06&0.30&0.06&...&...\\ 
G031.4919$+00.3568$&31.49192&$ +0.35684$&6.9&0.21&0.06&0.43&0.07&...&...\\ 
G031.4984$+00.2726$&31.49838&$ +0.27260$&5.4&0.19&0.07&0.35&0.07&...&...\\ 
G031.5000$+00.2059$&31.49997&$ +0.20586$&5.0&0.18&0.06&0.30&0.06&...&...\\ 
G031.5028$-00.7686$&31.50282&$ -0.76860$&5.0&0.14&0.06&0.32&0.07&...&...\\ 
G031.5032$-00.8332$&31.50324&$ -0.83319$&6.5&0.22&0.07&0.45&0.07&---&G031.503-00.833\\ 
G031.5101$+00.3379$&31.51011&$ +0.33788$&5.0&0.16&0.06&0.29&0.06&...&...\\ 
G031.5119$+00.3912$&31.51185&$ +0.39121$&5.1&0.17&0.06&0.30&0.06&...&...\\ 
G031.5139$+00.3631$&31.51393&$ +0.36309$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G031.5163$+00.8736$&31.51630&$ +0.87361$&5.3&0.18&0.06&0.32&0.06&...&...\\ 
G031.5239$-00.8570$&31.52387&$ -0.85701$&6.8&0.26&0.07&0.43&0.07&---&G031.524-00.857\\ 
G031.5355$-00.5348$&31.53546&$ -0.53484$&5.1&0.19&0.06&0.33&0.07&...&...\\ 
G031.5379$+00.7883$&31.53790&$ +0.78832$&5.2&0.15&0.06&0.31&0.06&...&...\\ 
G031.5434$-00.7818$&31.54338&$ -0.78180$&5.3&0.19&0.07&0.35&0.07&...&...\\ 
G031.5496$+00.4784$&31.54963&$ +0.47844$&6.1&0.20&0.06&0.36&0.06&...&...\\ 
G031.5512$+00.8767$&31.55116&$ +0.87666$&5.8&0.16&0.06&0.35&0.06&...&...\\ 
G031.5568$-00.2961$&31.55678&$ -0.29608$&5.8&0.17&0.06&0.34&0.06&...&...\\ 
G031.5571$-00.0780$&31.55713&$ -0.07802$&5.2&0.21&0.07&0.34&0.07&...&...\\ 
G031.5605$+00.3765$&31.56046&$ +0.37649$&6.7&0.25&0.06&0.41&0.07&...&...\\ 
G031.5622$-00.7653$&31.56220&$ -0.76534$&5.6&0.22&0.07&0.38&0.07&...&...\\ 
G031.5683$+00.9483$&31.56832&$ +0.94834$&5.0&0.18&0.06&0.30&0.06&...&...\\ 
G031.5694$+00.7113$&31.56942&$ +0.71130$&5.1&0.18&0.06&0.30&0.06&...&...\\ 
G031.5753$+00.2583$&31.57525&$ +0.25830$&5.2&0.14&0.06&0.30&0.06&...&...\\ 
G031.5875$-00.1038$&31.58748&$ -0.10379$&5.1&0.15&0.06&0.32&0.06&...&...\\ 
G031.5894$-00.3134$&31.58935&$ -0.31337$&5.2&0.15&0.06&0.30&0.06&...&...\\ 
G031.5909$-00.4328$&31.59088&$ -0.43282$&5.5&0.15&0.06&0.33&0.06&...&...\\ 
G031.5941$+00.7936$&31.59408&$ +0.79360$&5.1&0.15&0.06&0.29&0.06&...&...\\ 
G031.5984$-00.7969$&31.59839&$ -0.79694$&5.6&0.19&0.06&0.35&0.07&...&...\\ 
G031.6067$+00.2816$&31.60671&$ +0.28156$&5.0&0.19&0.06&0.30&0.06&...&...\\ 
G031.6091$+00.5154$&31.60908&$ +0.51538$&5.3&0.17&0.06&0.31&0.06&...&...\\ 
G031.6111$+00.0558$&31.61109&$ +0.05579$&5.2&0.20&0.06&0.33&0.07&...&...\\ 
G031.6166$-00.6713$&31.61658&$ -0.67130$&5.2&0.16&0.06&0.32&0.06&...&...\\ 
G031.6196$+00.8938$&31.61957&$ +0.89382$&5.1&0.16&0.06&0.29&0.06&...&...\\ 
G031.6245$+00.6730$&31.62450&$ +0.67296$&5.1&0.18&0.06&0.30&0.06&...&...\\ 
G031.6255$+00.7471$&31.62547&$ +0.74714$&6.4&0.17&0.06&0.38&0.06&...&...\\ 
G031.6278$-00.1141$&31.62775&$ -0.11407$&5.7&0.19&0.06&0.36&0.07&...&...\\ 
G031.6278$+00.7055$&31.62776&$ +0.70553$&5.0&0.15&0.06&0.29&0.06&...&...\\ 
G031.6310$+00.4789$&31.63095&$ +0.47892$&6.2&0.21&0.06&0.37&0.06&...&...\\ 
G031.6323$-00.5162$&31.63234&$ -0.51616$&5.0&0.16&0.06&0.32&0.07&...&...\\ 
G031.6325$+00.6426$&31.63248&$ +0.64261$&5.3&0.21&0.07&0.34&0.07&...&...\\ 
G031.6342$-00.2025$&31.63421&$ -0.20254$&5.1&0.17&0.06&0.29&0.06&...&...\\ 
G031.6503$-00.1946$&31.65032&$ -0.19462$&5.1&0.18&0.06&0.32&0.06&...&...\\ 
G031.6608$-00.4391$&31.66081&$ -0.43914$&5.2&0.15&0.06&0.32&0.06&...&...\\ 
G031.6641$+00.4236$&31.66415&$ +0.42365$&7.0&0.19&0.06&0.39&0.06&...&...\\ 
G031.6675$+00.0260$&31.66748&$ +0.02600$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G031.6849$-00.9399$&31.68486&$ -0.93987$&5.2&0.16&0.07&0.35&0.07&---&G031.685-00.940\\ 
G031.7004$+00.2807$&31.70039&$ +0.28073$&5.3&0.17&0.07&0.35&0.07&...&...\\ 
G031.7020$+00.5061$&31.70200&$ +0.50615$&5.1&0.17&0.06&0.29&0.06&...&...\\ 
G031.7040$-00.0255$&31.70400&$ -0.02546$&6.8&0.23&0.07&0.44&0.07&...&...\\ 
G031.7117$-00.8301$&31.71166&$ -0.83007$&5.1&0.17&0.07&0.34&0.07&...&...\\ 
G031.7326$+00.4249$&31.73255&$ +0.42490$&5.1&0.17&0.06&0.30&0.06&...&...\\ 
G031.7342$+00.7482$&31.73416&$ +0.74825$&5.6&0.14&0.06&0.31&0.06&---&G031.734+00.748\\ 
G031.7405$-00.4985$&31.74054&$ -0.49852$&5.3&0.17&0.06&0.32&0.06&...&...\\ 
G031.7422$-01.0181$&31.74224&$ -1.01808$&5.0&0.33&0.12&0.59&0.12&...&...\\ 
G031.7499$+00.1541$&31.74991&$ +0.15406$&5.0&0.17&0.06&0.32&0.07&...&...\\ 
G031.7528$+00.2703$&31.75276&$ +0.27031$&5.0&0.15&0.07&0.32&0.07&...&...\\ 
G031.7687$+00.2612$&31.76873&$ +0.26121$&5.2&0.18&0.07&0.32&0.07&...&...\\ 
G031.7694$+00.0658$&31.76942&$ +0.06579$&6.6&0.21&0.06&0.42&0.07&...&...\\ 
G031.7709$+00.6859$&31.77090&$ +0.68595$&5.0&0.15&0.06&0.28&0.06&...&...\\ 
G031.7725$-00.1464$&31.77248&$ -0.14636$&5.1&0.17&0.06&0.29&0.06&...&...\\ 
G031.7732$-00.8010$&31.77320&$ -0.80097$&5.0&0.16&0.06&0.32&0.07&...&...\\ 
G031.7823$-01.0143$&31.78231&$ -1.01433$&5.0&0.34&0.12&0.60&0.12&...&...\\ 
G031.7837$+00.1482$&31.78373&$ +0.14816$&5.9&0.18&0.06&0.36&0.07&...&...\\ 
G031.7870$+00.6946$&31.78701&$ +0.69463$&5.1&0.16&0.06&0.29&0.06&...&...\\ 
G031.8063$-00.7505$&31.80632&$ -0.75055$&5.1&0.18&0.06&0.31&0.06&...&...\\ 
G031.8129$+00.7507$&31.81285&$ +0.75075$&5.5&0.16&0.06&0.33&0.06&...&...\\ 
G031.8253$-00.5833$&31.82527&$ -0.58331$&5.1&0.19&0.06&0.31&0.06&...&...\\ 
G031.8280$-00.7342$&31.82799&$ -0.73423$&5.2&0.16&0.06&0.31&0.06&...&...\\ 
G031.8313$+00.9788$&31.83128&$ +0.97876$&5.5&0.24&0.07&0.37&0.07&...&...\\ 
G031.8371$-00.1902$&31.83713&$ -0.19018$&5.1&0.16&0.06&0.29&0.06&...&...\\ 
G031.8425$+00.7596$&31.84251&$ +0.75964$&5.0&0.15&0.06&0.29&0.06&...&...\\ 
G031.8427$+00.4747$&31.84270&$ +0.47469$&5.2&0.18&0.06&0.32&0.07&...&...\\ 
G031.8435$+00.0302$&31.84352&$ +0.03017$&6.7&0.23&0.07&0.44&0.07&...&...\\ 
G031.8452$+00.8794$&31.84523&$ +0.87937$&6.3&0.21&0.06&0.38&0.06&---&G031.845+00.880\\ 
G031.8491$-00.2468$&31.84915&$ -0.24678$&5.0&0.13&0.06&0.29&0.06&...&...\\ 
G031.8530$+00.5327$&31.85298&$ +0.53275$&5.2&0.16&0.06&0.30&0.06&...&...\\ 
G031.8540$+00.2002$&31.85401&$ +0.20017$&6.3&0.21&0.07&0.41&0.07&...&...\\ 
G031.8610$+00.3759$&31.86096&$ +0.37587$&5.5&0.17&0.06&0.34&0.07&...&...\\ 
G031.8639$-00.5498$&31.86388&$ -0.54984$&5.0&0.17&0.06&0.31&0.06&...&...\\ 
G031.8726$+00.2834$&31.87262&$ +0.28343$&5.1&0.19&0.07&0.33&0.07&...&...\\ 
G031.8767$-00.0667$&31.87671&$ -0.06671$&5.2&0.17&0.07&0.32&0.07&...&...\\ 
G031.8822$+00.3557$&31.88221&$ +0.35566$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G031.8826$-00.3558$&31.88255&$ -0.35580$&5.0&0.17&0.06&0.31&0.06&...&...\\ 
G031.8860$-00.2050$&31.88602&$ -0.20504$&6.1&0.21&0.06&0.37&0.07&...&...\\ 
G031.8908$+00.6150$&31.89076&$ +0.61504$&5.3&0.16&0.06&0.31&0.06&...&...\\ 
G031.8923$+00.8686$&31.89231&$ +0.86861$&5.4&0.26&0.07&0.35&0.07&...&...\\ 
G031.8958$-00.3709$&31.89582&$ -0.37087$&5.0&0.13&0.06&0.30&0.06&...&...\\ 
G031.8964$-00.4443$&31.89638&$ -0.44435$&5.0&0.18&0.07&0.37&0.08&...&...\\ 
G031.8974$-00.4509$&31.89735&$ -0.45095$&5.1&0.19&0.07&0.37&0.07&...&...\\ 
G031.9089$-00.1234$&31.90894&$ -0.12344$&5.1&0.15&0.06&0.30&0.06&...&...\\ 
G031.9115$+00.8173$&31.91155&$ +0.81728$&5.4&0.17&0.06&0.31&0.06&...&...\\ 
G031.9204$+00.7077$&31.92036&$ +0.70769$&5.3&0.17&0.06&0.30&0.06&...&...\\ 
G031.9217$-00.0155$&31.92171&$ -0.01552$&5.2&0.18&0.06&0.32&0.06&...&...\\ 
G031.9225$+00.0429$&31.92248&$ +0.04295$&5.5&0.24&0.07&0.35&0.07&...&...\\ 
G031.9300$+00.3405$&31.92999&$ +0.34052$&5.1&0.18&0.06&0.32&0.06&...&...\\ 
G031.9323$+01.0163$&31.93227&$ +1.01633$&5.0&0.27&0.11&0.54&0.12&...&...\\ 
G031.9324$+00.5322$&31.93243&$ +0.53219$&5.1&0.16&0.06&0.30&0.06&...&...\\ 
G031.9333$+00.5411$&31.93326&$ +0.54108$&5.2&0.15&0.06&0.31&0.06&...&...\\ 
G031.9350$-00.3959$&31.93499&$ -0.39594$&5.5&0.16&0.06&0.33&0.06&...&...\\ 
G031.9353$+00.2662$&31.93526&$ +0.26621$&5.2&0.17&0.07&0.34&0.07&...&...\\ 
G031.9395$+00.4453$&31.93951&$ +0.44531$&5.7&0.16&0.06&0.34&0.06&...&...\\ 
G031.9441$-00.5134$&31.94409&$ -0.51338$&5.6&0.29&0.07&0.36&0.07&---&G031.944-00.513\\ 
G031.9452$+00.5997$&31.94521&$ +0.59969$&5.4&0.17&0.06&0.33&0.07&---&G031.945+00.600\\ 
G031.9583$+00.4357$&31.95833&$ +0.43566$&5.5&0.20&0.06&0.32&0.06&...&...\\ 
G031.9673$-00.1098$&31.96734&$ -0.10976$&5.1&0.18&0.06&0.32&0.07&...&...\\ 
G031.9766$-00.2551$&31.97658&$ -0.25511$&5.0&0.17&0.06&0.29&0.06&...&...\\ 
G031.9899$-00.3218$&31.98992&$ -0.32185$&5.0&0.20&0.06&0.30&0.06&...&...\\ 
G031.9900$+00.9618$&31.98998&$ +0.96181$&5.1&0.19&0.06&0.31&0.06&...&...\\ 
G032.0031$+00.5589$&32.00314&$ +0.55886$&5.6&0.18&0.07&0.36&0.07&---&G032.003+00.560(I)\\ 
G032.0084$+00.3542$&32.00843&$ +0.35420$&7.0&0.22&0.06&0.43&0.07&---&G032.008+00.354\\ 
G032.0101$+00.8680$&32.01005&$ +0.86805$&6.4&0.27&0.06&0.39&0.07&...&...\\ 
G032.0107$-00.7139$&32.01069&$ -0.71388$&5.5&0.16&0.06&0.31&0.06&...&...\\ 
G032.0211$+00.1914$&32.02115&$ +0.19135$&5.5&0.24&0.07&0.35&0.07&...&...\\ 
G032.0293$+00.0490$&32.02934&$ +0.04899$&6.0&0.48&0.07&0.38&0.07&*&G032.030+00.049\\ 
G032.0354$+00.1557$&32.03538&$ +0.15573$&5.2&0.17&0.07&0.34&0.07&...&...\\ 
G032.0646$-00.4204$&32.06461&$ -0.42039$&5.3&0.16&0.06&0.30&0.06&...&...\\ 
G032.0682$-00.6825$&32.06820&$ -0.68249$&5.1&0.16&0.06&0.30&0.06&...&...\\ 
G032.0733$-00.8178$&32.07333&$ -0.81784$&5.6&0.19&0.06&0.35&0.06&...&...\\ 
G032.0736$+00.7707$&32.07361&$ +0.77075$&5.3&0.19&0.06&0.34&0.07&...&...\\ 
G032.0767$-00.4904$&32.07669&$ -0.49039$&5.4&0.17&0.06&0.32&0.06&...&...\\ 
G032.0804$+00.1629$&32.08039&$ +0.16295$&5.2&0.18&0.06&0.31&0.06&...&...\\ 
G032.0852$+00.0250$&32.08525&$ +0.02503$&5.2&0.19&0.06&0.32&0.06&...&...\\ 
G032.0877$+00.6670$&32.08772&$ +0.66699$&5.1&0.16&0.07&0.32&0.07&...&...\\ 
G032.0892$+00.8058$&32.08917&$ +0.80575$&5.1&0.15&0.06&0.32&0.06&...&...\\ 
G032.0936$+00.3135$&32.09358&$ +0.31350$&5.0&0.15&0.06&0.30&0.06&...&...\\ 
G032.1149$+00.1163$&32.11490&$ +0.11628$&5.5&0.20&0.07&0.38&0.07&...&...\\ 
G032.1154$-00.4402$&32.11538&$ -0.44018$&5.1&0.16&0.06&0.28&0.06&...&...\\ 
G032.1196$-00.1964$&32.11962&$ -0.19643$&5.5&0.21&0.06&0.33&0.06&...&...\\ 
G032.1340$+00.7044$&32.13397&$ +0.70435$&6.2&0.20&0.07&0.40&0.07&---&G032.134+00.704\\ 
G032.1551$-00.0725$&32.15511&$ -0.07254$&6.2&0.17&0.06&0.36&0.06&...&...\\ 
G032.1721$-00.4716$&32.17211&$ -0.47157$&6.4&0.22&0.06&0.38&0.06&...&...\\ 
G032.1736$-00.7060$&32.17363&$ -0.70603$&5.2&0.17&0.06&0.30&0.06&...&...\\ 
G032.1748$+00.2016$&32.17476&$ +0.20163$&6.8&0.22&0.06&0.42&0.07&...&...\\ 
G032.1781$+00.7573$&32.17807&$ +0.75734$&5.1&0.18&0.06&0.32&0.06&...&...\\ 
G032.1793$+00.1976$&32.17935&$ +0.19760$&5.4&0.19&0.06&0.34&0.07&...&...\\ 
G032.1825$-00.9731$&32.18250&$ -0.97314$&5.1&0.20&0.06&0.32&0.06&...&...\\ 
G032.1853$-00.3073$&32.18532&$ -0.30733$&5.5&0.18&0.06&0.34&0.06&...&...\\ 
G032.1930$+00.3064$&32.19296&$ +0.30635$&5.3&0.16&0.06&0.31&0.06&...&...\\ 
G032.1984$+00.9142$&32.19841&$ +0.91424$&5.3&0.17&0.06&0.33&0.06&...&...\\ 
G032.2039$-00.3948$&32.20392&$ -0.39476$&5.7&0.22&0.06&0.35&0.07&Rad&G032.204-00.395\\ 
G032.2081$-00.1778$&32.20810&$ -0.17782$&5.0&0.15&0.06&0.29&0.06&...&...\\ 
G032.2100$+00.5846$&32.21003&$ +0.58455$&5.0&0.17&0.06&0.31&0.07&...&...\\ 
G032.2113$-00.3073$&32.21129&$ -0.30726$&5.2&0.19&0.06&0.30&0.06&...&...\\ 
G032.2314$-00.2097$&32.23136&$ -0.20969$&5.1&0.20&0.06&0.32&0.06&...&...\\ 
G032.2348$+00.1384$&32.23476&$ +0.13836$&5.5&0.18&0.06&0.34&0.06&...&...\\ 
G032.2390$-00.7071$&32.23898&$ -0.70714$&5.3&0.18&0.06&0.33&0.07&...&...\\ 
G032.2391$+00.3176$&32.23907&$ +0.31760$&5.2&0.17&0.06&0.32&0.06&...&...\\ 
G032.2393$-00.3653$&32.23934&$ -0.36532$&5.0&0.17&0.07&0.35&0.07&...&...\\ 
G032.2453$+00.1216$&32.24525&$ +0.12163$&5.0&0.17&0.06&0.31&0.06&...&...\\ 
G032.2502$-00.7008$&32.25023&$ -0.70082$&5.5&0.21&0.06&0.33&0.06&...&...\\ 
G032.2555$-00.3306$&32.25553&$ -0.33060$&5.7&0.22&0.07&0.38&0.07&...&...\\ 
G032.2583$-00.8719$&32.25835&$ -0.87195$&5.3&0.17&0.06&0.31&0.06&...&...\\ 
G032.2692$-00.7535$&32.26919&$ -0.75346$&5.0&0.15&0.06&0.30&0.06&...&...\\ 
G032.2771$-00.1881$&32.27706&$ -0.18809$&5.2&0.17&0.06&0.31&0.06&...&...\\ 
G032.2777$-00.2882$&32.27775&$ -0.28823$&5.2&0.20&0.07&0.34&0.07&...&...\\ 
G032.2807$-00.4755$&32.28073&$ -0.47553$&6.5&0.19&0.06&0.39&0.06&...&...\\ 
G032.2875$+00.6826$&32.28746&$ +0.68262$&5.2&0.15&0.06&0.33&0.07&...&...\\ 
G032.2901$+00.1245$&32.29011&$ +0.12448$&6.3&0.26&0.07&0.41&0.07&...&...\\ 
G032.2908$+00.7221$&32.29079&$ +0.72206$&5.9&0.19&0.07&0.38&0.07&...&...\\ 
G032.2939$-00.3265$&32.29393&$ -0.32650$&6.2&0.30&0.09&0.55&0.09&...&...\\ 
G032.2994$+00.8033$&32.29940&$ +0.80332$&5.2&0.17&0.07&0.34&0.07&...&...\\ 
G032.3077$+00.4089$&32.30768&$ +0.40892$&5.0&0.17&0.06&0.30&0.06&...&...\\ 
G032.3105$-00.9056$&32.31051&$ -0.90563$&6.2&0.19&0.06&0.38&0.07&...&...\\ 
G032.3115$+00.9911$&32.31147&$ +0.99112$&5.2&0.32&0.13&0.67&0.13&---&G032.311+00.991\\ 
G032.3115$-00.7692$&32.31149&$ -0.76916$&5.1&0.16&0.06&0.29&0.06&...&...\\ 
G032.3182$-00.5345$&32.31816&$ -0.53449$&5.1&0.17&0.06&0.31&0.06&...&...\\ 
G032.3242$-00.7249$&32.32420&$ -0.72492$&5.5&0.20&0.06&0.33&0.06&...&...\\ 
G032.3314$-00.6407$&32.33142&$ -0.64075$&5.5&0.16&0.06&0.34&0.06&...&...\\ 
G032.3438$-00.1843$&32.34379&$ -0.18428$&5.3&0.15&0.06&0.31&0.06&...&...\\ 
G032.3505$-00.0750$&32.35053&$ -0.07497$&5.2&0.17&0.06&0.31&0.06&...&...\\ 
G032.3589$-00.6614$&32.35885&$ -0.66144$&5.2&0.17&0.06&0.30&0.06&...&...\\ 
G032.3608$-00.9940$&32.36079&$ -0.99398$&5.3&0.21&0.08&0.43&0.09&...&...\\ 
G032.3635$+00.9336$&32.36350&$ +0.93361$&6.5&1.92&0.23&1.41&0.22&Rad&G032.364+00.933(I)\\ 
G032.3641$+00.8058$&32.36406&$ +0.80582$&5.2&0.14&0.06&0.30&0.06&...&...\\ 
G032.3653$-00.3448$&32.36525&$ -0.34483$&5.5&0.21&0.08&0.44&0.09&...&...\\ 
G032.3675$+00.1677$&32.36747&$ +0.16767$&5.4&0.18&0.06&0.33&0.07&...&...\\ 
G032.3760$+00.4827$&32.37601&$ +0.48274$&5.1&0.18&0.06&0.31&0.06&...&...\\ 
G032.3775$-00.0666$&32.37747&$ -0.06664$&5.0&0.15&0.06&0.29&0.06&...&...\\ 
G032.3832$-00.7456$&32.38316&$ -0.74562$&5.1&0.19&0.07&0.32&0.07&...&...\\ 
G032.3925$+00.8378$&32.39246&$ +0.83777$&5.0&0.15&0.08&0.38&0.08&...&...\\ 
G032.4031$+00.0486$&32.40310&$ +0.04857$&5.5&0.16&0.06&0.33&0.06&...&...\\ 
G032.4048$-00.1895$&32.40477&$ -0.18948$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G032.4084$-00.9653$&32.40836&$ -0.96529$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G032.4089$+00.4150$&32.40886&$ +0.41503$&5.2&0.16&0.06&0.30&0.06&...&...\\ 
G032.4143$+00.5887$&32.41435&$ +0.58872$&5.5&0.18&0.06&0.35&0.07&...&...\\ 
G032.4240$-00.1930$&32.42400&$ -0.19303$&5.2&0.17&0.06&0.31&0.06&...&...\\ 
G032.4249$-00.2633$&32.42490&$ -0.26330$&5.4&0.17&0.06&0.34&0.07&...&...\\ 
G032.4279$+00.9062$&32.42788&$ +0.90625$&5.2&0.25&0.11&0.55&0.12&...&...\\ 
G032.4282$-00.7424$&32.42823&$ -0.74242$&5.1&0.19&0.07&0.35&0.07&...&...\\ 
G032.4292$-00.4691$&32.42921&$ -0.46914$&5.2&0.18&0.07&0.36&0.07&...&...\\ 
G032.4355$+00.8831$&32.43545&$ +0.88305$&5.2&0.28&0.12&0.62&0.12&...&...\\ 
G032.4357$-00.6852$&32.43566&$ -0.68519$&5.1&0.18&0.07&0.35&0.07&...&...\\ 
G032.4436$-00.8486$&32.44365&$ -0.84861$&5.1&0.18&0.07&0.33&0.07&...&...\\ 
G032.4450$-00.6014$&32.44497&$ -0.60144$&5.1&0.22&0.06&0.30&0.06&...&...\\ 
G032.4493$+00.3198$&32.44935&$ +0.31975$&5.6&0.19&0.06&0.33&0.06&...&...\\ 
G032.4546$+00.1714$&32.45463&$ +0.17142$&6.1&0.29&0.08&0.47&0.08&...&...\\ 
G032.4561$+00.9557$&32.45608&$ +0.95570$&5.3&0.34&0.11&0.56&0.11&...&...\\ 
G032.4634$-00.3355$&32.46338&$ -0.33553$&5.2&0.19&0.08&0.40&0.08&...&...\\ 
G032.4720$-00.8478$&32.47199&$ -0.84785$&5.1&0.19&0.07&0.35&0.07&...&...\\ 
G032.4739$+00.2019$&32.47393&$ +0.20191$&6.3&0.42&0.09&0.57&0.10&cor&G032.472+00.203(F)\\ 
G032.4748$-00.2353$&32.47477&$ -0.23532$&5.0&0.17&0.06&0.29&0.06&...&...\\ 
G032.4828$-00.7339$&32.48282&$ -0.73395$&5.1&0.25&0.07&0.36&0.07&...&...\\ 
G032.4934$+00.9945$&32.49338&$ +0.99446$&5.3&0.27&0.09&0.44&0.09&...&...\\ 
G032.4937$+00.1595$&32.49372&$ +0.15948$&6.8&0.25&0.07&0.47&0.07&...&...\\ 
G032.4978$-00.9798$&32.49775&$ -0.97981$&5.1&0.21&0.07&0.36&0.08&...&...\\ 
G032.5022$+00.1192$&32.50220&$ +0.11920$&5.2&0.16&0.06&0.33&0.07&...&...\\ 
G032.5053$-00.8810$&32.50525&$ -0.88098$&5.0&0.20&0.08&0.39&0.08&...&...\\ 
G032.5057$-00.0610$&32.50574&$ -0.06101$&5.6&0.19&0.06&0.33&0.06&...&...\\ 
G032.5109$+00.2418$&32.51088&$ +0.24177$&5.7&0.25&0.07&0.36&0.07&---&G032.510+00.242\\ 
G032.5218$+00.4125$&32.52178&$ +0.41253$&5.0&0.15&0.06&0.28&0.06&...&...\\ 
G032.5228$+00.7478$&32.52282&$ +0.74776$&5.3&0.17&0.06&0.32&0.06&...&...\\ 
G032.5518$+00.0061$&32.55178&$ +0.00607$&5.2&0.15&0.06&0.29&0.06&...&...\\ 
G032.5543$+00.0848$&32.55435&$ +0.08475$&6.0&0.19&0.06&0.35&0.06&...&...\\ 
G032.5639$-00.5985$&32.56387&$ -0.59852$&5.5&0.17&0.06&0.33&0.06&...&...\\ 
G032.5662$-00.4451$&32.56616&$ -0.44511$&5.0&0.23&0.07&0.36&0.07&...&...\\ 
G032.5712$+00.2759$&32.57123&$ +0.27593$&5.2&0.18&0.06&0.30&0.06&...&...\\ 
G032.5839$+00.7648$&32.58387&$ +0.76484$&5.4&0.18&0.06&0.29&0.06&...&...\\ 
G032.5899$-00.7483$&32.58991&$ -0.74825$&5.0&0.18&0.06&0.31&0.06&...&...\\ 
G032.5973$+00.6784$&32.59727&$ +0.67838$&5.9&0.19&0.06&0.36&0.06&...&...\\ 
G032.6015$+00.8627$&32.60151&$ +0.86270$&5.8&0.22&0.06&0.36&0.07&...&...\\ 
G032.6053$+00.9338$&32.60527&$ +0.93375$&5.2&0.17&0.06&0.31&0.06&...&...\\ 
G032.6159$+00.2736$&32.61588&$ +0.27364$&5.2&0.18&0.06&0.32&0.06&...&...\\ 
G032.6178$-00.0909$&32.61782&$ -0.09094$&5.0&0.15&0.07&0.34&0.07&...&...\\ 
G032.6197$+00.4696$&32.61970&$ +0.46962$&5.0&0.15&0.06&0.30&0.06&...&...\\ 
G032.6225$-00.1584$&32.62254&$ -0.15844$&5.0&0.18&0.07&0.35&0.07&...&...\\ 
G032.6304$-00.8369$&32.63041&$ -0.83694$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G032.6352$+00.9160$&32.63520&$ +0.91604$&5.0&0.15&0.06&0.29&0.06&...&...\\ 
G032.6413$+00.6898$&32.64130&$ +0.68977$&6.6&0.16&0.06&0.37&0.06&...&...\\ 
G032.6545$-00.6596$&32.65450&$ -0.65957$&6.2&0.24&0.07&0.40&0.07&...&...\\ 
G032.6550$+00.2977$&32.65505&$ +0.29767$&5.1&0.19&0.07&0.34&0.07&...&...\\ 
G032.6551$-00.8121$&32.65506&$ -0.81215$&5.1&0.14&0.06&0.29&0.06&...&...\\ 
G032.6614$-00.2182$&32.66137&$ -0.21816$&6.0&0.42&0.07&0.42&0.07&Rad&...\\ 
G032.6667$+00.5881$&32.66665&$ +0.58810$&5.3&0.17&0.06&0.30&0.06&...&...\\ 
G032.6673$+00.3436$&32.66734&$ +0.34364$&5.0&0.18&0.06&0.30&0.06&...&...\\ 
G032.6691$-00.9914$&32.66910&$ -0.99141$&5.4&0.27&0.08&0.43&0.08&...&...\\ 
G032.6703$-00.1708$&32.67032&$ -0.17080$&5.3&0.19&0.07&0.36&0.07&...&...\\ 
G032.6737$-00.0543$&32.67373&$ -0.05434$&5.0&0.16&0.07&0.34&0.07&...&...\\ 
G032.6772$-00.2811$&32.67720&$ -0.28108$&5.4&0.22&0.07&0.35&0.07&...&...\\ 
G032.6784$+00.5537$&32.67839&$ +0.55365$&5.0&0.15&0.06&0.29&0.06&...&...\\ 
G032.6799$-00.9548$&32.67986&$ -0.95481$&6.7&0.27&0.06&0.41&0.07&...&...\\ 
G032.6816$+00.3625$&32.68158&$ +0.36246$&6.2&0.20&0.06&0.34&0.06&...&...\\ 
G032.6818$-00.7556$&32.68180&$ -0.75562$&5.0&0.15&0.06&0.29&0.06&...&...\\ 
G032.6883$-00.7765$&32.68826&$ -0.77645$&5.2&0.18&0.06&0.30&0.06&...&...\\ 
G032.6906$+00.6552$&32.69061&$ +0.65518$&5.0&0.15&0.06&0.29&0.06&...&...\\ 
G032.6953$+00.6607$&32.69534&$ +0.66074$&6.6&0.23&0.06&0.39&0.06&...&...\\ 
G032.6996$-00.5655$&32.69957&$ -0.56553$&5.7&0.17&0.06&0.35&0.07&...&...\\ 
G032.7011$-00.7856$&32.70111&$ -0.78562$&6.9&0.21&0.06&0.39&0.06&...&...\\ 
G032.7053$+00.4489$&32.70526&$ +0.44892$&6.5&0.25&0.06&0.41&0.07&...&...\\ 
G032.7054$+00.0127$&32.70539&$ +0.01267$&6.6&0.22&0.07&0.45&0.07&...&...\\ 
G032.7092$-00.5020$&32.70915&$ -0.50199$&6.4&0.21&0.06&0.39&0.07&...&...\\ 
G032.7111$-00.9940$&32.71112&$ -0.99398$&6.6&0.32&0.08&0.54&0.09&---&G032.711-00.994\\ 
G032.7123$+00.2865$&32.71234&$ +0.28649$&5.8&0.30&0.09&0.52&0.09&...&...\\ 
G032.7185$-00.7746$&32.71847&$ -0.77458$&6.1&0.22&0.06&0.36&0.06&...&...\\ 
G032.7188$+00.4238$&32.71880&$ +0.42378$&5.0&0.20&0.06&0.30&0.06&...&...\\ 
G032.7208$+00.8137$&32.72076&$ +0.81374$&5.7&0.15&0.06&0.32&0.06&...&...\\ 
G032.7232$+00.9958$&32.72320&$ +0.99578$&5.2&0.25&0.08&0.41&0.08&...&...\\ 
G032.7268$+00.4639$&32.72679&$ +0.46386$&5.4&0.15&0.06&0.32&0.06&...&...\\ 
G032.7418$-00.8657$&32.74181&$ -0.86570$&6.0&0.20&0.06&0.37&0.06&...&...\\ 
G032.7453$-00.0358$&32.74532&$ -0.03580$&5.0&0.16&0.07&0.36&0.08&...&...\\ 
G032.7492$-00.0652$&32.74921&$ -0.06518$&5.4&0.87&0.10&0.49&0.09&HII&...\\ 
G032.7509$+00.9332$&32.75091&$ +0.93320$&5.4&0.16&0.06&0.31&0.06&...&...\\ 
G032.7517$-00.8208$&32.75167&$ -0.82076$&6.7&0.22&0.06&0.40&0.06&...&...\\ 
G032.7526$+00.8396$&32.75264&$ +0.83957$&5.7&0.20&0.06&0.33&0.06&...&...\\ 
G032.7551$-00.9298$&32.75515&$ -0.92980$&6.9&0.24&0.07&0.44&0.07&---&G032.755-00.930\\ 
G032.7596$-00.7310$&32.75958&$ -0.73096$&5.6&0.21&0.06&0.35&0.07&---&G032.760-00.731\\ 
G032.7625$-00.1338$&32.76255&$ -0.13379$&5.0&0.20&0.07&0.32&0.07&...&...\\ 
G032.7631$-00.7824$&32.76306&$ -0.78242$&6.2&0.19&0.06&0.38&0.06&...&...\\ 
G032.7664$+00.7876$&32.76639&$ +0.78756$&5.3&0.18&0.06&0.32&0.06&...&...\\ 
G032.7701$-00.5118$&32.77006&$ -0.51178$&5.1&0.19&0.07&0.33&0.07&...&...\\ 
G032.7727$+00.6494$&32.77270&$ +0.64942$&5.8&0.20&0.06&0.33&0.06&...&...\\ 
G032.7795$-00.5872$&32.77950&$ -0.58720$&5.0&0.14&0.06&0.31&0.06&...&...\\ 
G032.7810$-00.7289$&32.78104&$ -0.72895$&5.2&0.21&0.07&0.34&0.07&...&...\\ 
G032.8047$+00.9473$&32.80467&$ +0.94730$&5.5&0.19&0.06&0.34&0.07&...&...\\ 
G032.8094$+00.0297$&32.80935&$ +0.02968$&5.0&0.22&0.07&0.34&0.07&...&...\\ 
G032.8137$-00.1737$&32.81366&$ -0.17365$&5.0&0.17&0.06&0.30&0.06&...&...\\ 
G032.8287$-00.8135$&32.82869&$ -0.81347$&5.1&0.15&0.06&0.32&0.07&...&...\\ 
G032.8393$-00.1019$&32.83928&$ -0.10191$&5.0&0.19&0.07&0.37&0.08&...&...\\ 
G032.8453$-00.1202$&32.84533&$ -0.12018$&5.3&0.20&0.07&0.37&0.07&...&...\\ 
G032.8515$+00.8478$&32.85147&$ +0.84784$&5.1&0.18&0.06&0.30&0.06&...&...\\ 
G032.8546$-00.1817$&32.85463&$ -0.18171$&5.1&0.21&0.07&0.36&0.07&...&...\\ 
G032.8577$+00.0630$&32.85769&$ +0.06302$&7.0&0.24&0.07&0.48&0.07&...&...\\ 
G032.8792$+00.7369$&32.87925&$ +0.73693$&5.0&0.19&0.06&0.31&0.07&...&...\\ 
G032.8818$-00.0556$&32.88178&$ -0.05559$&5.1&0.18&0.07&0.32&0.07&...&...\\ 
G032.8830$+00.4808$&32.88298&$ +0.48080$&5.2&0.16&0.06&0.33&0.07&...&...\\ 
G032.8848$+00.3780$&32.88478&$ +0.37802$&5.1&0.19&0.06&0.31&0.06&...&...\\ 
G032.8946$-00.3546$&32.89457&$ -0.35456$&5.6&0.19&0.07&0.37&0.07&...&...\\ 
G032.8958$+00.9013$&32.89579&$ +0.90132$&5.2&0.17&0.06&0.31&0.06&...&...\\ 
G032.9023$+00.3382$&32.90235&$ +0.33823$&5.5&0.21&0.07&0.38&0.08&...&...\\ 
G032.9025$-00.6262$&32.90250&$ -0.62623$&5.9&0.21&0.06&0.35&0.06&...&...\\ 
G032.9062$+00.5005$&32.90617&$ +0.50052$&5.6&0.21&0.07&0.38&0.07&...&...\\ 
G032.9111$-00.2951$&32.91110&$ -0.29511$&5.0&0.19&0.07&0.33&0.07&...&...\\ 
G032.9117$+00.4631$&32.91173&$ +0.46309$&5.0&0.17&0.07&0.31&0.07&...&...\\ 
G032.9192$-00.3709$&32.91922&$ -0.37094$&5.7&0.20&0.08&0.43&0.08&...&...\\ 
G032.9290$+00.6052$&32.92903&$ +0.60518$&5.8&0.42&0.11&0.62&0.12&bub&G032.928+00.606(F)\\ 
G032.9308$-00.9275$&32.93080&$ -0.92751$&5.1&0.30&0.08&0.38&0.08&...&...\\ 
G032.9339$+00.3025$&32.93394&$ +0.30246$&5.2&0.21&0.07&0.36&0.07&...&...\\ 
G032.9394$-00.2137$&32.93936&$ -0.21372$&5.1&0.22&0.07&0.33&0.07&...&...\\ 
G032.9514$-00.1873$&32.95137&$ -0.18733$&5.3&0.17&0.07&0.35&0.07&...&...\\ 
G032.9528$+00.3416$&32.95283&$ +0.34163$&5.8&0.23&0.07&0.40&0.07&...&...\\ 
G032.9720$-00.6072$&32.97195&$ -0.60720$&5.3&0.17&0.07&0.35&0.07&...&...\\ 
G032.9729$+00.5096$&32.97292&$ +0.50955$&5.3&0.23&0.10&0.50&0.10&...&...\\ 
G032.9739$-00.2760$&32.97387&$ -0.27601$&5.1&0.18&0.07&0.35&0.07&...&...\\ 
G032.9796$-00.2611$&32.97957&$ -0.26108$&5.7&0.19&0.07&0.37&0.07&...&...\\ 
G032.9800$-00.8945$&32.97997&$ -0.89452$&5.1&0.20&0.07&0.33&0.07&...&...\\ 
G032.9823$-00.0569$&32.98227&$ -0.05691$&6.4&0.25&0.07&0.46&0.08&...&...\\ 
G032.9839$-00.1396$&32.98387&$ -0.13955$&5.1&0.15&0.07&0.34&0.07&...&...\\ 
G032.9863$+00.2597$&32.98631&$ +0.25968$&5.1&0.17&0.07&0.34&0.07&...&...\\ 
G032.9931$+00.7009$&32.99314&$ +0.70088$&5.1&0.18&0.07&0.33&0.07&...&...\\ 
G032.9985$-00.6586$&32.99849&$ -0.65860$&5.2&0.19&0.06&0.32&0.07&...&...\\ 
G033.0068$-00.1284$&33.00684&$ -0.12837$&5.1&0.20&0.07&0.34&0.07&...&...\\ 
G033.0139$-00.1086$&33.01393&$ -0.10865$&6.1&0.30&0.07&0.43&0.08&...&...\\ 
G033.0169$-00.4075$&33.01690&$ -0.40754$&6.4&0.35&0.09&0.57&0.10&...&...\\ 
G033.0225$+00.9845$&33.02254&$ +0.98445$&5.2&0.21&0.07&0.37&0.07&...&...\\ 
G033.0228$+00.3959$&33.02281&$ +0.39587$&6.1&0.24&0.07&0.40&0.07&...&...\\ 
G033.0239$-00.1668$&33.02393&$ -0.16678$&5.0&0.21&0.07&0.34&0.07&...&...\\ 
G033.0255$+00.5487$&33.02550&$ +0.54865$&5.4&0.19&0.08&0.45&0.09&...&...\\ 
G033.0260$-00.4719$&33.02600&$ -0.47192$&6.2&0.23&0.07&0.43&0.07&...&...\\ 
G033.0273$+00.0815$&33.02733&$ +0.08149$&5.4&0.22&0.07&0.34&0.07&...&...\\ 
G033.0552$-00.3750$&33.05524&$ -0.37504$&5.9&0.21&0.08&0.44&0.08&...&...\\ 
G033.0606$-00.1195$&33.06059&$ -0.11948$&5.3&0.24&0.08&0.41&0.08&...&...\\ 
G033.0641$-00.0389$&33.06414&$ -0.03886$&5.2&0.23&0.07&0.38&0.08&...&...\\ 
G033.0695$-00.7623$&33.06952&$ -0.76228$&5.0&0.21&0.07&0.33&0.07&...&...\\ 
G033.0711$-00.2271$&33.07115&$ -0.22712$&5.2&0.18&0.07&0.34&0.07&...&...\\ 
G033.0731$+00.7853$&33.07306&$ +0.78526$&5.0&0.20&0.06&0.30&0.06&...&...\\ 
G033.0783$+00.8714$&33.07826&$ +0.87138$&5.2&0.19&0.06&0.30&0.06&...&...\\ 
G033.0809$+00.2398$&33.08094&$ +0.23982$&5.0&0.17&0.07&0.32&0.07&...&...\\ 
G033.0827$+00.2950$&33.08267&$ +0.29496$&5.5&0.17&0.07&0.36&0.07&...&...\\ 
G033.0852$+00.9685$&33.08519&$ +0.96848$&5.3&0.19&0.07&0.34&0.07&...&...\\ 
G033.0952$-00.3872$&33.09524&$ -0.38719$&5.7&0.21&0.07&0.36&0.07&...&...\\ 
G033.0956$+00.4177$&33.09559&$ +0.41767$&5.0&0.22&0.07&0.36&0.08&...&...\\ 
G033.1031$-00.6951$&33.10307&$ -0.69506$&5.6&0.21&0.07&0.35&0.07&...&...\\ 
G033.1039$-00.5261$&33.10391&$ -0.52609$&5.1&0.17&0.07&0.34&0.07&...&...\\ 
G033.1095$+00.2310$&33.10948&$ +0.23100$&5.5&0.22&0.07&0.37&0.07&...&...\\ 
G033.1130$+00.8761$&33.11298&$ +0.87611$&5.1&0.17&0.06&0.30&0.06&...&...\\ 
G033.1205$-00.3207$&33.12045&$ -0.32067$&5.2&0.19&0.07&0.34&0.07&...&...\\ 
G033.1237$+00.3575$&33.12371&$ +0.35753$&5.0&0.19&0.07&0.33&0.07&...&...\\ 
G033.1275$+00.5464$&33.12752&$ +0.54636$&6.8&0.25&0.07&0.43&0.07&...&...\\ 
G033.1295$+00.5487$&33.12947&$ +0.54865$&5.0&0.17&0.06&0.32&0.07&...&...\\ 
G033.1390$-00.8482$&33.13896&$ -0.84819$&5.0&0.23&0.07&0.35&0.07&...&...\\ 
G033.1518$+00.5049$&33.15183&$ +0.50490$&5.2&0.17&0.07&0.33&0.07&...&...\\ 
G033.1600$+00.0609$&33.15997&$ +0.06093$&5.5&0.22&0.07&0.39&0.07&...&...\\ 
G033.1633$+00.7624$&33.16335&$ +0.76241$&5.4&0.18&0.07&0.35&0.07&...&...\\ 
G033.1636$+00.4914$&33.16357&$ +0.49136$&5.0&0.19&0.07&0.34&0.07&...&...\\ 
G033.1637$+00.1081$&33.16372&$ +0.10809$&5.2&0.21&0.07&0.33&0.07&...&...\\ 
G033.1701$-00.5301$&33.17010&$ -0.53012$&5.6&0.17&0.06&0.33&0.06&...&...\\ 
G033.1703$+00.0934$&33.17032&$ +0.09343$&6.8&0.27&0.07&0.45&0.07&...&...\\ 
G033.1714$-00.4739$&33.17135&$ -0.47386$&6.5&0.20&0.06&0.39&0.06&...&...\\ 
G033.1728$-00.5234$&33.17281&$ -0.52345$&5.3&0.16&0.06&0.32&0.06&...&...\\ 
G033.1801$+00.8729$&33.18014&$ +0.87291$&6.8&0.23&0.06&0.41&0.07&---&G033.180+00.873\\ 
G033.1811$-00.2785$&33.18108&$ -0.27851$&5.2&0.19&0.06&0.30&0.06&...&...\\ 
G033.2019$+00.2849$&33.20191&$ +0.28489$&5.5&0.19&0.07&0.35&0.07&...&...\\ 
G033.2064$+00.5332$&33.20642&$ +0.53323$&5.0&0.19&0.06&0.32&0.07&...&...\\ 
G033.2141$-00.3898$&33.21406&$ -0.38976$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G033.2181$+00.6807$&33.21808&$ +0.68074$&5.0&0.16&0.06&0.31&0.07&...&...\\ 
G033.2204$-00.0724$&33.22039&$ -0.07240$&5.3&0.18&0.07&0.35&0.07&...&...\\ 
G033.2237$-00.1037$&33.22365&$ -0.10372$&5.6&0.25&0.07&0.37&0.07&...&...\\ 
G033.2246$-00.2093$&33.22456&$ -0.20928$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G033.2364$+00.6523$&33.23642&$ +0.65234$&6.6&0.24&0.06&0.41&0.07&...&...\\ 
G033.2415$-00.9864$&33.24153&$ -0.98641$&5.3&0.22&0.08&0.40&0.08&...&...\\ 
G033.2438$+00.7971$&33.24384&$ +0.79707$&5.1&0.18&0.06&0.32&0.06&...&...\\ 
G033.2487$-00.5657$&33.24871&$ -0.56574$&5.1&0.16&0.06&0.31&0.07&...&...\\ 
G033.2549$+00.2584$&33.25490&$ +0.25843$&5.1&0.21&0.07&0.36&0.07&...&...\\ 
G033.2556$-00.5245$&33.25559&$ -0.52449$&5.4&0.19&0.06&0.33&0.06&...&...\\ 
G033.2682$-00.5510$&33.26823&$ -0.55102$&5.3&0.20&0.07&0.36&0.07&...&...\\ 
G033.2682$+00.0822$&33.26824&$ +0.08218$&5.0&0.17&0.07&0.33&0.07&...&...\\ 
G033.2707$-00.0688$&33.27067&$ -0.06879$&5.1&0.19&0.07&0.33&0.07&...&...\\ 
G033.2729$-01.0129$&33.27292&$ -1.01287$&5.0&0.29&0.11&0.53&0.11&...&...\\ 
G033.2803$-00.1664$&33.28025&$ -0.16643$&5.5&0.21&0.06&0.33&0.06&...&...\\ 
G033.2816$-00.2610$&33.28164&$ -0.26101$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G033.2836$-00.4280$&33.28358&$ -0.42796$&5.3&0.18&0.06&0.33&0.06&...&...\\ 
G033.2848$+00.3415$&33.28483&$ +0.34149$&5.0&0.22&0.10&0.51&0.10&...&...\\ 
G033.2862$-00.1688$&33.28622&$ -0.16879$&6.7&0.22&0.06&0.43&0.07&IR&...\\ 
G033.2889$+00.5991$&33.28892&$ +0.59907$&5.8&0.17&0.06&0.36&0.07&...&...\\ 
G033.2988$+00.8652$&33.29884&$ +0.86520$&5.9&0.18&0.07&0.38&0.07&...&...\\ 
G033.3134$+00.5593$&33.31344&$ +0.55934$&5.3&0.17&0.06&0.33&0.06&...&...\\ 
G033.3202$-00.6341$&33.32017&$ -0.63408$&5.5&0.18&0.06&0.35&0.07&...&...\\ 
G033.3208$+00.7035$&33.32079&$ +0.70345$&5.8&0.22&0.07&0.39&0.07&...&...\\ 
G033.3233$+00.5565$&33.32330&$ +0.55650$&5.1&0.15&0.06&0.32&0.07&...&...\\ 
G033.3363$-00.0010$&33.33629&$ -0.00101$&6.8&0.38&0.11&0.71&0.11&...&...\\ 
G033.3400$+00.8106$&33.34003&$ +0.81061$&5.4&0.15&0.06&0.32&0.06&...&...\\ 
G033.3448$-00.7709$&33.34482&$ -0.77090$&5.1&0.18&0.07&0.36&0.07&...&...\\ 
G033.3493$+00.6644$&33.34927&$ +0.66442$&5.1&0.20&0.07&0.34&0.07&...&...\\ 
G033.3553$-00.3564$&33.35532&$ -0.35643$&5.0&0.17&0.06&0.31&0.07&...&...\\ 
G033.3637$-00.6738$&33.36372&$ -0.67380$&5.8&0.19&0.07&0.37&0.07&...&...\\ 
G033.3678$-00.3596$&33.36782&$ -0.35962$&5.9&0.19&0.07&0.38&0.07&...&...\\ 
G033.3681$+00.6051$&33.36809&$ +0.60511$&5.1&0.19&0.07&0.34&0.07&...&...\\ 
G033.3687$+00.5465$&33.36872&$ +0.54650$&5.2&0.21&0.07&0.33&0.07&...&...\\ 
G033.3802$+00.1389$&33.38018&$ +0.13892$&5.5&0.37&0.12&0.65&0.13&...&...\\ 
G033.3848$-00.5971$&33.38476&$ -0.59713$&5.7&0.27&0.09&0.47&0.09&...&...\\ 
G033.3883$+00.8601$&33.38830&$ +0.86006$&5.0&0.16&0.06&0.31&0.06&...&...\\ 
G033.3934$+00.2539$&33.39338&$ +0.25385$&5.4&0.23&0.08&0.40&0.08&...&...\\ 
G033.4006$-00.8835$&33.40059&$ -0.88355$&6.5&0.27&0.07&0.42&0.07&...&...\\ 
G033.4046$-00.0043$&33.40463&$ -0.00434$&5.7&0.32&0.11&0.61&0.12&...&...\\ 
G033.4162$+00.5787$&33.41622&$ +0.57865$&5.0&0.18&0.07&0.32&0.07&...&...\\ 
G033.4172$-00.0037$&33.41720&$ -0.00372$&5.0&0.32&0.11&0.55&0.11&HII&G033.418-00.004\\ 
G033.4211$-00.9890$&33.42107&$ -0.98905$&5.0&0.22&0.08&0.38&0.08&...&...\\ 
G033.4215$+00.5347$&33.42150&$ +0.53469$&6.9&0.25&0.06&0.44&0.07&...&...\\ 
G033.4282$+00.6684$&33.42816&$ +0.66838$&5.3&0.20&0.07&0.39&0.08&...&...\\ 
G033.4291$+00.0171$&33.42914&$ +0.01711$&6.3&0.32&0.10&0.58&0.10&...&...\\ 
G033.4307$-00.2234$&33.43074&$ -0.22337$&5.2&0.19&0.06&0.32&0.06&...&...\\ 
G033.4363$+00.7726$&33.43629&$ +0.77262$&5.2&0.15&0.07&0.34&0.07&...&...\\ 
G033.4429$-00.1933$&33.44289&$ -0.19330$&5.0&0.18&0.06&0.31&0.07&...&...\\ 
G033.4444$-00.5932$&33.44442&$ -0.59317$&5.3&0.25&0.08&0.44&0.09&...&...\\ 
G033.4661$-00.3523$&33.46609&$ -0.35226$&5.2&0.18&0.06&0.32&0.07&...&...\\ 
G033.4662$-00.8065$&33.46622&$ -0.80652$&5.3&0.16&0.07&0.36&0.07&...&...\\ 
G033.4693$-00.1447$&33.46928&$ -0.14469$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G033.4729$-00.9054$&33.47289&$ -0.90535$&5.5&0.17&0.06&0.34&0.07&...&...\\ 
G033.4746$-00.3600$&33.47456&$ -0.36004$&6.9&0.28&0.07&0.48&0.08&Rad&G033.474-00.360\\ 
G033.4893$+00.8992$&33.48928&$ +0.89916$&5.0&0.17&0.07&0.33&0.07&...&...\\ 
G033.4919$-00.9386$&33.49192&$ -0.93855$&5.5&0.20&0.07&0.35&0.07&...&...\\ 
G033.4957$+00.9083$&33.49567&$ +0.90826$&5.4&0.20&0.07&0.35&0.07&...&...\\ 
G033.4966$-00.8601$&33.49657&$ -0.86014$&5.0&0.17&0.07&0.33&0.07&...&...\\ 
G033.4971$-00.8405$&33.49713&$ -0.84049$&5.0&0.20&0.07&0.35&0.07&...&...\\ 
G033.5016$+00.4934$&33.50164&$ +0.49344$&5.1&0.19&0.07&0.34&0.07&...&...\\ 
G033.5025$+00.1182$&33.50247&$ +0.11823$&5.2&0.32&0.10&0.50&0.10&...&...\\ 
G033.5050$-00.2702$&33.50504&$ -0.27018$&5.2&0.14&0.06&0.30&0.06&...&...\\ 
G033.5134$-00.3709$&33.51345&$ -0.37094$&5.2&0.18&0.07&0.34&0.07&...&...\\ 
G033.5148$-00.7706$&33.51484&$ -0.77062$&5.2&0.28&0.07&0.36&0.07&...&...\\ 
G033.5203$-00.8144$&33.52032&$ -0.81444$&5.2&0.23&0.08&0.38&0.08&...&...\\ 
G033.5259$-00.6298$&33.52588&$ -0.62984$&5.2&0.26&0.08&0.41&0.08&...&...\\ 
G033.5286$-00.6323$&33.52859&$ -0.63227$&6.8&0.28&0.08&0.53&0.09&...&...\\ 
G033.5326$+00.9094$&33.53262&$ +0.90944$&5.2&0.19&0.07&0.33&0.07&...&...\\ 
G033.5446$+00.5262$&33.54456&$ +0.52622$&5.5&0.19&0.07&0.35&0.07&...&...\\ 
G033.5448$-00.0049$&33.54477&$ -0.00490$&5.2&0.17&0.06&0.32&0.07&...&...\\ 
G033.5495$-00.1825$&33.54949&$ -0.18254$&6.5&0.21&0.06&0.41&0.07&...&...\\ 
G033.5536$+00.7908$&33.55359&$ +0.79082$&5.1&0.17&0.06&0.31&0.06&...&...\\ 
G033.5555$+00.8177$&33.55547&$ +0.81770$&6.6&0.23&0.07&0.42&0.07&...&...\\ 
G033.5598$-00.5103$&33.55977&$ -0.51032$&5.0&0.20&0.07&0.33&0.07&...&...\\ 
G033.5645$+00.3166$&33.56449&$ +0.31663$&5.1&0.25&0.08&0.39&0.08&...&...\\ 
G033.5680$-00.8976$&33.56797&$ -0.89765$&5.3&0.15&0.06&0.30&0.06&...&...\\ 
G033.5703$-00.4323$&33.57032&$ -0.43233$&5.2&0.21&0.07&0.35&0.07&...&...\\ 
G033.5794$+00.3841$&33.57935&$ +0.38406$&5.6&0.18&0.07&0.37&0.07&...&...\\ 
G033.5873$+00.8092$&33.58734&$ +0.80915$&5.4&0.18&0.06&0.33&0.06&...&...\\ 
G033.5990$+00.7949$&33.59901&$ +0.79492$&5.0&0.16&0.06&0.31&0.06&---&G033.600+00.794\\ 
G033.6015$-00.3021$&33.60150&$ -0.30205$&5.2&0.15&0.06&0.30&0.06&...&...\\ 
G033.6146$-00.1197$&33.61463&$ -0.11969$&5.3&0.19&0.06&0.34&0.07&...&...\\ 
G033.6246$+00.3073$&33.62456&$ +0.30725$&5.0&0.18&0.08&0.38&0.08&...&...\\ 
G033.6259$-00.3114$&33.62595&$ -0.31143$&5.0&0.16&0.06&0.31&0.07&...&...\\ 
G033.6316$+00.5728$&33.63165&$ +0.57282$&5.3&0.19&0.06&0.32&0.06&...&...\\ 
G033.6380$+00.6139$&33.63804&$ +0.61393$&5.0&0.14&0.06&0.29&0.06&...&...\\ 
G033.6385$-00.8116$&33.63846&$ -0.81159$&5.3&0.17&0.07&0.34&0.07&...&...\\ 
G033.6505$-00.1687$&33.65053&$ -0.16872$&5.0&0.17&0.07&0.33&0.07&...&...\\ 
G033.6557$-00.7563$&33.65568&$ -0.75631$&5.4&0.22&0.07&0.36&0.07&...&...\\ 
G033.6604$-00.2877$&33.66039&$ -0.28775$&5.1&0.20&0.07&0.34&0.07&...&...\\ 
G033.6606$-00.5853$&33.66061&$ -0.58526$&5.0&0.17&0.07&0.34&0.07&...&...\\ 
G033.6674$-01.0122$&33.66743&$ -1.01224$&5.0&0.27&0.10&0.51&0.11&...&...\\ 
G033.6813$+00.3402$&33.68130&$ +0.34017$&5.0&0.18&0.06&0.30&0.06&...&...\\ 
G033.6977$-00.2509$&33.69769&$ -0.25094$&5.4&0.20&0.07&0.35&0.07&...&...\\ 
G033.7137$-00.9877$&33.71369&$ -0.98773$&5.2&0.20&0.08&0.38&0.08&...&...\\ 
G033.7270$-00.6336$&33.72700&$ -0.63359$&5.3&0.21&0.07&0.36&0.07&...&...\\ 
G033.7298$-00.0550$&33.72984&$ -0.05504$&5.1&0.16&0.06&0.30&0.06&...&...\\ 
G033.7311$-00.8487$&33.73111&$ -0.84868$&5.0&0.20&0.06&0.31&0.06&...&...\\ 
G033.7319$+00.2825$&33.73185&$ +0.28246$&5.7&0.19&0.07&0.36&0.07&...&...\\ 
G033.7328$+00.4584$&33.73276&$ +0.45837$&5.5&0.16&0.06&0.32&0.06&...&...\\ 
G033.7437$+00.4493$&33.74373&$ +0.44934$&5.6&0.17&0.06&0.34&0.06&...&...\\ 
G033.7570$-00.5407$&33.75700&$ -0.54074$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G033.7638$+00.7319$&33.76382&$ +0.73193$&5.2&0.15&0.06&0.29&0.06&...&...\\ 
G033.7659$-00.4288$&33.76589&$ -0.42879$&6.6&0.21&0.06&0.41&0.07&...&...\\ 
G033.7661$+00.9599$&33.76612&$ +0.95994$&5.5&0.21&0.07&0.36&0.07&...&...\\ 
G033.7750$-00.4681$&33.77499&$ -0.46810$&5.4&0.20&0.07&0.36&0.07&...&...\\ 
G033.7827$+00.8566$&33.78272&$ +0.85659$&5.1&0.16&0.06&0.30&0.06&...&...\\ 
G033.7898$-00.1502$&33.78984&$ -0.15025$&5.3&0.21&0.07&0.35&0.07&...&...\\ 
G033.7955$+00.4326$&33.79554&$ +0.43260$&5.5&0.25&0.08&0.40&0.08&...&...\\ 
G033.7959$-00.2418$&33.79588&$ -0.24178$&5.2&0.21&0.07&0.36&0.07&sg?&...\\ 
G033.7966$+00.0036$&33.79657&$ +0.00364$&5.1&0.21&0.06&0.32&0.07&...&...\\ 
G033.8080$-00.1865$&33.80796&$ -0.18650$&5.2&0.45&0.12&0.59&0.12&Rad&G033.810-00.188(F)\\ 
G033.8084$+00.5277$&33.80839&$ +0.52775$&5.2&0.16&0.06&0.32&0.06&...&...\\ 
G033.8235$-00.5591$&33.82346&$ -0.55914$&5.4&0.22&0.07&0.38&0.07&...&...\\ 
G033.8416$+00.2589$&33.84158&$ +0.25892$&5.0&0.18&0.07&0.32&0.07&...&...\\ 
G033.8513$+00.0642$&33.85130&$ +0.06420$&6.2&0.30&0.08&0.47&0.08&...&...\\ 
G033.8517$-00.7219$&33.85174&$ -0.72186$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G033.8660$-00.6095$&33.86604&$ -0.60949$&5.2&0.21&0.07&0.34&0.07&...&...\\ 
G033.8738$-00.0506$&33.87380&$ -0.05059$&6.4&0.27&0.07&0.43&0.07&...&...\\ 
G033.8798$+00.6223$&33.87979&$ +0.62227$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G033.8803$+00.7213$&33.88029&$ +0.72130$&5.2&0.19&0.06&0.32&0.06&...&...\\ 
G033.8825$-00.0191$&33.88255&$ -0.01907$&6.1&0.22&0.07&0.41&0.07&...&...\\ 
G033.8854$-00.5976$&33.88542&$ -0.59762$&5.3&0.19&0.06&0.32&0.07&...&...\\ 
G033.8942$+00.6824$&33.89417&$ +0.68241$&5.0&0.15&0.06&0.30&0.06&...&...\\ 
G033.9150$+00.8253$&33.91502&$ +0.82534$&5.6&0.18&0.06&0.33&0.06&...&...\\ 
G033.9156$+00.6621$&33.91563&$ +0.66206$&5.0&0.19&0.06&0.32&0.07&...&...\\ 
G033.9251$-00.4425$&33.92513&$ -0.44247$&5.9&0.18&0.07&0.38&0.07&...&...\\ 
G033.9275$+01.0009$&33.92747&$ +1.00091$&5.3&0.24&0.10&0.50&0.10&...&...\\ 
G033.9484$+00.6669$&33.94841&$ +0.66685$&5.0&0.17&0.07&0.34&0.07&...&...\\ 
G033.9501$-00.6474$&33.95008&$ -0.64741$&5.0&0.20&0.07&0.33&0.07&...&...\\ 
G033.9616$+00.4329$&33.96159&$ +0.43288$&5.1&0.20&0.07&0.34&0.07&...&...\\ 
G033.9738$+00.6989$&33.97384&$ +0.69894$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G033.9739$-00.8574$&33.97385&$ -0.85743$&5.2&0.18&0.07&0.34&0.07&...&...\\ 
G033.9830$+00.0484$&33.98304&$ +0.04836$&5.0&0.21&0.07&0.33&0.07&...&...\\ 
G033.9846$-00.7755$&33.98461&$ -0.77548$&5.2&0.19&0.07&0.36&0.07&...&...\\ 
G033.9937$+00.2192$&33.99373&$ +0.21920$&5.5&0.20&0.07&0.38&0.07&...&...\\ 
G033.9962$-00.9779$&33.99623&$ -0.97786$&5.1&0.17&0.08&0.41&0.08&---&G033.996-00.978\\ 
G034.0015$+00.3436$&34.00149&$ +0.34357$&5.5&0.21&0.07&0.36&0.07&...&...\\ 
G034.0055$+00.9754$&34.00545&$ +0.97542$&5.2&0.20&0.07&0.36&0.07&...&...\\ 
G034.0108$+00.5733$&34.01085&$ +0.57330$&5.2&0.18&0.07&0.37&0.07&...&...\\ 
G034.0150$+00.4651$&34.01502&$ +0.46511$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G034.0185$-00.1434$&34.01851&$ -0.14344$&6.1&0.19&0.06&0.38&0.07&...&...\\ 
G034.0333$-00.5525$&34.03328&$ -0.55248$&5.9&0.20&0.07&0.39&0.07&...&...\\ 
G034.0343$-00.1534$&34.03434&$ -0.15344$&6.3&0.26&0.07&0.42&0.07&...&...\\ 
G034.0369$-00.1752$&34.03691&$ -0.17518$&5.8&0.23&0.06&0.36&0.07&---&G034.037-00.176(I)\\ 
G034.0393$+00.3473$&34.03934&$ +0.34732$&5.5&0.20&0.07&0.37&0.07&...&...\\ 
G034.0448$+00.2302$&34.04476&$ +0.23017$&5.3&0.19&0.07&0.34&0.07&...&...\\ 
G034.0650$-00.1136$&34.06504&$ -0.11358$&5.0&0.18&0.07&0.32&0.07&...&...\\ 
G034.0739$-00.1863$&34.07393&$ -0.18629$&5.2&0.18&0.07&0.33&0.07&...&...\\ 
G034.0750$-00.0102$&34.07504&$ -0.01025$&5.2&0.19&0.07&0.34&0.07&...&...\\ 
G034.0768$+00.1728$&34.07677&$ +0.17281$&5.0&0.24&0.07&0.34&0.07&...&...\\ 
G034.0776$-00.9731$&34.07762&$ -0.97307$&5.0&0.20&0.07&0.35&0.07&...&...\\ 
G034.0793$-00.6913$&34.07932&$ -0.69131$&6.9&0.36&0.07&0.45&0.07&---&G034.079-00.691(I)\\ 
G034.0797$-00.6919$&34.07973&$ -0.69193$&6.4&0.26&0.07&0.41&0.07&...&...\\ 
G034.0803$+00.5258$&34.08030&$ +0.52580$&5.1&0.18&0.07&0.35&0.07&...&...\\ 
G034.0819$-00.5116$&34.08190&$ -0.51157$&5.1&0.16&0.07&0.32&0.07&...&...\\ 
G034.0848$+00.0786$&34.08476&$ +0.07857$&5.1&0.22&0.07&0.33&0.07&...&...\\ 
G034.0850$+00.2541$&34.08497&$ +0.25406$&5.0&0.17&0.06&0.31&0.07&...&...\\ 
G034.0864$+00.9895$&34.08644&$ +0.98952$&5.1&0.24&0.09&0.43&0.09&...&...\\ 
G034.0865$+00.5274$&34.08648&$ +0.52740$&5.0&0.20&0.07&0.34&0.07&...&...\\ 
G034.1072$-00.3568$&34.10719&$ -0.35678$&5.0&0.19&0.07&0.32&0.07&...&...\\ 
G034.1141$+00.7877$&34.11410&$ +0.78769$&5.0&0.17&0.07&0.32&0.07&...&...\\ 
G034.1146$-00.8372$&34.11458&$ -0.83722$&5.1&0.19&0.06&0.32&0.06&...&...\\ 
G034.1216$+00.0239$&34.12164&$ +0.02392$&5.8&0.21&0.07&0.39&0.07&...&...\\ 
G034.1231$-00.7285$&34.12307&$ -0.72846$&5.2&0.17&0.06&0.33&0.07&...&...\\ 
G034.1303$-00.0172$&34.13032&$ -0.01719$&5.0&0.17&0.07&0.33&0.07&...&...\\ 
G034.1563$-00.3732$&34.15628&$ -0.37324$&5.2&0.20&0.06&0.33&0.07&...&...\\ 
G034.1617$-00.0431$&34.16171&$ -0.04309$&5.2&0.21&0.07&0.34&0.07&...&...\\ 
G034.1665$+00.9786$&34.16652&$ +0.97862$&6.7&0.23&0.07&0.46&0.07&...&...\\ 
G034.1682$-00.3857$&34.16823&$ -0.38574$&5.5&0.21&0.06&0.34&0.07&...&...\\ 
G034.1719$-00.4592$&34.17191&$ -0.45921$&6.5&0.23&0.06&0.40&0.07&...&...\\ 
G034.1726$-00.6521$&34.17259&$ -0.65214$&5.3&0.20&0.07&0.35&0.07&...&...\\ 
G034.1842$-00.6370$&34.18419&$ -0.63700$&5.0&0.20&0.07&0.33&0.07&...&...\\ 
G034.1850$-00.6867$&34.18502&$ -0.68665$&6.2&0.20&0.07&0.39&0.07&---&G034.185-00.687\\ 
G034.1876$-00.9422$&34.18757&$ -0.94216$&5.1&0.19&0.07&0.33&0.07&...&...\\ 
G034.1943$+00.3336$&34.19427&$ +0.33364$&5.4&0.22&0.07&0.37&0.07&...&...\\ 
G034.2033$+00.3669$&34.20330&$ +0.36691$&6.2&0.21&0.07&0.41&0.07&...&...\\ 
G034.2105$-00.2402$&34.21046&$ -0.24025$&5.2&0.17&0.06&0.33&0.07&...&...\\ 
G034.2132$-00.1863$&34.21317&$ -0.18629$&5.8&0.18&0.06&0.36&0.07&...&...\\ 
G034.2193$-00.0228$&34.21935&$ -0.02282$&5.2&0.18&0.06&0.33&0.07&...&...\\ 
G034.2250$+00.7971$&34.22502&$ +0.79714$&5.0&0.17&0.07&0.33&0.07&...&...\\ 
G034.2273$-00.4351$&34.22726&$ -0.43511$&5.0&0.18&0.06&0.31&0.06&...&...\\ 
G034.2334$-00.3548$&34.23337&$ -0.35483$&5.3&0.19&0.06&0.33&0.07&...&...\\ 
G034.2356$+00.2966$&34.23560&$ +0.29663$&7.0&0.28&0.07&0.50&0.08&...&...\\ 
G034.2397$-00.6973$&34.23975&$ -0.69735$&5.2&0.16&0.06&0.31&0.06&...&...\\ 
G034.2670$-00.2847$&34.26699&$ -0.28469$&5.5&0.19&0.06&0.34&0.07&...&...\\ 
G034.2707$-00.8149$&34.27072&$ -0.81493$&5.3&0.17&0.06&0.33&0.07&...&...\\ 
G034.2719$-00.8432$&34.27189&$ -0.84319$&5.4&0.19&0.06&0.33&0.06&...&...\\ 
G034.2896$-00.2595$&34.28963&$ -0.25948$&5.6&0.19&0.06&0.33&0.06&...&...\\ 
G034.2915$-00.8652$&34.29155&$ -0.86521$&6.8&0.23&0.07&0.45&0.07&...&...\\ 
G034.2922$-00.8935$&34.29217&$ -0.89348$&5.2&0.20&0.06&0.32&0.07&...&...\\ 
G034.2934$+00.4201$&34.29344&$ +0.42010$&5.3&0.18&0.07&0.35&0.07&...&...\\ 
G034.2974$-00.7452$&34.29739&$ -0.74520$&5.2&0.21&0.06&0.33&0.07&...&...\\ 
G034.3004$+00.0697$&34.30039&$ +0.06968$&5.8&0.63&0.14&0.77&0.14&...&...\\ 
G034.3012$+00.0695$&34.30122&$ +0.06954$&5.0&0.63&0.14&0.67&0.14&...&...\\ 
G034.3094$-00.8887$&34.30940&$ -0.88869$&5.0&0.19&0.07&0.32&0.07&...&...\\ 
G034.3163$+00.9301$&34.31634&$ +0.93014$&5.2&0.19&0.06&0.31&0.06&...&...\\ 
G034.3194$-00.6087$&34.31941&$ -0.60866$&5.0&0.19&0.07&0.34&0.07&...&...\\ 
G034.3218$+00.8461$&34.32183&$ +0.84610$&5.1&0.20&0.07&0.37&0.08&...&...\\ 
G034.3243$+00.8545$&34.32433&$ +0.85451$&6.3&0.23&0.07&0.42&0.07&...&...\\ 
G034.3325$-00.7451$&34.33246&$ -0.74506$&5.2&0.18&0.06&0.33&0.07&...&...\\ 
G034.3326$+00.0166$&34.33261&$ +0.01656$&5.5&0.24&0.06&0.34&0.07&...&...\\ 
G034.3348$+00.5383$&34.33483&$ +0.53830$&5.0&0.19&0.06&0.32&0.07&...&...\\ 
G034.3378$+00.5396$&34.33781&$ +0.53962$&5.0&0.19&0.06&0.32&0.07&...&...\\ 
G034.3502$-00.2179$&34.35018&$ -0.21789$&5.3&0.19&0.06&0.33&0.07&...&...\\ 
G034.3521$-00.1258$&34.35213&$ -0.12580$&5.5&0.21&0.06&0.33&0.06&...&...\\ 
G034.3575$-00.9815$&34.35752&$ -0.98155$&5.4&0.25&0.08&0.42&0.08&...&...\\ 
G034.3621$-00.0506$&34.36206&$ -0.05059$&5.1&0.17&0.06&0.31&0.06&...&...\\ 
G034.3698$-00.4168$&34.36976&$ -0.41678$&5.0&0.19&0.07&0.34&0.07&...&...\\ 
G034.3698$-00.3037$&34.36983&$ -0.30372$&5.6&0.19&0.07&0.35&0.07&...&...\\ 
G034.3864$-00.6818$&34.38636&$ -0.68179$&5.4&0.19&0.07&0.35&0.07&...&...\\ 
G034.3907$+00.0939$&34.39074&$ +0.09392$&5.1&0.25&0.07&0.37&0.08&...&...\\ 
G034.3946$+00.5085$&34.39455&$ +0.50851$&5.8&0.20&0.07&0.38&0.07&...&...\\ 
G034.4060$+01.0170$&34.40600&$ +1.01703$&5.0&0.24&0.10&0.52&0.11&...&...\\ 
G034.4113$+00.2349$&34.41129&$ +0.23489$&5.9&0.20&0.07&0.41&0.08&cor&...\\ 
G034.4124$-00.4915$&34.41240&$ -0.49150$&5.9&0.18&0.07&0.38&0.07&...&...\\ 
G034.4185$-00.7499$&34.41851&$ -0.74992$&5.5&0.17&0.06&0.33&0.06&...&...\\ 
G034.4240$-00.9988$&34.42399&$ -0.99877$&5.4&0.36&0.10&0.53&0.10&...&...\\ 
G034.4393$-00.0573$&34.43935&$ -0.05733$&6.3&0.22&0.06&0.40&0.07&...&...\\ 
G034.4407$-00.7665$&34.44073&$ -0.76645$&5.2&0.16&0.06&0.32&0.07&...&...\\ 
G034.4409$-00.1556$&34.44095&$ -0.15559$&5.4&0.22&0.07&0.36&0.07&...&...\\ 
G034.4418$+00.0936$&34.44178&$ +0.09357$&5.1&0.19&0.06&0.33&0.07&...&...\\ 
G034.4480$+00.8358$&34.44802&$ +0.83575$&5.2&0.20&0.07&0.34&0.07&...&...\\ 
G034.4544$+00.7713$&34.45442&$ +0.77130$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G034.4596$-00.4217$&34.45963&$ -0.42171$&6.2&0.24&0.07&0.42&0.07&...&...\\ 
G034.4701$-00.7888$&34.47011&$ -0.78881$&5.1&0.21&0.07&0.32&0.07&...&...\\ 
G034.4729$-00.4252$&34.47289&$ -0.42518$&5.7&0.23&0.07&0.40&0.07&...&...\\ 
G034.4739$-00.6171$&34.47393&$ -0.61713$&5.2&0.20&0.07&0.35&0.07&...&...\\ 
G034.4793$+00.7442$&34.47928&$ +0.74422$&5.3&0.17&0.06&0.30&0.06&...&...\\ 
G034.4875$-00.6143$&34.48747&$ -0.61429$&5.3&0.18&0.07&0.35&0.07&...&...\\ 
G034.4903$+00.0144$&34.49032&$ +0.01441$&5.1&0.19&0.06&0.32&0.06&...&...\\ 
G034.4968$-00.5860$&34.49678&$ -0.58602$&5.0&0.17&0.07&0.35&0.07&...&...\\ 
G034.4988$+00.1065$&34.49879&$ +0.10649$&5.3&0.19&0.06&0.34&0.07&...&...\\ 
G034.4996$+00.1779$&34.49963&$ +0.17788$&5.6&0.15&0.06&0.34&0.06&...&...\\ 
G034.5040$+00.9259$&34.50400&$ +0.92590$&5.4&0.20&0.07&0.37&0.07&...&...\\ 
G034.5197$-00.6254$&34.51970&$ -0.62540$&6.0&0.23&0.07&0.44&0.08&...&...\\ 
G034.5223$-00.3998$&34.52227&$ -0.39976$&5.2&0.18&0.07&0.36&0.07&...&...\\ 
G034.5223$+00.3421$&34.52234&$ +0.34212$&6.2&0.21&0.06&0.38&0.07&...&...\\ 
G034.5236$+00.4499$&34.52359&$ +0.44990$&5.1&0.17&0.06&0.31&0.06&...&...\\ 
G034.5424$-00.3822$&34.54241&$ -0.38219$&5.2&0.19&0.07&0.34&0.07&...&...\\ 
G034.5435$-00.7310$&34.54352&$ -0.73103$&5.0&0.17&0.07&0.34&0.07&...&...\\ 
G034.5494$-00.3296$&34.54935&$ -0.32955$&5.1&0.18&0.07&0.34&0.07&...&...\\ 
G034.5520$-00.5323$&34.55199&$ -0.53227$&5.1&0.21&0.07&0.36&0.07&...&...\\ 
G034.5542$+00.4250$&34.55421&$ +0.42496$&5.1&0.15&0.06&0.30&0.06&...&...\\ 
G034.5549$-00.1841$&34.55491&$ -0.18407$&5.1&0.26&0.07&0.35&0.07&...&...\\ 
G034.5550$-00.4854$&34.55505&$ -0.48539$&5.9&0.23&0.08&0.43&0.08&...&...\\ 
G034.5572$+00.4234$&34.55720&$ +0.42344$&5.0&0.18&0.06&0.30&0.06&...&...\\ 
G034.5575$+00.5235$&34.55755&$ +0.52351$&5.0&0.16&0.06&0.30&0.06&...&...\\ 
G034.5603$+00.3371$&34.56032&$ +0.33712$&6.8&0.23&0.06&0.41&0.07&...&...\\ 
G034.5638$-00.5580$&34.56380&$ -0.55803$&5.0&0.19&0.07&0.35&0.07&...&...\\ 
G034.5705$+00.0587$&34.57046&$ +0.05871$&5.2&0.19&0.06&0.32&0.07&...&...\\ 
G034.5772$+00.3755$&34.57720&$ +0.37552$&5.1&0.18&0.06&0.31&0.06&...&...\\ 
G034.5838$+00.7442$&34.58380&$ +0.74422$&5.8&0.18&0.06&0.32&0.06&...&...\\ 
G034.5857$+00.1803$&34.58574&$ +0.18031$&5.0&0.17&0.07&0.32&0.07&...&...\\ 
G034.5862$-00.6216$&34.58616&$ -0.62165$&5.1&0.18&0.07&0.35&0.07&...&...\\ 
G034.5892$-00.4157$&34.58921&$ -0.41567$&6.0&0.22&0.07&0.42&0.07&...&...\\ 
G034.5898$+00.2295$&34.58984&$ +0.22948$&5.1&0.17&0.06&0.31&0.06&...&...\\ 
G034.5912$+00.2252$&34.59116&$ +0.22524$&5.3&0.17&0.06&0.32&0.06&...&...\\ 
G034.5926$+00.2437$&34.59261&$ +0.24371$&6.1&0.95&0.09&0.46&0.07&smm&G034.592+00.244\\ 
G034.5936$+00.4262$&34.59359&$ +0.42622$&6.0&0.23&0.06&0.36&0.06&...&...\\ 
G034.5999$-01.0068$&34.59992&$ -1.00683$&6.7&0.39&0.10&0.63&0.10&...&...\\ 
G034.6109$-00.0068$&34.61088&$ -0.00677$&5.1&0.22&0.07&0.33&0.07&...&...\\ 
G034.6110$+00.7905$&34.61096&$ +0.79054$&5.0&0.16&0.06&0.30&0.06&...&...\\ 
G034.6120$+00.9711$&34.61201&$ +0.97112$&5.1&0.17&0.07&0.35&0.07&...&...\\ 
G034.6356$-00.0984$&34.63560&$ -0.09837$&5.3&0.20&0.07&0.36&0.07&...&...\\ 
G034.6471$-00.4562$&34.64706&$ -0.45622$&5.4&0.22&0.07&0.38&0.07&...&...\\ 
G034.6475$+00.7161$&34.64749&$ +0.71609$&5.2&0.19&0.06&0.31&0.06&...&...\\ 
G034.6514$+00.7199$&34.65145&$ +0.71991$&5.1&0.18&0.06&0.32&0.06&...&...\\ 
G034.6596$+00.8067$&34.65957&$ +0.80672$&5.5&0.20&0.06&0.34&0.07&...&...\\ 
G034.6609$+00.8039$&34.66089&$ +0.80388$&5.1&0.19&0.06&0.32&0.06&...&...\\ 
G034.6721$+00.1673$&34.67213&$ +0.16732$&5.2&0.19&0.06&0.32&0.06&...&...\\ 
G034.6725$-00.6599$&34.67249&$ -0.65991$&5.2&0.18&0.07&0.35&0.07&...&...\\ 
G034.6837$+00.8862$&34.68375&$ +0.88625$&5.6&0.21&0.06&0.34&0.06&...&...\\ 
G034.6884$-00.0271$&34.68845&$ -0.02705$&5.6&0.30&0.07&0.38&0.07&...&...\\ 
G034.6908$+00.9122$&34.69083&$ +0.91222$&5.3&0.15&0.06&0.31&0.06&...&...\\ 
G034.6913$-00.8011$&34.69131&$ -0.80111$&5.1&0.16&0.06&0.30&0.06&...&...\\ 
G034.6930$-00.2670$&34.69296&$ -0.26698$&5.1&0.22&0.07&0.35&0.07&...&...\\ 
G034.7002$+00.6519$&34.70020&$ +0.65185$&5.8&0.21&0.06&0.35&0.06&...&...\\ 
G034.7037$+00.5714$&34.70367&$ +0.57143$&5.5&0.16&0.06&0.33&0.06&...&...\\ 
G034.7046$-00.3714$&34.70463&$ -0.37136$&6.9&0.29&0.07&0.47&0.08&...&...\\ 
G034.7065$-00.9988$&34.70647&$ -0.99884$&5.0&0.24&0.09&0.44&0.09&...&...\\ 
G034.7134$-00.0237$&34.71345&$ -0.02372$&5.0&0.19&0.07&0.33&0.07&...&...\\ 
G034.7158$-00.7583$&34.71583&$ -0.75832$&5.2&0.17&0.06&0.32&0.06&...&...\\ 
G034.7214$-00.6764$&34.72138&$ -0.67637$&5.1&0.20&0.07&0.35&0.07&...&...\\ 
G034.7349$+00.1866$&34.73491&$ +0.18656$&5.3&0.16&0.07&0.35&0.07&...&...\\ 
G034.7441$+00.3466$&34.74415&$ +0.34656$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G034.7489$-00.3014$&34.74887&$ -0.30136$&5.2&0.20&0.07&0.37&0.08&...&...\\ 
G034.7569$+00.3555$&34.75686&$ +0.35552$&5.4&0.22&0.07&0.35&0.07&...&...\\ 
G034.7621$+00.6253$&34.76207&$ +0.62532$&5.5&0.17&0.06&0.33&0.06&...&...\\ 
G034.7648$+00.4436$&34.76484&$ +0.44358$&5.1&0.21&0.06&0.32&0.06&...&...\\ 
G034.7902$+00.0971$&34.79018&$ +0.09711$&5.1&0.19&0.07&0.35&0.07&...&...\\ 
G034.7962$+00.5452$&34.79617&$ +0.54525$&5.6&0.20&0.06&0.35&0.07&---&G034.796+00.545\\ 
G034.7994$+00.5216$&34.79943&$ +0.52163$&5.1&0.17&0.06&0.30&0.06&...&...\\ 
G034.8010$-00.6633$&34.80104&$ -0.66332$&5.1&0.19&0.07&0.34&0.07&...&...\\ 
G034.8012$+00.4207$&34.80116&$ +0.42073$&5.4&0.18&0.07&0.34&0.07&...&...\\ 
G034.8054$-00.2714$&34.80540&$ -0.27136$&6.1&0.23&0.07&0.44&0.08&...&...\\ 
G034.8054$-00.7192$&34.80542&$ -0.71922$&5.1&0.20&0.07&0.34&0.07&...&...\\ 
G034.8113$-00.4882$&34.81131&$ -0.48817$&5.2&0.24&0.08&0.38&0.08&...&...\\ 
G034.8201$+00.2257$&34.82012&$ +0.22566$&6.0&0.21&0.07&0.40&0.07&...&...\\ 
G034.8305$-00.8297$&34.83050&$ -0.82972$&5.1&0.17&0.06&0.32&0.06&...&...\\ 
G034.8320$-00.1861$&34.83199&$ -0.18608$&5.2&0.18&0.07&0.35&0.07&...&...\\ 
G034.8324$+00.6852$&34.83236&$ +0.68519$&6.3&0.26&0.06&0.39&0.07&---&G034.832+00.685\\ 
G034.8360$+00.9824$&34.83600&$ +0.98237$&5.7&0.23&0.08&0.42&0.08&...&...\\ 
G034.8368$-00.3573$&34.83679&$ -0.35733$&5.1&0.17&0.07&0.34&0.07&...&...\\ 
G034.8378$+01.0047$&34.83781&$ +1.00473$&5.9&0.47&0.11&0.59&0.11&...&...\\ 
G034.8410$+00.5031$&34.84103&$ +0.50309$&5.4&0.17&0.06&0.33&0.07&---&G034.842+00.503\\ 
G034.8425$-00.0780$&34.84248&$ -0.07796$&5.1&0.22&0.07&0.36&0.07&...&...\\ 
G034.8443$-00.9420$&34.84426&$ -0.94196$&5.4&0.20&0.06&0.33&0.07&...&...\\ 
G034.8508$-00.3571$&34.85082&$ -0.35712$&5.9&0.22&0.07&0.42&0.08&...&...\\ 
G034.8523$-00.7385$&34.85230&$ -0.73846$&6.3&0.19&0.06&0.39&0.07&...&...\\ 
G034.8660$+00.1205$&34.86595&$ +0.12052$&5.1&0.20&0.07&0.34&0.07&...&...\\ 
G034.8688$-00.1300$&34.86880&$ -0.12997$&5.1&0.20&0.07&0.36&0.07&...&...\\ 
G034.8693$+00.4439$&34.86929&$ +0.44392$&5.4&0.22&0.07&0.36&0.07&...&...\\ 
G034.8894$-00.7871$&34.88939&$ -0.78708$&5.2&0.17&0.06&0.31&0.06&...&...\\ 
G034.8971$-00.2195$&34.89713&$ -0.21948$&5.1&0.20&0.07&0.35&0.07&...&...\\ 
G034.8987$+00.7162$&34.89869&$ +0.71623$&6.7&0.22&0.07&0.43&0.07&...&...\\ 
G034.8988$-00.3086$&34.89880&$ -0.30858$&5.3&0.21&0.07&0.37&0.07&...&...\\ 
G034.8989$-00.1066$&34.89894&$ -0.10657$&5.4&0.23&0.07&0.37&0.07&...&...\\ 
G034.8994$-00.4868$&34.89944&$ -0.48678$&5.0&0.19&0.07&0.35&0.07&...&...\\ 
G034.9015$+00.1463$&34.90151&$ +0.14628$&5.2&0.18&0.07&0.35&0.07&...&...\\ 
G034.9041$-00.6812$&34.90410&$ -0.68124$&5.2&0.22&0.06&0.32&0.06&...&...\\ 
G034.9155$+00.0481$&34.91553&$ +0.04809$&5.4&0.19&0.07&0.35&0.07&...&...\\ 
G034.9188$-00.9379$&34.91878&$ -0.93786$&5.3&0.24&0.07&0.38&0.07&...&...\\ 
G034.9198$+00.8565$&34.91982&$ +0.85645$&6.6&0.26&0.07&0.45&0.07&...&...\\ 
G034.9234$+00.1806$&34.92338&$ +0.18059$&5.2&0.19&0.07&0.34&0.07&...&...\\ 
G034.9263$-00.8657$&34.92628&$ -0.86570$&5.2&0.17&0.07&0.35&0.07&...&...\\ 
G034.9264$-00.0005$&34.92637&$ -0.00052$&5.2&0.19&0.07&0.35&0.07&...&...\\ 
G034.9302$+00.8765$&34.93017&$ +0.87652$&5.3&0.20&0.07&0.35&0.07&...&...\\ 
G034.9309$-00.8540$&34.93086&$ -0.85396$&5.1&0.18&0.07&0.34&0.07&...&...\\ 
G034.9329$+00.8407$&34.93287&$ +0.84069$&6.0&0.23&0.07&0.40&0.07&---&G034.933+00.840\\ 
G034.9329$+00.2475$&34.93290&$ +0.24746$&6.7&0.24&0.07&0.45&0.07&...&...\\ 
G034.9362$+00.1831$&34.93616&$ +0.18309$&5.2&0.17&0.06&0.32&0.06&...&...\\ 
G034.9421$+00.5905$&34.94209&$ +0.59053$&5.0&0.18&0.06&0.32&0.07&...&...\\ 
G034.9470$+00.6714$&34.94702&$ +0.67137$&5.1&0.16&0.07&0.33&0.07&...&...\\ 
G034.9512$+00.4075$&34.95117&$ +0.40753$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G034.9530$+00.0007$&34.95297&$ +0.00066$&5.0&0.16&0.06&0.31&0.07&...&...\\ 
G034.9572$-00.3286$&34.95721&$ -0.32858$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G034.9592$+00.4376$&34.95923&$ +0.43760$&6.8&0.29&0.07&0.48&0.08&---&G034.959+00.438\\ 
G034.9623$+00.2837$&34.96235&$ +0.28371$&5.0&0.18&0.07&0.34&0.07&...&...\\ 
G034.9746$+00.3589$&34.97464&$ +0.35885$&5.1&0.21&0.07&0.37&0.08&...&...\\ 
G034.9863$-00.2293$&34.98630&$ -0.22934$&5.1&0.17&0.06&0.29&0.06&...&...\\ 
G034.9903$+00.2832$&34.99026&$ +0.28316$&5.1&0.22&0.07&0.36&0.07&...&...\\ 
G034.9908$+00.7411$&34.99079&$ +0.74109$&5.4&0.26&0.07&0.38&0.07&---&G034.990+00.741\\ 
G034.9940$-00.1296$&34.99401&$ -0.12962$&5.0&0.16&0.06&0.30&0.06&...&...\\ 
G035.0032$-00.0380$&35.00316&$ -0.03802$&5.8&0.18&0.06&0.35&0.06&...&...\\ 
G035.0060$+00.3968$&35.00600&$ +0.39684$&6.5&0.25&0.08&0.49&0.08&...&...\\ 
G035.0065$-00.0511$&35.00650&$ -0.05115$&5.3&0.18&0.06&0.33&0.06&...&...\\ 
G035.0366$+00.4327$&35.03655&$ +0.43274$&5.4&0.22&0.07&0.39&0.07&...&...\\ 
G035.0390$-00.0049$&35.03900&$ -0.00490$&5.1&0.19&0.06&0.31&0.06&...&...\\ 
G035.0513$-00.5178$&35.05134&$ -0.51775$&6.5&0.39&0.08&0.51&0.09&HII&G035.052-00.518(F)\\ 
G035.0540$+00.7732$&35.05396&$ +0.77325$&5.8&0.25&0.07&0.40&0.07&...&...\\ 
G035.0642$-00.6518$&35.06418&$ -0.65179$&5.4&0.23&0.06&0.34&0.07&...&...\\ 
G035.0678$+00.5049$&35.06780&$ +0.50490$&5.5&0.22&0.07&0.37&0.07&...&...\\ 
G035.0693$+00.4293$&35.06933&$ +0.42934$&5.5&0.20&0.07&0.39&0.07&...&...\\ 
G035.0817$+00.0070$&35.08171&$ +0.00704$&6.3&0.21&0.06&0.39&0.06&...&...\\ 
G035.0861$+00.9929$&35.08609&$ +0.99293$&5.4&0.24&0.08&0.43&0.08&---&G035.086+00.993\\ 
G035.0884$+00.0905$&35.08837&$ +0.09052$&5.3&0.18&0.06&0.32&0.06&...&...\\ 
G035.0916$-00.4030$&35.09163&$ -0.40296$&6.0&0.18&0.06&0.35&0.06&...&...\\ 
G035.1161$-00.4150$&35.11607&$ -0.41504$&5.0&0.17&0.06&0.30&0.06&...&...\\ 
G035.1185$+00.0043$&35.11851&$ +0.00427$&6.0&0.20&0.06&0.34&0.06&...&...\\ 
G035.1216$-00.2052$&35.12157&$ -0.20518$&5.1&0.18&0.06&0.30&0.06&...&...\\ 
G035.1234$+00.5252$&35.12336&$ +0.52518$&6.3&0.31&0.07&0.43&0.07&...&...\\ 
G035.1262$-00.2250$&35.12622&$ -0.22504$&5.3&0.19&0.06&0.31&0.06&...&...\\ 
G035.1277$+00.0873$&35.12775&$ +0.08732$&5.1&0.23&0.06&0.30&0.06&...&...\\ 
G035.1300$+00.5011$&35.12996&$ +0.50108$&5.0&0.22&0.07&0.33&0.07&...&...\\ 
G035.1318$-00.8501$&35.13181&$ -0.85014$&5.8&0.33&0.07&0.39&0.07&...&...\\ 
G035.1403$-00.1083$&35.14032&$ -0.10830$&6.5&0.21&0.06&0.37&0.06&...&...\\ 
G035.1449$-00.7559$&35.14487&$ -0.75589$&6.1&0.24&0.07&0.40&0.07&...&...\\ 
G035.1494$+00.9083$&35.14944&$ +0.90826$&5.0&0.21&0.07&0.35&0.07&...&...\\ 
G035.1625$+00.0907$&35.16254&$ +0.09073$&5.2&0.17&0.06&0.31&0.06&...&...\\ 
G035.1652$+00.2529$&35.16518&$ +0.25288$&5.3&0.19&0.06&0.34&0.07&...&...\\ 
G035.1662$+00.4909$&35.16621&$ +0.49087$&5.4&0.21&0.06&0.34&0.07&...&...\\ 
G035.1767$-00.5500$&35.17669&$ -0.54998$&5.1&0.18&0.06&0.31&0.06&...&...\\ 
G035.1772$+00.9139$&35.17722&$ +0.91389$&5.2&0.17&0.07&0.33&0.07&...&...\\ 
G035.1802$+00.8435$&35.18022&$ +0.84353$&5.0&0.19&0.07&0.33&0.07&...&...\\ 
G035.1875$+00.1372$&35.18754&$ +0.13718$&5.0&0.18&0.06&0.30&0.06&...&...\\ 
G035.1942$+01.0149$&35.19416&$ +1.01494$&5.5&0.33&0.12&0.65&0.12&...&...\\ 
G035.1968$-00.7422$&35.19675&$ -0.74221$&6.6&0.31&0.08&0.48&0.08&Rad&G035.197-00.743(I)\\ 
G035.1999$-00.8681$&35.19987&$ -0.86813$&5.2&0.19&0.06&0.32&0.06&...&...\\ 
G035.2027$-00.9852$&35.20271&$ -0.98516$&5.6&0.22&0.07&0.37&0.07&...&...\\ 
G035.2137$+00.9685$&35.21368&$ +0.96855$&5.2&0.20&0.07&0.37&0.08&...&...\\ 
G035.2158$+00.4287$&35.21580&$ +0.42872$&5.8&0.26&0.07&0.40&0.07&...&...\\ 
G035.2161$-00.3498$&35.21615&$ -0.34983$&5.0&0.19&0.06&0.30&0.06&...&...\\ 
G035.2164$+00.4281$&35.21642&$ +0.42809$&5.7&0.22&0.07&0.40&0.07&Rad&G035.216+00.428(I)\\ 
G035.2256$-00.9034$&35.22563&$ -0.90341$&5.2&0.18&0.07&0.33&0.07&...&...\\ 
G035.2360$-00.3866$&35.23601&$ -0.38657$&5.4&0.19&0.06&0.32&0.06&...&...\\ 
G035.2412$+00.6787$&35.24121&$ +0.67873$&7.0&0.23&0.07&0.45&0.07&...&...\\ 
G035.2450$-00.1521$&35.24497&$ -0.15212$&6.5&0.21&0.06&0.37&0.06&...&...\\ 
G035.2509$-00.5344$&35.25094&$ -0.53442$&5.1&0.15&0.06&0.30&0.06&...&...\\ 
G035.2574$+00.8326$&35.25738&$ +0.83263$&5.2&0.23&0.07&0.36&0.07&...&...\\ 
G035.2675$+00.7489$&35.26745&$ +0.74894$&7.0&0.27&0.07&0.46&0.07&...&...\\ 
G035.2779$-00.8173$&35.27787&$ -0.81729$&5.3&0.22&0.07&0.35&0.07&...&...\\ 
G035.2859$+00.6193$&35.28593&$ +0.61935$&5.2&0.19&0.07&0.32&0.07&...&...\\ 
G035.2873$-00.0360$&35.28734&$ -0.03601$&5.0&0.16&0.06&0.30&0.06&...&...\\ 
G035.2930$-00.3267$&35.29296&$ -0.32671$&5.0&0.20&0.06&0.30&0.06&...&...\\ 
G035.2935$-00.9020$&35.29349&$ -0.90202$&5.1&0.15&0.06&0.32&0.07&...&...\\ 
G035.3122$-00.4152$&35.31219&$ -0.41518$&5.1&0.16&0.06&0.30&0.06&...&...\\ 
G035.3132$-00.3778$&35.31316&$ -0.37782$&5.2&0.15&0.06&0.31&0.06&...&...\\ 
G035.3174$-00.1600$&35.31740&$ -0.16004$&5.2&0.17&0.06&0.30&0.06&...&...\\ 
G035.3183$-00.9868$&35.31828&$ -0.98682$&5.6&0.23&0.07&0.40&0.08&...&...\\ 
G035.3373$+00.3383$&35.33733&$ +0.33830$&5.2&0.23&0.10&0.50&0.10&...&...\\ 
G035.3429$+00.7561$&35.34295&$ +0.75609$&6.7&0.21&0.07&0.43&0.07&...&...\\ 
G035.3455$-00.2473$&35.34553&$ -0.24733$&6.6&0.23&0.07&0.43&0.07&...&...\\ 
G035.3564$-00.9057$&35.35642&$ -0.90570$&5.7&0.18&0.07&0.37&0.07&...&...\\ 
G035.3639$-00.1418$&35.36386&$ -0.14178$&5.0&0.15&0.06&0.28&0.06&...&...\\ 
G035.3669$+00.6548$&35.36691&$ +0.65484$&5.0&0.23&0.07&0.34&0.07&...&...\\ 
G035.3672$-00.0768$&35.36720&$ -0.07684$&5.2&0.18&0.06&0.31&0.06&...&...\\ 
G035.3712$-00.5935$&35.37122&$ -0.59345$&6.3&0.22&0.06&0.39&0.07&...&...\\ 
G035.3773$-00.5845$&35.37733&$ -0.58449$&5.1&0.14&0.06&0.29&0.06&...&...\\ 
G035.3856$-00.1064$&35.38560&$ -0.10643$&6.3&0.20&0.06&0.36&0.06&AB?&...\\ 
G035.3894$+00.6538$&35.38941&$ +0.65379$&5.1&0.19&0.07&0.33&0.07&...&...\\ 
G035.3898$-00.7811$&35.38976&$ -0.78110$&6.1&0.19&0.06&0.35&0.06&...&...\\ 
G035.4010$+00.3234$&35.40101&$ +0.32337$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G035.4063$-00.0386$&35.40629&$ -0.03858$&5.5&0.18&0.06&0.33&0.06&...&...\\ 
G035.4116$-00.4883$&35.41157&$ -0.48831$&5.2&0.19&0.06&0.33&0.07&...&...\\ 
G035.4208$-00.2279$&35.42081&$ -0.22789$&5.5&0.20&0.06&0.35&0.07&...&...\\ 
G035.4342$-00.0673$&35.43421&$ -0.06726$&5.2&0.16&0.06&0.32&0.06&...&...\\ 
G035.4373$+00.9922$&35.43726&$ +0.99223$&5.5&0.22&0.09&0.46&0.09&...&...\\ 
G035.4501$+00.2743$&35.45011&$ +0.27427$&5.0&0.19&0.07&0.32&0.07&...&...\\ 
G035.4523$-00.2949$&35.45234&$ -0.29490$&6.7&0.24&0.06&0.43&0.07&cor&G035.452-00.295\\ 
G035.4573$-00.0167$&35.45727&$ -0.01671$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G035.4643$-00.8513$&35.46428&$ -0.85125$&5.3&0.21&0.07&0.35&0.07&...&...\\ 
G035.4724$+00.8741$&35.47240&$ +0.87409$&6.6&0.22&0.06&0.38&0.06&---&G035.473+00.874\\ 
G035.4738$+00.0878$&35.47379&$ +0.08781$&6.8&0.27&0.07&0.46&0.07&...&...\\ 
G035.4782$+00.4277$&35.47824&$ +0.42767$&5.1&0.28&0.08&0.42&0.09&...&...\\ 
G035.4805$-00.7358$&35.48046&$ -0.73582$&5.1&0.17&0.06&0.30&0.06&...&...\\ 
G035.4819$-00.0985$&35.48192&$ -0.09851$&5.2&0.17&0.06&0.32&0.06&...&...\\ 
G035.4850$-00.5137$&35.48497&$ -0.51373$&5.1&0.18&0.06&0.31&0.07&...&...\\ 
G035.4891$-00.9756$&35.48914&$ -0.97564$&5.0&0.23&0.08&0.37&0.08&...&...\\ 
G035.4943$+00.5262$&35.49428&$ +0.52622$&5.7&0.21&0.06&0.34&0.06&...&...\\ 
G035.4948$+00.8555$&35.49477&$ +0.85555$&5.0&0.16&0.06&0.31&0.07&---&G035.495+00.856\\ 
G035.4962$-00.4152$&35.49622&$ -0.41518$&5.2&0.29&0.08&0.43&0.09&...&...\\ 
G035.5099$-00.1904$&35.50991&$ -0.19039$&5.6&0.21&0.06&0.34&0.06&...&...\\ 
G035.5107$-00.3611$&35.51074&$ -0.36108$&5.3&0.21&0.07&0.36&0.07&...&...\\ 
G035.5135$-00.6341$&35.51352&$ -0.63408$&5.1&0.15&0.06&0.31&0.06&...&...\\ 
G035.5215$-00.0831$&35.52150&$ -0.08309$&5.3&0.18&0.06&0.33&0.07&...&...\\ 
G035.5261$-00.8142$&35.52609&$ -0.81416$&5.1&0.22&0.06&0.32&0.07&---&G035.525-00.814\\ 
G035.5412$-00.7492$&35.54116&$ -0.74916$&6.2&0.23&0.07&0.40&0.07&...&...\\ 
G035.5463$-00.2068$&35.54629&$ -0.20684$&5.0&0.16&0.06&0.29&0.06&...&...\\ 
G035.5504$+00.1150$&35.55039&$ +0.11496$&5.2&0.17&0.06&0.32&0.06&...&...\\ 
G035.5565$+00.7432$&35.55651&$ +0.74325$&6.0&0.21&0.07&0.38&0.07&...&...\\ 
G035.5594$-00.5184$&35.55935&$ -0.51845$&5.2&0.19&0.07&0.36&0.07&...&...\\ 
G035.5633$-00.1639$&35.56331&$ -0.16386$&5.0&0.18&0.06&0.30&0.06&...&...\\ 
G035.5652$-00.4914$&35.56519&$ -0.49136$&5.5&1.06&0.10&0.51&0.09&---&G035.564-00.492(F)\\ 
G035.5716$-00.4532$&35.57157&$ -0.45317$&5.1&0.20&0.07&0.34&0.07&...&...\\ 
G035.5717$+00.0681$&35.57171&$ +0.06809$&6.9&0.45&0.08&0.55&0.09&...&...\\ 
G035.5726$+00.0679$&35.57261&$ +0.06795$&7.0&0.69&0.09&0.57&0.09&...&...\\ 
G035.5744$+00.0675$&35.57435&$ +0.06753$&6.1&0.92&0.09&0.53&0.09&...&...\\ 
G035.5770$-00.0289$&35.57699&$ -0.02893$&5.1&0.52&0.13&0.63&0.13&Mas&...\\ 
G035.5793$-00.5221$&35.57928&$ -0.52213$&5.5&0.22&0.07&0.37&0.07&...&...\\ 
G035.5796$-00.0321$&35.57956&$ -0.03212$&5.2&0.50&0.12&0.62&0.13&MoC&...\\ 
G035.5837$-00.1100$&35.58366&$ -0.11004$&5.7&0.19&0.06&0.35&0.06&...&...\\ 
G035.5992$+00.8113$&35.59922&$ +0.81131$&6.0&0.22&0.07&0.42&0.08&...&...\\ 
G035.6094$+00.6839$&35.60943&$ +0.68387$&5.0&0.15&0.07&0.33&0.07&...&...\\ 
G035.6111$-00.2412$&35.61109&$ -0.24122$&6.4&0.19&0.06&0.39&0.06&...&...\\ 
G035.6186$+00.1427$&35.61859&$ +0.14274$&5.2&0.16&0.06&0.31&0.06&...&...\\ 
G035.6216$-00.5865$&35.62158&$ -0.58651$&5.3&0.18&0.06&0.31&0.06&...&...\\ 
G035.6230$+00.4490$&35.62303&$ +0.44899$&5.3&0.18&0.06&0.33&0.07&...&...\\ 
G035.6303$+00.1015$&35.63032&$ +0.10149$&5.3&0.16&0.06&0.33&0.06&...&...\\ 
G035.6361$-00.7349$&35.63610&$ -0.73492$&6.6&0.22&0.07&0.42&0.07&...&...\\ 
G035.6385$+00.4164$&35.63845&$ +0.41642$&5.7&0.19&0.07&0.36&0.07&...&...\\ 
G035.6415$-00.6046$&35.64151&$ -0.60463$&5.1&0.17&0.06&0.32&0.07&...&...\\ 
G035.6419$-00.1764$&35.64185&$ -0.17636$&5.0&0.15&0.06&0.28&0.06&...&...\\ 
G035.6430$+00.5333$&35.64304&$ +0.53330$&5.2&0.17&0.06&0.33&0.07&...&...\\ 
G035.6471$-01.0115$&35.64708&$ -1.01148$&5.3&0.27&0.11&0.54&0.11&...&...\\ 
G035.6589$-00.1935$&35.65886&$ -0.19351$&5.0&0.16&0.06&0.30&0.06&...&...\\ 
G035.6589$+00.3289$&35.65894&$ +0.32892$&5.1&0.17&0.07&0.34&0.07&...&...\\ 
G035.6600$+00.3011$&35.65998&$ +0.30107$&5.9&0.20&0.07&0.37&0.07&...&...\\ 
G035.6671$+00.9088$&35.66715&$ +0.90882$&5.1&0.14&0.06&0.29&0.06&...&...\\ 
G035.6718$-00.7303$&35.67179&$ -0.73027$&5.3&0.16&0.06&0.32&0.06&...&...\\ 
G035.6796$-00.5278$&35.67964&$ -0.52782$&5.1&0.17&0.06&0.30&0.06&...&...\\ 
G035.6907$-00.0947$&35.69074&$ -0.09469$&5.0&0.19&0.06&0.31&0.07&...&...\\ 
G035.7025$-00.9749$&35.70250&$ -0.97488$&6.8&0.28&0.07&0.48&0.08&...&...\\ 
G035.7059$+00.7198$&35.70589&$ +0.71984$&5.0&0.14&0.06&0.32&0.07&...&...\\ 
G035.7080$-00.1568$&35.70803&$ -0.15684$&5.2&0.18&0.07&0.34&0.07&...&...\\ 
G035.7118$-00.4371$&35.71179&$ -0.43706$&5.1&0.18&0.07&0.32&0.07&...&...\\ 
G035.7174$+00.2404$&35.71741&$ +0.24038$&6.7&0.22&0.06&0.41&0.07&...&...\\ 
G035.7188$-00.6722$&35.71881&$ -0.67221$&5.1&0.22&0.07&0.33&0.07&...&...\\ 
G035.7258$-00.5133$&35.72582&$ -0.51331$&6.3&0.22&0.06&0.39&0.07&...&...\\ 
G035.7297$-00.5712$&35.72971&$ -0.57123$&5.3&0.20&0.07&0.33&0.07&...&...\\ 
G035.7329$+00.3628$&35.73290&$ +0.36281$&6.7&0.23&0.07&0.44&0.07&---&G035.733+00.363\\ 
G035.7338$+00.2917$&35.73380&$ +0.29170$&5.4&0.15&0.07&0.34&0.07&...&...\\ 
G035.7349$-00.7982$&35.73486&$ -0.79819$&5.0&0.20&0.07&0.34&0.07&...&...\\ 
G035.7365$+00.2189$&35.73651&$ +0.21892$&5.2&0.16&0.06&0.33&0.07&...&...\\ 
G035.7379$-00.4357$&35.73790&$ -0.43574$&5.2&0.15&0.06&0.32&0.06&...&...\\ 
G035.7433$+00.7635$&35.74333&$ +0.76353$&5.2&0.19&0.06&0.32&0.07&...&...\\ 
G035.7444$+00.4775$&35.74436&$ +0.47754$&5.1&0.14&0.06&0.32&0.07&...&...\\ 
G035.7492$-00.9156$&35.74917&$ -0.91556$&5.3&0.19&0.07&0.34&0.07&...&...\\ 
G035.7677$+00.3127$&35.76769&$ +0.31274$&5.3&0.20&0.07&0.35&0.07&...&...\\ 
G035.7715$+00.8446$&35.77146&$ +0.84458$&6.0&0.22&0.07&0.39&0.07&...&...\\ 
G035.7729$-00.8383$&35.77285&$ -0.83826$&5.4&0.21&0.07&0.39&0.08&...&...\\ 
G035.7748$+00.4354$&35.77484&$ +0.43538$&5.0&0.20&0.07&0.33&0.07&...&...\\ 
G035.7761$+00.4306$&35.77609&$ +0.43059$&5.3&0.19&0.07&0.36&0.07&...&...\\ 
G035.7781$-00.2031$&35.77810&$ -0.20309$&5.6&0.20&0.06&0.36&0.07&...&...\\ 
G035.7781$-00.4057$&35.77811&$ -0.40574$&5.0&0.18&0.06&0.31&0.07&...&...\\ 
G035.7793$+00.0427$&35.77928&$ +0.04267$&6.0&0.23&0.06&0.36&0.06&...&...\\ 
G035.7822$+00.6340$&35.78222&$ +0.63400$&5.1&0.22&0.06&0.31&0.07&...&...\\ 
G035.7831$-00.4827$&35.78311&$ -0.48268$&5.2&0.17&0.07&0.34&0.07&...&...\\ 
G035.7831$+00.7082$&35.78312&$ +0.70817$&5.0&0.19&0.06&0.31&0.06&...&...\\ 
G035.7853$-00.6198$&35.78534&$ -0.61977$&5.1&0.18&0.06&0.32&0.07&...&...\\ 
G035.7864$-00.2971$&35.78644&$ -0.29712$&5.1&0.17&0.06&0.32&0.06&...&...\\ 
G035.7962$+00.1141$&35.79623&$ +0.11406$&5.0&0.17&0.06&0.31&0.07&...&...\\ 
G035.8091$-00.6642$&35.80909&$ -0.66422$&6.0&0.29&0.07&0.41&0.07&...&...\\ 
G035.8119$-00.3852$&35.81193&$ -0.38518$&5.4&0.20&0.07&0.36&0.07&---&G035.812-00.385\\ 
G035.8127$+00.8882$&35.81272&$ +0.88819$&5.1&0.17&0.06&0.30&0.06&...&...\\ 
G035.8132$+00.5825$&35.81319&$ +0.58254$&5.2&0.20&0.06&0.32&0.06&...&...\\ 
G035.8142$+00.8872$&35.81418&$ +0.88722$&5.2&0.16&0.06&0.31&0.06&...&...\\ 
G035.8177$+00.9421$&35.81773&$ +0.94209$&5.2&0.16&0.06&0.30&0.06&...&...\\ 
G035.8191$-00.2862$&35.81908&$ -0.28615$&5.3&0.18&0.06&0.32&0.06&...&...\\ 
G035.8205$+00.0432$&35.82046&$ +0.04316$&5.1&0.16&0.06&0.31&0.06&...&...\\ 
G035.8210$-00.4126$&35.82103&$ -0.41261$&5.4&0.16&0.06&0.34&0.07&...&...\\ 
G035.8319$-00.9888$&35.83190&$ -0.98877$&6.9&0.35&0.08&0.56&0.09&...&...\\ 
G035.8353$+00.0657$&35.83525&$ +0.06566$&6.7&0.22&0.06&0.42&0.07&...&...\\ 
G035.8471$-00.1288$&35.84706&$ -0.12879$&5.0&0.18&0.06&0.29&0.06&...&...\\ 
G035.8517$-00.6971$&35.85174&$ -0.69707$&5.2&0.16&0.07&0.35&0.07&...&...\\ 
G035.8573$+00.8823$&35.85731&$ +0.88229$&5.0&0.18&0.06&0.31&0.07&...&...\\ 
G035.8599$-00.3753$&35.85992&$ -0.37532$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G035.8603$-00.8360$&35.86029&$ -0.83604$&5.3&0.18&0.07&0.34&0.07&...&...\\ 
G035.8636$-00.9515$&35.86357&$ -0.95154$&5.4&0.23&0.07&0.38&0.07&...&...\\ 
G035.8653$-00.6151$&35.86535&$ -0.61512$&5.4&0.23&0.06&0.34&0.07&...&...\\ 
G035.8689$+00.3475$&35.86887&$ +0.34746$&5.1&0.19&0.08&0.38&0.08&...&...\\ 
G035.8707$-00.1434$&35.87067&$ -0.14344$&5.2&0.18&0.06&0.32&0.07&...&...\\ 
G035.8710$-00.1949$&35.87102&$ -0.19490$&5.4&0.18&0.06&0.33&0.07&...&...\\ 
G035.8720$-00.9877$&35.87205&$ -0.98773$&5.0&0.22&0.08&0.40&0.08&...&...\\ 
G035.8776$+00.6481$&35.87764&$ +0.64810$&6.9&0.25&0.07&0.45&0.07&---&G035.878+00.648\\ 
G035.8783$+00.6603$&35.87827&$ +0.66032$&6.7&0.21&0.06&0.41&0.06&---&G035.878+00.660\\ 
G035.8812$-00.3155$&35.88116&$ -0.31553$&5.1&0.16&0.06&0.32&0.07&...&...\\ 
G035.8879$-00.0856$&35.88790&$ -0.08559$&5.2&0.17&0.06&0.32&0.06&...&...\\ 
G035.8914$+00.1455$&35.89137&$ +0.14552$&6.5&0.23&0.07&0.45&0.08&...&...\\ 
G035.8933$+00.5591$&35.89326&$ +0.55914$&5.0&0.19&0.07&0.34&0.07&...&...\\ 
G035.8983$-00.6220$&35.89833&$ -0.62200$&5.3&0.16&0.06&0.32&0.07&...&...\\ 
G035.8985$+00.3400$&35.89853&$ +0.33996$&5.6&0.24&0.08&0.45&0.08&...&...\\ 
G035.9031$-01.0127$&35.90310&$ -1.01266$&6.5&0.41&0.11&0.68&0.11&...&...\\ 
G035.9073$+00.9670$&35.90726&$ +0.96702$&5.3&0.20&0.07&0.35&0.07&...&...\\ 
G035.9112$-00.8633$&35.91121&$ -0.86334$&5.0&0.18&0.06&0.32&0.07&...&...\\ 
G035.9200$+01.0079$&35.92004&$ +1.00793$&5.3&0.30&0.10&0.51&0.10&...&...\\ 
G035.9229$-00.7186$&35.92286&$ -0.71860$&5.0&0.17&0.07&0.32&0.07&...&...\\ 
G035.9241$-00.3807$&35.92409&$ -0.38067$&5.2&0.20&0.07&0.34&0.07&...&...\\ 
G035.9304$+00.5862$&35.93042&$ +0.58615$&5.1&0.20&0.07&0.34&0.07&...&...\\ 
G035.9341$+00.8974$&35.93406&$ +0.89743$&5.0&0.20&0.07&0.33&0.07&...&...\\ 
G035.9394$-00.6168$&35.93938&$ -0.61679$&5.6&0.19&0.06&0.35&0.07&---&G035.939-00.617\\ 
G035.9420$-00.6501$&35.94195&$ -0.65005$&5.1&0.17&0.06&0.31&0.06&...&...\\ 
G035.9449$-00.7002$&35.94494&$ -0.70020$&6.8&0.23&0.07&0.44&0.07&...&...\\ 
G035.9556$-00.0659$&35.95560&$ -0.06594$&5.1&0.21&0.07&0.34&0.07&...&...\\ 
G035.9558$-00.6360$&35.95584&$ -0.63595$&5.6&0.20&0.07&0.37&0.07&---&G035.955-00.636\\ 
G035.9564$-00.1150$&35.95637&$ -0.11504$&5.0&0.18&0.07&0.33&0.07&...&...\\ 
G035.9576$-00.3954$&35.95763&$ -0.39539$&6.1&0.22&0.07&0.44&0.08&...&...\\ 
G035.9578$+00.3370$&35.95777&$ +0.33698$&5.6&0.37&0.11&0.58&0.11&...&...\\ 
G035.9640$-00.4321$&35.96402&$ -0.43213$&5.3&0.22&0.08&0.39&0.08&...&...\\ 
G035.9695$+00.8367$&35.96947&$ +0.83666$&5.4&0.24&0.07&0.39&0.08&...&...\\ 
G035.9709$-00.9631$&35.97095&$ -0.96307$&6.6&0.28&0.08&0.55&0.09&---&G035.971-00.963\\ 
G035.9712$-00.0619$&35.97123&$ -0.06191$&5.4&0.24&0.07&0.38&0.07&...&...\\ 
G035.9828$+00.3830$&35.98284&$ +0.38302$&5.2&0.33&0.11&0.57&0.11&...&...\\ 
G035.9850$-00.7080$&35.98502&$ -0.70797$&5.1&0.20&0.08&0.40&0.08&...&...\\ 
G035.9869$-00.0763$&35.98686&$ -0.07629$&5.1&0.19&0.08&0.40&0.08&...&...\\ 
G035.9910$+00.7142$&35.99099&$ +0.71422$&5.2&0.27&0.09&0.44&0.09&...&...\\ 
G035.9928$-00.6868$&35.99279&$ -0.68679$&5.2&0.23&0.08&0.42&0.08&...&...\\ 
G035.9989$-00.1350$&35.99894&$ -0.13504$&5.0&0.26&0.09&0.47&0.10&...&...\\ 
\hline
 \end{tabular}
 \end{minipage}
\end{center}
\end{table*}
